Learning Dynamical Systems with Side Information

We present a mathematical and computational framework for the problem of learning a dynamical system from noisy observations of a few trajectories and subject to side information. Side information is any knowledge we might have about the dynamical system we would like to learn besides trajectory data. It is typically inferred from domain-specific knowledge or basic principles of a scientific discipline. We are interested in explicitly integrating side information into the learning process in order to compensate for scarcity of trajectory observations. We identify six types of side information that arise naturally in many applications and lead to convex constraints in the learning problem. First, we show that when our model for the unknown dynamical system is parameterized as a polynomial, one can impose our side information constraints computationally via semidefinite programming. We then demonstrate the added value of side information for learning the dynamics of basic models in physics and cell biology, as well as for learning and controlling the dynamics of a model in epidemiology. Finally, we study how well polynomial dynamical systems can approximate continuously-differentiable ones while satisfying side information (either exactly or approximately). Our overall learning methodology combines ideas from convex optimization, real algebra, dynamical systems, and functional approximation theory, and can potentially lead to new synergies between these areas.

==> Learning with Side Info r1 -arxiv submission jan 17 2022 compressed/abstract.tex <==
We present a mathematical formalism of the problem of
learning a dynamical system from (scarce and limited)
observed trajectories and contextual side information
(e.g. physical laws or contextual knowledge). We show
that sum of squares optimization is particularly suited
for learning a dynamical system that best agrees with the
observations and respects the side information.  We
demonstrate the efficacy of our learning technique to
applications from epidemiology and physics.

% In several safety-critical applications, one has
% to learn the behavior of an unknown dynamical
% system from noisy observations of a very limited
% number of trajectories. For example, to
% autonomously land an airplane that has just gone
% through engine failure, limited time is available
% to learn the modified dynamics of the plane before
% appropriate control action can be
% taken. Similarly, when a new infectious disease
% breaks out, few observations are initially
% available to understand the dynamics of contagion.
% In situations of this type where data is limited,
% it is essential to 


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "Learning_with_side_information_L4DC_v1"
%%% End:


==> Learning with Side Info r1 -arxiv submission jan 17 2022 compressed/applications.tex <==
\section{Illustrative Experiments}

\subsection{Diffusion of a contagious disease}
The following dynamical system has appeared in the epidemiology literature (see, e.g., \cite{anderson1992infectious}) as a model for the spread of Gonorrhea in a heterosexual population:
\begin{equation}  \label{eq:diffusion_disease}
    \dot \ix = f(\ix)
  \quad \text{where} \; \ix \in \R^2 \text{ and }
  f(\ix) = \left(
    \begin{array}{l}
      -a_1   x_1 + b_1 (1-x_1) x_2\\
      -a_2   x_2 + b_2 (1-x_1) x_2
    \end{array}\right).
\end{equation}
Here, the quantity $x_1(t)$ (resp. $x_2(t)$) represents the fraction of infected males (resp. females). The parameters $a_i$ and $b_i$ denotes the recovery and infection rates respectively for males when $i=1$, and for females when $i=2$. We take \[(a_1, b_1, a_2, b_2) = (0.05 , 0.1, 0.05, 0.1),\] and we plot the resulting vector field $f$ in \cref{fig:vf_diffusion_disease}. We suppose that this vector field is unknown to us, and our goal is to approximate it based on the noisy sample observations
\[ \mathcal D \coloneqq \left\{ (\ix(t_i), f(\ix(t_i))+ 10^{-4} \begin{pmatrix}\varepsilon_i^1\\\varepsilon_i^2\end{pmatrix}) \right\}_{i=1}^{20}, \]
where $\ix(t, x_0)$ is the trajectory obtained when the flow in \eqref{eq:diffusion_disease} is started from the initial condition $\ix_0 = (0.7, 0.3)^T$, the $t_i \coloneqq  i/20$ represent regular subdivision of the time interval $[0, 1]$, and the $\varepsilon_i^{1}, \varepsilon_i^{2}$ are independent standard normal variables.

\begin{figure}
  \centering
  % Vertical alignment is controlled through optional argumants [c], [t] or [b] of minipage`.
  \begin{minipage}[c]{.5\textwidth}
    \includegraphics[width=.5\textwidth, trim=0 10 0 0, clip]{imgs/disease/disease_true_vf.png}
  \end{minipage}
  \begin{minipage}[c]{.4\textwidth}
    \caption{\label{fig:vf_diffusion_disease}The vector field in \eqref{eq:diffusion_disease} corresponding to $(a_1, a_2, b_1, b_2, c_1, c_2) = (.05,.1,.05,.1,1.,1.)$ together with a sample trajectory.}
  \end{minipage}
\end{figure}

Following our methodology in \cref{sec:learn-poly-vec}, we
parameterize our candidate vector field $p: \R^2 \rightarrow \R^2$ as
a polynomial of degree $d$, and we minimize the least square error
between the values taken by the vector fields $f$ and $p$ on the
observed trajectories; i.e., we solve the following convex
optimization problem:

\begin{equation}
  \min_{p \in \mathcal P_d} \sum_{(\ix_i, \iy_i) \in \mathcal D} \| p(\ix_i) - \iy_i\|^2.\label{eq:disease-fitting-polynomial-lsq}
\end{equation}

Note that the ground vector field $f$ is a polynomial of degree
$2$. In the following, we pretend that $f$ is unknown to us and we
consider an over-parameterized model of the truth by taking $d=3$.  To
help with the task of learning, we consider, the following list of side
information (that we can guess without knowing the exact structure
$f$). We also show that the imposing this side information leads to a
semidefinite programming constraints.

\begin{itemize}
\item {\bf Equilibrium point at the origin.} A disease cannot spread
  if no male or female is already infected. This corresponds to our
  vector field $p$ having an equilibrium at the origin, i.e.,
  $p(0, 0) = 0$. The is a simple linear constraint that we add to our
  optimization problem in \eqref{eq:disease-fitting-polynomial-lsq}.
  
\item {\bf Invariance of the box $[0, 1] \times [0, 1]$.} The
  components of a trajectory $\ix(t)$ following the dynamics in
  \eqref{eq:diffusion_disease} represents fractions, and as such, the
  vector $\ix(t)$ should be contained in the box
  $[0, 1] \times [0, 1]$ at all times $t \ge 0$. Mathematically, this
  corresponds to the constraints
  %
  \[p_2(x_1, 0) \ge 0, p_2(x_1, 1) \le 0 \quad \forall x_1 \in [0, 1],
    \quad p_1(0, x_2) \ge 0, p_2(1, x_2) \ge 0 \quad \forall x_2 \in
    [0, 1],\]
  %
  which imply that the vector field is pointing inwards on
  the boundaries of the unit box.
  % 
  Note that since
  $[0, 1] = \{ u \in \R \; | \; u \ge 0, 1-u \ge 0 \}$, the set
  $[0, 1]$ is closed semialgebraic. Following our discussion in
  \cref{sec:learn-poly-vec}, we replace these nonnegativity
  constraints with their corresponding Putinar's certificate in
  \eqref{eq:putinar-certificate} of degree two. For instance, we
  replace the constraint $p_2(x_1, 0) \ge 0$ with the linear
  constraints obtained from equating the coefficients of the two side
  of the polynomial equation
  $p_2(x_1, 0) = x_1s_0(x_1) + (1-x_1) s_1(x_1)$.  Here, the new
  decision variables $s_0$ and $s_1$ are (univariate) quadratic
  sum-of-squares polynomials.
  
\item {\bf Directional monotonicity.}
%
  We expect that, everything else being equal, if the fraction of
  males infected rises in the population, the rate of infection of
  females should increase. Mathematically, we can write
  \[\frac {\partial p_2}{\partial x_1}(\ix) \ge 0 \quad \forall \ix
    \in [0, 1]^2.\]
%
  Similarly, by changing the roles played by males and females, we
  obtain the constraint
    \[\frac {\partial p_1}{\partial x_2}(\ix) \ge 0 \quad \forall \ix
      \in [0, 1]^2.\]
%
    Note again that $[0, 1]^2$ is closed semialgebraic, so in the same
    spirit as the previous bullet point, we replace each one of these
    constraints with their corresponding Putinar's certificate of
    degree two.
\end{itemize}


We show in \cref{fig:disease-lsq-deg-3} the streamplot of the best
polynomial vector fields of degree $3$ obtained by solving the
least-squares problem in \eqref{eq:disease-fitting-polynomial-lsq} and
imposing some or all of the side information above.


\begin{figure}
  \subfigure[Least-squares\\ solution]{
    \includegraphics[width=.25\textwidth, trim=0 10 0 0, clip]{imgs/disease/deg_3_no_side_info.png}}~\;~
  \subfigure[Equilibrium at\\ the origin]{
    \includegraphics[width=.25\textwidth, trim=0 10 0 0, clip]{imgs/disease/deg_3_eq.png}}~\;~
  \subfigure[Equilibrium \\+ Invariance]{
    \includegraphics[width=.25\textwidth, trim=0 10 0 0, clip]{imgs/disease/deg_3_eq_invariance.png}}~\;~
  \subfigure[Equilibrium \\+ Invariance \\+ Monotonicity]{
    \includegraphics[width=.25\textwidth, trim=0 10 0 0, clip]{imgs/disease/deg_3_eq_invariance_monotone.png}}
  \caption{\label{fig:disease-lsq-deg-3}Streamplot of the best
  polynomial solution of degree 2 fitting the vector field $f$ defined
in \eqref{eq:diffusion_disease}}
\end{figure}


% \newcommand{\plotvfdisease}[2]{
%   \begin{minipage}[b]{.48\textwidth}
%     \begin{tikzpicture}[scale=.7]
%       \loadvf{data/disease/disease_segments_#1.csv}{data/disease/disease_arrows_#1.csv}
%       \begin{axis}[no markers, enlargelimits=false]
%         \boxtikz
%         %\draw[red, thick] (0, 0) circle (.3cm);
%         \plotsegmentsvf{}
%         \plotarrowsvf{}
%       \end{axis}
%   \end{tikzpicture}
%   \caption{#2}
%   \end{minipage}
% }
% \tikzsetnextfilename{disease_poly_deg_3_vf_pdf}
% \begin{figure}[H]
%   \centering
%   \plotvfdisease{deg_3_no_side_info}{\label{fig:deg-3-node-side-info}No
%   side information}~%
%   \plotvfdisease{deg_3_eq}{\label{fig:deg-3-eq}Equilibrium point at
%     the origin.}\\
%   \plotvfdisease{deg_3_eq_invariance}{\label{fig:deg-3-eq-invariance}Equilibrium point at the origin and invariance of the box $[0,1]\times[0,1]$.}~\plotvfdisease{deg_3_eq_invariance_monotone}{\label{fig:deg-3-eq-invariance-monotone}Equilibrium point at the origin, invariance of the box $[0,1]\times[0,1]$, and monotonicity.}
%   \caption{\label{fig:disease-lsq-deg-3}Streamplot of the best
%     polynomial vector fields of degree 3 solution to \eqref{eq:disease-fitting-polynomial-lsq} and satisfying additiona side information.}
% \end{figure}


\subsection{The simple pendulum}

\tikzsetnextfilename{simple_pendulum_pdf}
\begin{figure}[H]
  \centering
  \begin{minipage}[c]{.6\textwidth}
  \input{img/simple_pendulum.tikz}\quad\quad\quad\quad\quad\quad
  \includegraphics[width=.5\textwidth]{imgs/pendulum/pendulum_true_vf_with_data.png}
\end{minipage}
\begin{minipage}[c]{.3\textwidth}
  \caption{\label{fig:simple-pendulum}(Left) Simple pendulum. (Right) Phase portrait of the simple pendulum.}
\end{minipage}
\end{figure}

In this section we consider the simple pendulum system, i.e., a mass
$m$ hanging from a mass-less string of length $\ell$ and attached to a
fixed point $O$ (see \cref{fig:simple-pendulum}). By applying Newton's
second law for rotational systems, the equation of motion for the
pendulum may be obtained
\[ \ddot \theta = -\frac g\ell \sin \theta,\] where $g$ is is the
local acceleration of gravity.  This is a one-dimensional second-order
system. We convert it to a first-order system as follows.
\begin{equation}
\begin{pmatrix}\ddot \theta\\\dot \theta\end{pmatrix} =  f(\dot \theta, \theta) \coloneqq \begin{pmatrix}-\frac g\ell \sin \theta\\\dot \theta\end{pmatrix}.\label{eq:ode-pendulum}
\end{equation}


We take the vector field in \eqref{eq:ode-pendulum} to be the ground
truth with $g=\ell=1$, and we generate from it two noisy trajectories
$\theta_1$ and $\theta_2$ sampled at times $t_k = k/5$. More
precisely, we assume that we have the following data
\begin{equation}
  \mathcal D \coloneqq \left\{ (\ddot \theta_1(t_k), \dot \theta_1(t_k), \theta_1(t_k)) + 10^{-2} \varepsilon_k^1 \right\}_{k=0, \ldots, 5} \cup \left\{ (\ddot \theta_2(t_k), \dot \theta_2(t_k), \theta_2(t_k)) + 10^{-2} \varepsilon_k^2 \right\}_{k=0, \ldots, 5},\label{eq:data-pendulum}
\end{equation}
%
where the trajectory $\theta_1$ (resp. $\theta_2$) was obtained by
displacing the mass from to an initial angle $\frac \pi 3$ (resp.
$\frac{9\pi}{20}$) and released with a zero initial angular velocity,
and the $\varepsilon^i_k$ (for $i=1,2$ and $k=0,\ldots,5$) are
independent $3 \times 1$ normal vectors. The trajectories $\theta_1$
and $\theta_2$ together with the training data is plotted in
\cref{fig:trajectory-pendulum}.


We are interested in learning the vector field $f$ over the set
$\Omega = [-\pi, \pi]^2$ from the training data in
\eqref{eq:data-pendulum} and the side information below. We
parameterize our candidate vector field $p$ as a $\text{degree-}5$
polynomial.

\begin{itemize}
\item{\bf Hamiltonian.} The system in \eqref{eq:ode-pendulum} is {Hamiltonian}. Indeed,
  we assume that there is no dissipation of energy (through resistance
  of the air for example) so the total energy associated to the
  pendulum is conserved and is a Hamiltonian associated with the
  system.
  \begin{equation}
    E(\theta, \dot \theta) = \frac m2 {\dot \theta}^2 + \frac12 \frac gl (1 - \cos(\theta))\label{eq:total-energy-pendulum}
  \end{equation}
  The two terms appearing in the left can be interpreted physically as
  the kinetic energy and potential energy. Note that neither the
  vector field in \eqref{eq:ode-pendulum} describing the dynamics of
  the simple pendulum or the associated Hamiltonian in
  \eqref{eq:total-energy-pendulum} are polynomial functions.  In our
  learning procedure, we use only the fact that the system is
  Hamiltonian, i.e., that there exists a function $H$ such that
%
  \[ p_1(\dot \theta, \theta) = - \frac{\partial H}{\partial \dot
      \theta}(\dot \theta, \theta), \quad p_2(\dot \theta, \theta) =
    \frac{\partial H}{\partial \theta}(\dot \theta, \theta), \]
%
  but not the exact form of this Hamiltonian
  \eqref{eq:total-energy-pendulum}. Note that this is an affine
  constraint in the coefficients of the polynomial $p$.
  
\item {\bf Symmetry.} The pendulum system in \cref{fig:simple-pendulum} is symmetric
  with respect the vertical dotted axis. Then, our candidate vector
  field $p$ needs to satisfy the same symmetries.
  \[p(- \dot \theta, - \theta) = - p(\dot \theta, \theta) \quad
    \forall \theta, \dot \theta \in \R.\] Note that this is again an
  affine constraint in the coefficients of the polynomial $p$.
\item {\bf Coordinate nonnegativity.} The only external force applied on the pendulum system is gravitational force represented by the vector $g$ in \cref{fig:simple-pendulum}. This force pulls the mass down and pushes the angle $\theta$ towards $0$. In other terms, the angular velocity $\dot \theta$  decreases when $\theta$ is positive and increases when $\theta$ is negative. 
Mathematically,
\[p_2(\dot \theta, \theta) \le 0 \; \forall (\dot\theta,\theta) \in
  [-\pi, \pi] \times [0, \pi] \text{ and } p_2(\dot \theta, \theta)
  \ge 0 \; \forall (\dot\theta,\theta) \in [-\pi, \pi]\times [-\pi,
  0].\]
We replace each one of these constraints with their corresponding Putinar's certificate of degree $5$.
(Note that, because of symmetry, we actually only need to impose the first of these two constraints.)
\end{itemize}



\begin{figure}
  \subfigure[Least-squares solution]{
    \includegraphics[width=.25\textwidth, trim=0 10 0 0,
    clip]{imgs/pendulum/deg_5_sym_false_sign_false_hamiltonian_false.png}}~\;~
  \subfigure[Symmetry]{ \includegraphics[width=.25\textwidth,
    trim=0 10 0 0,
    clip]{imgs/pendulum/deg_5_sym_true_sign_false_hamiltonian_false.png}}~\;~
  \subfigure[Symmetry + Sign]{\includegraphics[width=.25\textwidth, trim=0 10 0 0,
    clip]{imgs/pendulum/deg_5_sym_true_sign_true_hamiltonian_false.png}}~\;~
  \subfigure[Symmetry \\+ Sign \\+ Hamiltonian]{\includegraphics[width=.25\textwidth, trim=0 10
    0
    0,clip]{imgs/pendulum/deg_5_sym_true_sign_false_hamiltonian_true.png}}
  
  \caption{\label{fig:simple-pendulum-learned-vf}Streamplots of learned vector fields of degree 5.}
\end{figure}

\input{imgs/pendulum/trajectory_pendulum.tikz}

%%% Local Variables:
%%% mode: latex
%%% TeX-engine: default
%%% TeX-master: "Learning_with_side_information_L4DC_v1"
%%% End:


==> Learning with Side Info r1 -arxiv submission jan 17 2022 compressed/data/tables/disease.tex <==


\section*{Diffusion of a contagious disease, degree = $2$}\\
\begin{tabular}{ll|rr|rr|rr}
\toprule
      & {} & \multicolumn{2}{l}{training error} & \multicolumn{2}{l}{test error (vector field)} & \multicolumn{2}{l}{test error (trajectories)} \\
      & side information used? $\rightarrow$ &         no &     yes &        no &     yes &     no &     yes \\
noise & \# trajectories $\downarrow$ &           &       &          &       &       &       \\
\midrule
\multirow{3}{*}{0.001} & 1 &     0.001 & 0.001 &      189 & 0.068 &   $\infty$ & 0.008 \\
      & 2 &     0.001 & 0.002 &    0.044 & 0.081 & 0.004 & 0.005 \\
      & 3 &     0.001 & 0.002 &    0.018 & 0.083 & 0.002 & 0.005 \\
\cline{1-8}
\multirow{3}{*}{0.010} & 1 &     0.008 & 0.009 & 1.89e+03 & 0.071 &   $\infty$ & 0.012 \\
      & 2 &     0.008 & 0.009 &    0.444 & 0.061 & 0.031 & 0.004 \\
      & 3 &     0.009 & 0.009 &    0.179 & 0.074 &   $\infty$ & 0.006 \\
\cline{1-8}
\multirow{3}{*}{0.100} & 1 &      0.08 & 0.087 & 1.89e+04 & 0.075 &   $\infty$ &  0.02 \\
      & 2 &     0.085 & 0.088 &     4.44 & 0.068 &   $\infty$ & 0.019 \\
      & 3 &     0.086 & 0.088 &     1.78 &  0.11 &   $\infty$ & 0.016 \\
\bottomrule
\end{tabular}

\section*{Diffusion of a contagious disease, degree = $3$}\\
\begin{tabular}{ll|rr|rr|rr}
\toprule
      & {} & \multicolumn{2}{l}{training error} & \multicolumn{2}{l}{test error (vector field)} & \multicolumn{2}{l}{test error (trajectories)} \\
      & side information used? $\rightarrow$ &         no &     yes &        no &     yes &     no &     yes \\
noise & \# trajectories $\downarrow$ &           &       &          &       &       &       \\
\midrule
\multirow{3}{*}{0.001} & 1 &     0.001 & 0.001 &      229 &  4.22 &  $\infty$ & 0.065 \\
      & 2 &     0.001 & 0.001 &     21.8 & 0.248 &  $\infty$ & 0.005 \\
      & 3 &     0.001 & 0.001 &     1.65 & 0.151 &  $\infty$ & 0.004 \\
\cline{1-8}
\multirow{3}{*}{0.010} & 1 &     0.008 & 0.008 & 2.29e+03 &  43.4 &  $\infty$ & 0.581 \\
      & 2 &     0.008 & 0.009 &      218 &  0.47 &  $\infty$ & 0.013 \\
      & 3 &     0.008 & 0.009 &     16.5 & 0.292 &  $\infty$ & 0.007 \\
\cline{1-8}
\multirow{3}{*}{0.100} & 1 &     0.079 & 0.084 & 2.29e+04 &   435 &  $\infty$ &   5.8 \\
      & 2 &     0.082 & 0.087 & 2.18e+03 &  2.64 &  $\infty$ & 0.079 \\
      & 3 &     0.084 & 0.087 &      165 & 0.982 &  $\infty$ & 0.023 \\
\bottomrule
\end{tabular}

\section*{Diffusion of a contagious disease, degree = $4$}\\
\begin{tabular}{ll|rr|rr|rr}
\toprule
      & {} & \multicolumn{2}{l}{training error} & \multicolumn{2}{l}{test error (vector field)} & \multicolumn{2}{l}{test error (trajectories)} \\
      & side information used? $\rightarrow$ &         no &     yes &        no &     yes &     no &     yes \\
noise & \# trajectories $\downarrow$ &           &       &          &       &       &       \\
\midrule
\multirow{3}{*}{0.001} & 1 &     0.001 & 0.001 & 1.63e+04 &     21.7 &  $\infty$ & 0.092 \\
      & 2 &     0.001 & 0.001 & 2.58e+03 &    0.726 &  $\infty$ & 0.004 \\
      & 3 &     0.001 & 0.001 &      421 &    0.575 &  $\infty$ & 0.002 \\
\cline{1-8}
\multirow{3}{*}{0.010} & 1 &     0.008 & 0.008 & 1.62e+05 &      191 &  $\infty$ & 0.822 \\
      & 2 &     0.008 & 0.009 & 2.58e+04 &     1.83 &  $\infty$ & 0.046 \\
      & 3 &     0.008 & 0.009 & 4.21e+03 &     1.53 &  $\infty$ & 0.031 \\
\cline{1-8}
\multirow{3}{*}{0.100} & 1 &     0.076 & 0.083 & 1.57e+06 & 1.92e+03 &  $\infty$ &  8.22 \\
      & 2 &     0.079 & 0.087 & 2.58e+05 &     8.01 &  $\infty$ & 0.018 \\
      & 3 &     0.081 & 0.087 & 4.21e+04 &     7.99 &  $\infty$ & 0.017 \\
\bottomrule
\end{tabular}


==> Learning with Side Info r1 -arxiv submission jan 17 2022 compressed/data/tables/disease_10_samples.tex <==

\section*{Diffusion of a contagious diseas, degree = $2$}\\

\begin{tabular}{llrrrr|rrrr|rrrr}
\toprule
      & {} & \multicolumn{4}{l}{training error} & \multicolumn{4}{l}{test error (vector field)} & \multicolumn{4}{l}{test error (trajectories)} \\
      & \# side information: &         0 &     1 &     2 &     3 &        0 &     1 &     2 &     3 &     0 &     1 &     2 &     3 \\
noise & \# trajectories &           &       &       &       &          &       &       &       &       &       &       &       \\
\midrule
\multirow{4}{*}{0.001} & 1 &     0.001 & 0.001 & 0.001 & 0.001 &      219 &  4.42 & 0.863 &  0.09 &   $\infty$ &   $\infty$ & 0.048 &  0.01 \\
      & 2 &     0.001 & 0.001 & 0.002 & 0.002 &    0.061 & 0.019 & 0.076 & 0.076 & 0.004 & 0.002 & 0.005 & 0.005 \\
      & 3 &     0.001 & 0.001 & 0.002 & 0.002 &    0.015 & 0.016 & 0.083 & 0.083 & 0.002 & 0.002 & 0.006 & 0.006 \\
      & 4 &     0.001 & 0.001 & 0.002 & 0.002 &    0.006 & 0.006 & 0.065 & 0.074 &     0 &     0 & 0.002 & 0.003 \\
\cline{1-14}
\multirow{4}{*}{0.010} & 1 &     0.008 & 0.008 &  0.01 &  0.01 & 2.19e+03 &  44.2 &  1.08 & 0.098 &   $\infty$ &   $\infty$ & 0.095 & 0.012 \\
      & 2 &      0.01 &  0.01 &  0.01 &  0.01 &    0.612 & 0.191 & 0.148 &   0.1 & 0.044 &  0.02 & 0.017 & 0.012 \\
      & 3 &      0.01 &  0.01 &  0.01 &  0.01 &    0.147 & 0.159 & 0.129 &   0.1 & 0.015 & 0.015 & 0.012 &  0.01 \\
      & 4 &      0.01 &  0.01 &  0.01 &  0.01 &    0.063 & 0.056 & 0.082 & 0.086 & 0.003 & 0.003 & 0.004 & 0.004 \\
\cline{1-14}
\multirow{4}{*}{0.100} & 1 &     0.082 & 0.083 & 0.096 & 0.098 & 2.19e+04 &   442 &  6.15 & 0.588 &   $\infty$ &   $\infty$ & 0.675 & 0.097 \\
      & 2 &     0.095 & 0.096 & 0.098 & 0.098 &     6.12 &  1.91 & 0.548 & 0.302 &   $\infty$ & 0.197 & 0.076 & 0.053 \\
      & 3 &     0.097 & 0.097 & 0.099 & 0.099 &     1.47 &  1.58 & 0.345 &  0.34 &   $\infty$ &   $\infty$ & 0.021 & 0.022 \\
      & 4 &     0.098 & 0.098 &   0.1 &   0.1 &     0.63 & 0.557 & 0.233 & 0.229 &   $\infty$ &   $\infty$ &  0.01 & 0.009 \\
\bottomrule
\end{tabular}

\section*{Diffusion of a contagious diseas, degree = $3$}\\

\begin{tabular}{llrrrr|rrrr|rrrr}
\toprule
      & {} & \multicolumn{4}{l}{training error} & \multicolumn{4}{l}{test error (vector field)} & \multicolumn{4}{l}{test error (trajectories)} \\
      & \# side information: &         0 &     1 &     2 &     3 &        0 &        1 &        2 &     3 &    0 &    1 &     2 &     3 \\
noise & \# trajectories &           &       &       &       &          &          &          &       &      &      &       &       \\
\midrule
\multirow{4}{*}{0.001} & 1 &         0 &     0 & 0.001 & 0.001 & 3.08e+07 & 3.13e+06 &  3.2e+04 & 0.638 &  $\infty$ &  $\infty$ &   $\infty$ & 0.036 \\
      & 2 &     0.001 & 0.001 & 0.001 & 0.001 &     36.2 &     54.6 &    0.403 & 0.292 &  $\infty$ &  $\infty$ & 0.025 & 0.014 \\
      & 3 &     0.001 & 0.001 & 0.001 & 0.001 &     2.37 &     3.04 &    0.297 &  0.16 &  $\infty$ &  $\infty$ & 0.016 & 0.007 \\
      & 4 &     0.001 & 0.001 & 0.001 & 0.001 &    0.693 &    0.489 &    0.171 & 0.095 &  $\infty$ & 0.02 & 0.002 & 0.002 \\
\cline{1-14}
\multirow{4}{*}{0.010} & 1 &         0 & 0.002 & 0.008 & 0.009 & 3.08e+08 & 3.12e+07 & 3.14e+05 &  7.55 &  $\infty$ &  $\infty$ &   $\infty$ &  0.37 \\
      & 2 &     0.009 & 0.009 & 0.009 &  0.01 &      362 &      546 &     1.61 & 0.544 &  $\infty$ &  $\infty$ & 0.106 & 0.046 \\
      & 3 &     0.009 & 0.009 &  0.01 &  0.01 &     23.7 &     30.4 &    0.698 & 0.206 &  $\infty$ &  $\infty$ & 0.046 & 0.018 \\
      & 4 &      0.01 &  0.01 &  0.01 &  0.01 &     6.93 &     4.89 &    0.168 & 0.097 &  $\infty$ &  $\infty$ & 0.006 & 0.004 \\
\cline{1-14}
\multirow{4}{*}{0.100} & 1 &         0 & 0.024 & 0.077 & 0.093 & 3.08e+09 & 3.12e+08 & 2.48e+06 &  80.4 &  $\infty$ &  $\infty$ &   $\infty$ &  3.73 \\
      & 2 &     0.085 & 0.087 & 0.095 & 0.097 & 3.62e+03 & 5.46e+03 &     14.2 &  3.53 &  $\infty$ &  $\infty$ & 0.878 & 0.321 \\
      & 3 &     0.093 & 0.093 & 0.097 & 0.098 &      237 &      304 &     5.18 &  0.56 &  $\infty$ &  $\infty$ & 0.348 & 0.042 \\
      & 4 &     0.096 & 0.096 & 0.099 & 0.099 &     69.3 &     48.9 &     1.25 &  1.13 &  $\infty$ &  $\infty$ & 0.018 & 0.014 \\
\bottomrule
\end{tabular}

\section*{Diffusion of a contagious diseas, degree = $4$}\\

\begin{tabular}{llrrrr|rrrr|rrrr}
\toprule
      & {} & \multicolumn{4}{l}{training error} & \multicolumn{4}{l}{test error (vector field)} & \multicolumn{4}{l}{test error (trajectories)} \\
      & \# side information: &         0 &     1 &     2 &     3 &        0 &        1 &        2 &     3 &    0 &   1 &     2 &     3 \\
noise & \# trajectories &           &       &       &       &          &          &          &       &      &     &       &       \\
\midrule
\multirow{4}{*}{0.001} & 1 &     0.001 & 0.001 & 0.001 & 0.001 & 4.85e+03 & 4.57e+03 & 4.66e+03 &  4.56 &  $\infty$ & $\infty$ &   $\infty$ & 0.112 \\
      & 2 &     0.001 & 0.001 & 0.001 & 0.001 & 1.32e+03 & 1.39e+04 &     82.1 &  2.55 &  $\infty$ & $\infty$ &  1.97 & 0.041 \\
      & 3 &     0.001 & 0.001 & 0.001 & 0.001 & 1.56e+03 & 1.38e+03 &     3.31 &  1.58 &  $\infty$ & $\infty$ & 0.091 & 0.022 \\
      & 4 &     0.001 & 0.001 & 0.001 & 0.001 &     29.2 &     20.2 &        3 & 0.254 &  $\infty$ & $\infty$ & 0.018 & 0.001 \\
\cline{1-14}
\multirow{4}{*}{0.010} & 1 &     0.006 & 0.006 & 0.007 & 0.009 &    4e+04 & 4.44e+04 & 4.34e+04 &  56.8 &  $\infty$ & $\infty$ &   $\infty$ & 0.796 \\
      & 2 &     0.008 & 0.007 & 0.008 & 0.009 & 1.32e+04 & 1.39e+05 &      751 &  12.1 &  $\infty$ & $\infty$ &  18.1 & 0.295 \\
      & 3 &     0.009 & 0.009 & 0.009 & 0.009 & 1.56e+04 & 1.38e+04 &     20.8 &  7.05 &  $\infty$ & $\infty$ & 0.175 & 0.127 \\
      & 4 &     0.009 & 0.009 &  0.01 &  0.01 &      292 &      202 &     4.67 & 0.704 &  $\infty$ & $\infty$ & 0.017 & 0.004 \\
\cline{1-14}
\multirow{4}{*}{0.100} & 1 &     0.057 & 0.057 & 0.065 & 0.091 & 3.44e+05 & 3.12e+05 & 4.69e+05 &   574 &  $\infty$ & $\infty$ &   $\infty$ &  7.67 \\
      & 2 &     0.076 & 0.067 & 0.082 & 0.095 & 1.32e+05 & 1.39e+06 & 7.35e+03 &  51.6 &  $\infty$ & $\infty$ &   $\infty$ &  2.03 \\
      & 3 &     0.085 & 0.087 & 0.094 & 0.096 & 1.56e+05 & 1.38e+05 &      205 &  40.5 &  $\infty$ & $\infty$ &  1.46 &  1.22 \\
      & 4 &     0.093 & 0.093 & 0.098 & 0.098 & 2.92e+03 & 2.02e+03 &     16.1 &  6.19 &  $\infty$ & $\infty$ & 0.068 & 0.019 \\
\bottomrule
\end{tabular}



==> Learning with Side Info r1 -arxiv submission jan 17 2022 compressed/data/tables/disease_20_samples.tex <==

\section*{Diffusion of a contagious diseas, degree = $2$}\\

\begin{tabular}{llrrrr|rrrr|rrrr}
\toprule
      & {} & \multicolumn{4}{l}{training error} & \multicolumn{4}{l}{test error (vector field)} & \multicolumn{4}{l}{test error (trajectories)} \\
      & \# side information: &         0 &     1 &     2 &     3 &        0 &     1 &     2 &     3 &     0 &     1 &     2 &     3 \\
noise & \# trajectories &           &       &       &       &          &       &       &       &       &       &       &       \\
\midrule
\multirow{3}{*}{0.001} & 1 &     0.001 & 0.001 & 0.001 & 0.001 &      189 &  1.42 & 0.432 & 0.068 &   $\infty$ &   $\infty$ & 0.045 & 0.008 \\
      & 2 &     0.001 & 0.001 & 0.002 & 0.002 &    0.044 & 0.023 & 0.081 & 0.081 & 0.004 & 0.002 & 0.005 & 0.005 \\
      & 3 &     0.001 & 0.001 & 0.002 & 0.002 &    0.018 & 0.018 & 0.083 & 0.083 & 0.002 & 0.002 & 0.005 & 0.005 \\
\cline{1-14}
\multirow{3}{*}{0.010} & 1 &     0.008 & 0.008 & 0.008 & 0.009 & 1.89e+03 &  14.2 &   1.3 & 0.071 &   $\infty$ &   $\infty$ & 0.129 & 0.012 \\
      & 2 &     0.008 & 0.008 & 0.009 & 0.009 &    0.444 & 0.233 & 0.062 & 0.061 & 0.031 &   $\infty$ & 0.006 & 0.004 \\
      & 3 &     0.009 & 0.009 & 0.009 & 0.009 &    0.179 &  0.18 & 0.075 & 0.074 &   $\infty$ &   $\infty$ & 0.007 & 0.006 \\
\cline{1-14}
\multirow{3}{*}{0.100} & 1 &      0.08 & 0.082 & 0.085 & 0.087 & 1.89e+04 &   142 &  8.08 & 0.075 &   $\infty$ &   $\infty$ & 0.665 &  0.02 \\
      & 2 &     0.085 & 0.085 & 0.087 & 0.088 &     4.44 &  2.33 & 0.077 & 0.068 &   $\infty$ &   $\infty$ & 0.021 & 0.019 \\
      & 3 &     0.086 & 0.086 & 0.088 & 0.088 &     1.78 &   1.8 & 0.088 &  0.11 &   $\infty$ &   $\infty$ & 0.019 & 0.016 \\
\bottomrule
\end{tabular}

\section*{Diffusion of a contagious diseas, degree = $3$}\\

\begin{tabular}{llrrrr|rrrr|rrrr}
\toprule
      & {} & \multicolumn{4}{l}{training error} & \multicolumn{4}{l}{test error (vector field)} & \multicolumn{4}{l}{test error (trajectories)} \\
      & \# side information: &         0 &     1 &     2 &     3 &        0 &        1 &        2 &     3 &    0 &     1 &     2 &     3 \\
noise & \# trajectories &           &       &       &       &          &          &          &       &      &       &       &       \\
\midrule
\multirow{3}{*}{0.001} & 1 &     0.001 & 0.001 & 0.001 & 0.001 &      229 &      363 &      497 &  4.22 &  $\infty$ &   $\infty$ &  12.3 & 0.065 \\
      & 2 &     0.001 & 0.001 & 0.001 & 0.001 &     21.8 &     22.2 &    0.221 & 0.248 &  $\infty$ &   $\infty$ &  0.01 & 0.005 \\
      & 3 &     0.001 & 0.001 & 0.001 & 0.001 &     1.65 &     2.15 &    0.141 & 0.151 &  $\infty$ & 0.026 & 0.003 & 0.004 \\
\cline{1-14}
\multirow{3}{*}{0.010} & 1 &     0.008 & 0.008 & 0.008 & 0.008 & 2.29e+03 & 3.63e+03 & 4.86e+03 &  43.4 &  $\infty$ &   $\infty$ &   $\infty$ & 0.581 \\
      & 2 &     0.008 & 0.008 & 0.008 & 0.009 &      218 &      222 &     1.92 &  0.47 &  $\infty$ &   $\infty$ & 0.081 & 0.013 \\
      & 3 &     0.008 & 0.008 & 0.009 & 0.009 &     16.5 &     21.5 &     0.47 & 0.292 &  $\infty$ & 0.251 & 0.008 & 0.007 \\
\cline{1-14}
\multirow{3}{*}{0.100} & 1 &     0.079 & 0.079 &  0.08 & 0.084 & 2.29e+04 & 3.63e+04 &  4.2e+04 &   435 &  $\infty$ &   $\infty$ &   $\infty$ &   5.8 \\
      & 2 &     0.082 & 0.083 & 0.085 & 0.087 & 2.18e+03 & 2.22e+03 &     15.9 &  2.64 &  $\infty$ &   $\infty$ & 0.662 & 0.079 \\
      & 3 &     0.084 & 0.084 & 0.086 & 0.087 &      165 &      215 &     3.12 & 0.982 &  $\infty$ &   $\infty$ & 0.052 & 0.023 \\
\bottomrule
\end{tabular}

\section*{Diffusion of a contagious diseas, degree = $4$}\\

\begin{tabular}{llrrrr|rrrr|rrrr}
\toprule
      & {} & \multicolumn{4}{l}{training error} & \multicolumn{4}{l}{test error (vector field)} & \multicolumn{4}{l}{test error (trajectories)} \\
      & \# side information: &         0 &     1 &     2 &     3 &        0 &        1 &        2 &        3 &    0 &   1 &     2 &     3 \\
noise & \# trajectories &           &       &       &       &          &          &          &          &      &     &       &       \\
\midrule
\multirow{3}{*}{0.001} & 1 &     0.001 & 0.001 & 0.001 & 0.001 & 1.63e+04 &      831 &      232 &     21.7 &  $\infty$ & $\infty$ &  14.6 & 0.092 \\
      & 2 &     0.001 & 0.001 & 0.001 & 0.001 & 2.58e+03 &      407 &     39.7 &    0.726 &  $\infty$ & $\infty$ & 0.097 & 0.004 \\
      & 3 &     0.001 & 0.001 & 0.001 & 0.001 &      421 &      393 &     15.2 &    0.575 &  $\infty$ & $\infty$ & 0.107 & 0.002 \\
\cline{1-14}
\multirow{3}{*}{0.010} & 1 &     0.008 & 0.008 & 0.008 & 0.008 & 1.62e+05 & 8.31e+03 &  1.6e+03 &      191 &  $\infty$ & $\infty$ &   $\infty$ & 0.822 \\
      & 2 &     0.008 & 0.008 & 0.008 & 0.009 & 2.58e+04 & 4.07e+03 &      300 &     1.83 &  $\infty$ & $\infty$ &  1.12 & 0.046 \\
      & 3 &     0.008 & 0.008 & 0.008 & 0.009 & 4.21e+03 & 3.93e+03 &      162 &     1.53 &  $\infty$ & $\infty$ & 0.792 & 0.031 \\
\cline{1-14}
\multirow{3}{*}{0.100} & 1 &     0.076 & 0.075 &  0.08 & 0.083 & 1.57e+06 & 8.31e+04 & 1.63e+04 & 1.92e+03 &  $\infty$ & $\infty$ &   $\infty$ &  8.22 \\
      & 2 &     0.079 & 0.079 & 0.082 & 0.087 & 2.58e+05 & 4.07e+04 & 2.91e+03 &     8.01 &  $\infty$ & $\infty$ &  11.9 & 0.018 \\
      & 3 &     0.081 & 0.082 & 0.084 & 0.087 & 4.21e+04 & 3.93e+04 & 1.77e+03 &     7.99 &  $\infty$ & $\infty$ &  6.31 & 0.017 \\
\bottomrule
\end{tabular}


==> Learning with Side Info r1 -arxiv submission jan 17 2022 compressed/data/tables/lorenz.tex <==

\section*{Lorenz, degree = $2$}\\
\begin{tabular}{ll|rr|rr|rr}
\toprule
      & {} & \multicolumn{2}{l}{training error} & \multicolumn{2}{l}{test error (vector field)} & \multicolumn{2}{l}{test error (trajectories)} \\
      & side information used? $\rightarrow$ &         no &     yes &        no &     yes &     no &     yes \\
noise & \# trajectories $\downarrow$ &           &       &          &       &       &       \\
\midrule
\multirow{3}{*}{0.001} & 1 &     0.001 & 0.001 & 0.049 & 0.001 & 0.028 & 0.002 \\
      & 2 &     0.001 & 0.001 & 0.002 & 0.001 & 0.002 & 0.001 \\
      & 3 &     0.001 & 0.001 & 0.002 & 0.001 & 0.003 & 0.001 \\
\cline{1-8}
\multirow{3}{*}{0.010} & 1 &     0.007 & 0.008 & 0.491 & 0.009 & 0.285 & 0.018 \\
      & 2 &     0.008 & 0.009 &  0.02 & 0.007 & 0.018 & 0.008 \\
      & 3 &     0.008 & 0.009 & 0.018 & 0.007 & 0.025 & 0.005 \\
\cline{1-8}
\multirow{3}{*}{0.100} & 1 &     0.068 & 0.083 &  4.91 &  0.09 &  3.01 &  0.17 \\
      & 2 &     0.079 & 0.086 & 0.202 & 0.074 & 0.185 & 0.064 \\
      & 3 &     0.083 & 0.088 & 0.185 & 0.071 & 0.251 & 0.052 \\
\bottomrule
\end{tabular}

\section*{Lorenz, degree = $3$}\\
\begin{tabular}{ll|rr|rr|rr}
\toprule
      & {} & \multicolumn{2}{l}{training error} & \multicolumn{2}{l}{test error (vector field)} & \multicolumn{2}{l}{test error (trajectories)} \\
      & side information used? $\rightarrow$ &         no &     yes &        no &     yes &     no &     yes \\
noise & \# trajectories $\downarrow$ &           &       &          &       &       &       \\
\midrule
\multirow{3}{*}{0.001} & 1 &         0 &     0 &      110 &  10.9 &   $\infty$ &  13.7 \\
      & 2 &     0.001 & 0.001 &    0.046 & 0.008 & 0.016 & 0.005 \\
      & 3 &     0.001 & 0.001 &    0.014 & 0.044 & 0.006 & 0.034 \\
\cline{1-8}
\multirow{3}{*}{0.010} & 1 &     0.003 & 0.005 &      192 &  10.9 &  57.9 &  14.2 \\
      & 2 &     0.006 & 0.007 &    0.461 & 0.063 & 0.157 &  0.05 \\
      & 3 &     0.008 & 0.008 &    0.138 & 0.035 & 0.058 & 0.019 \\
\cline{1-8}
\multirow{3}{*}{0.100} & 1 &     0.032 & 0.057 & 1.47e+03 &  54.9 &   237 &  23.6 \\
      & 2 &     0.064 & 0.071 &     4.61 & 0.963 &  1.59 & 0.461 \\
      & 3 &     0.075 & 0.078 &     1.38 & 0.352 & 0.576 & 0.279 \\
\bottomrule
\end{tabular}
\newpage
\section*{Lorenz, degree = $4$}\\
\begin{tabular}{ll|rr|rr|rr}
\toprule
      & {} & \multicolumn{2}{l}{training error} & \multicolumn{2}{l}{test error (vector field)} & \multicolumn{2}{l}{test error (trajectories)} \\
      & side information used? $\rightarrow$ &         no &     yes &        no &     yes &     no &     yes \\
noise & \# trajectories $\downarrow$ &           &       &          &       &       &       \\
\midrule
\multirow{3}{*}{0.001} & 1 &         0 &     0 &      167 &      532 &  82.7 &  94.4 \\
      & 2 &         0 &     0 &     46.1 &    0.479 &  51.8 & 0.832 \\
      & 3 &     0.001 &     0 &    0.283 &    0.205 & 0.047 & 0.421 \\
\cline{1-8}
\multirow{3}{*}{0.010} & 1 &         0 & 0.001 &      858 & 6.22e+03 &   $\infty$ &   286 \\
      & 2 &     0.003 & 0.004 &      461 &     1.71 &   $\infty$ &  1.97 \\
      & 3 &     0.006 & 0.005 &     2.83 &    0.407 & 0.468 & 0.179 \\
\cline{1-8}
\multirow{3}{*}{0.100} & 1 &         0 & 0.031 & 8.92e+03 & 2.55e+03 &   $\infty$ &   120 \\
      & 2 &     0.028 & 0.057 & 4.61e+03 &     6.21 &   $\infty$ &  5.15 \\
      & 3 &     0.061 & 0.069 &     28.3 &     2.47 &  4.84 & 0.939 \\
\bottomrule
\end{tabular}


==> Learning with Side Info r1 -arxiv submission jan 17 2022 compressed/data/tables/lorenz_10_samples.tex <==

\section*{Lorentz, degree = $2$}\\

\begin{tabular}{llrrrr|rrrr|rrrr}
\toprule
      & {} & \multicolumn{4}{l}{training error} & \multicolumn{4}{l}{test error (vector field)} & \multicolumn{4}{l}{test error (trajectories)} \\
      & \# side information: &         0 &     1 &     2 &     3 &     0 &     1 &     2 &     3 &     0 &     1 &     2 &     3 \\
noise & \# trajectories &           &       &       &       &       &       &       &       &       &       &       &       \\
\midrule
\multirow{4}{*}{0.001} & 1 &        -0 &     0 &     0 & 0.001 &  0.49 & 0.208 &  0.17 & 0.003 &  1.04 & 0.235 & 0.134 & 0.003 \\
      & 2 &     0.001 & 0.001 & 0.001 & 0.001 & 0.003 & 0.002 & 0.002 & 0.001 & 0.005 & 0.005 & 0.004 & 0.003 \\
      & 3 &     0.001 & 0.001 & 0.001 & 0.001 & 0.002 & 0.001 & 0.002 & 0.001 & 0.004 & 0.003 & 0.003 & 0.003 \\
      & 4 &     0.001 & 0.001 & 0.001 & 0.001 & 0.001 & 0.001 & 0.001 & 0.001 & 0.003 & 0.002 & 0.002 & 0.002 \\
\cline{1-14}
\multirow{4}{*}{0.010} & 1 &        -0 & 0.003 & 0.004 & 0.007 &   4.9 &  2.08 &   1.7 & 0.027 &   9.8 &  2.31 &  1.33 & 0.033 \\
      & 2 &     0.007 & 0.007 & 0.007 & 0.008 &  0.03 & 0.024 & 0.021 & 0.011 & 0.053 & 0.049 & 0.047 & 0.025 \\
      & 3 &     0.007 & 0.007 & 0.007 & 0.008 & 0.024 & 0.013 & 0.015 & 0.006 & 0.041 &  0.03 & 0.027 & 0.027 \\
      & 4 &     0.007 & 0.007 & 0.007 & 0.008 & 0.011 & 0.008 & 0.008 & 0.006 & 0.027 & 0.025 & 0.023 & 0.023 \\
\cline{1-14}
\multirow{4}{*}{0.100} & 1 &        -0 & 0.026 & 0.043 & 0.074 &    49 &  20.8 &    17 & 0.267 &  55.8 &  19.9 &  13.4 & 0.331 \\
      & 2 &     0.066 & 0.068 & 0.071 & 0.078 & 0.297 &  0.24 & 0.214 & 0.109 & 0.533 & 0.487 & 0.466 & 0.243 \\
      & 3 &     0.071 & 0.073 & 0.074 & 0.079 & 0.237 & 0.128 & 0.158 & 0.065 & 0.412 & 0.302 & 0.273 & 0.271 \\
      & 4 &     0.071 & 0.072 & 0.074 & 0.079 & 0.113 & 0.082 & 0.076 & 0.064 & 0.274 & 0.247 &  0.23 & 0.212 \\
\bottomrule
\end{tabular}

\section*{Lorentz, degree = $3$}\\

\begin{tabular}{llrrrr|rrrr|rrrr}
\toprule
      & {} & \multicolumn{4}{l}{training error} & \multicolumn{4}{l}{test error (vector field)} & \multicolumn{4}{l}{test error (trajectories)} \\
      & \# side information: &         0 &     1 &     2 &     3 &     0 &     1 &     2 &        3 &     0 &     1 &     2 &     3 \\
noise & \# trajectories &           &       &       &       &       &       &       &          &       &       &       &       \\
\midrule
\multirow{4}{*}{0.001} & 1 &         0 &     0 &     0 &     0 &   165 &   165 &   157 &      267 &   $\infty$ &   $\infty$ &   $\infty$ &   $\infty$ \\
      & 2 &         0 &     0 &     0 &     0 &  3.64 &  3.17 &  30.4 &    0.076 &  1.34 & 0.758 &  5.57 & 0.022 \\
      & 3 &     0.001 & 0.001 &     0 &     0 &  0.25 & 0.157 & 0.851 &    0.019 & 0.058 & 0.026 & 0.219 & 0.022 \\
      & 4 &     0.001 & 0.001 & 0.001 & 0.001 &  0.01 & 0.006 &  0.03 &    0.009 & 0.004 & 0.003 & 0.018 & 0.005 \\
\cline{1-14}
\multirow{4}{*}{0.010} & 1 &         0 &     0 & 0.003 & 0.003 &   166 &   166 &   158 & 1.09e+03 &   $\infty$ &   $\infty$ &   $\infty$ &   $\infty$ \\
      & 2 &         0 & 0.003 & 0.004 & 0.005 &  37.7 &  31.4 &  34.6 &    0.521 &  10.7 &  8.51 &  7.79 & 0.402 \\
      & 3 &     0.006 & 0.006 & 0.006 & 0.006 &   2.5 &  1.57 &  1.46 &    0.049 & 0.577 & 0.258 & 0.242 &  0.07 \\
      & 4 &     0.006 & 0.006 & 0.007 & 0.007 & 0.098 & 0.065 &  0.04 &     0.03 & 0.042 &  0.03 & 0.034 & 0.034 \\
\cline{1-14}
\multirow{4}{*}{0.100} & 1 &         0 &     0 & 0.039 & 0.038 &   168 &   168 &   160 &      668 &   $\infty$ &   $\infty$ &   $\infty$ &   $\infty$ \\
      & 2 &         0 & 0.035 & 0.046 & 0.058 &   375 &   312 &   338 &     9.38 &   $\infty$ &   $\infty$ &   $\infty$ &  8.25 \\
      & 3 &      0.06 & 0.062 & 0.066 & 0.069 &    25 &  15.7 &    15 &    0.542 &  5.49 &  2.61 &  2.71 & 0.616 \\
      & 4 &     0.064 & 0.065 & 0.068 & 0.069 & 0.985 & 0.648 &  0.37 &    0.234 & 0.419 & 0.306 & 0.349 & 0.313 \\
\bottomrule
\end{tabular}

\section*{Lorentz, degree = $4$}\\

\begin{tabular}{llrrrr|rrrr|rrrr}
\toprule
      & {} & \multicolumn{4}{l}{training error} & \multicolumn{4}{l}{test error (vector field)} & \multicolumn{4}{l}{test error (trajectories)} \\
      & \# side information: &         0 &     1 &     2 &     3 &        0 &        1 &        2 &       3 &     0 &    1 &   2 &     3 \\
noise & \# trajectories &           &       &       &       &          &          &          &         &       &      &     &       \\
\midrule
\multirow{4}{*}{0.001} & 1 &         0 &     0 &     0 &     0 &      118 &      118 &      108 & 1.1e+03 &   $\infty$ &  $\infty$ & $\infty$ &   134 \\
      & 2 &         0 &     0 &     0 &     0 &      579 &      580 &      570 &    98.8 &   $\infty$ &  $\infty$ & $\infty$ &  25.3 \\
      & 3 &         0 &     0 &     0 &     0 &      934 &      919 & 9.81e+03 &    0.95 &   $\infty$ &  140 & $\infty$ & 0.389 \\
      & 4 &         0 &     0 &     0 &     0 &     9.23 &     8.32 & 1.91e+03 &   0.094 & 0.968 & 1.03 & $\infty$ & 0.236 \\
\cline{1-14}
\multirow{4}{*}{0.010} & 1 &         0 &     0 &     0 &     0 &      118 &      118 &      108 &     587 &   $\infty$ &  $\infty$ & $\infty$ &   109 \\
      & 2 &         0 &     0 &     0 &     0 &      576 &      577 &      567 &     214 &   $\infty$ &  $\infty$ & $\infty$ &  46.3 \\
      & 3 &         0 &     0 & 0.002 & 0.002 &      972 &      948 &  2.7e+03 &    2.17 &   $\infty$ &  $\infty$ & 243 &  1.35 \\
      & 4 &     0.004 & 0.004 & 0.001 & 0.004 &     92.3 &     83.2 & 1.66e+03 &   0.657 &   $\infty$ &  $\infty$ & $\infty$ & 0.378 \\
\cline{1-14}
\multirow{4}{*}{0.100} & 1 &         0 &     0 &     0 &     0 &      118 &      118 &      111 &     966 &   $\infty$ &  $\infty$ & $\infty$ &   126 \\
      & 2 &         0 &     0 & 0.008 & 0.037 &      554 &      555 &      544 &     152 &   177 &  177 & 168 &  28.2 \\
      & 3 &         0 &     0 &  0.03 &  0.05 & 1.29e+03 & 1.27e+03 & 1.81e+03 &    17.9 &   $\infty$ &  $\infty$ & 200 &  3.46 \\
      & 4 &     0.039 &  0.04 & 0.035 & 0.054 &      923 &      832 & 8.92e+03 &    2.84 &   $\infty$ &  $\infty$ & $\infty$ &  1.07 \\
\bottomrule
\end{tabular}


==> Learning with Side Info r1 -arxiv submission jan 17 2022 compressed/data/tables/lorenz_20_samples.tex <==

\section*{Lorentz, degree = $2$}\\

\begin{tabular}{llrrrr|rrrr|rrrr}
\toprule
      & {} & \multicolumn{4}{l}{training error} & \multicolumn{4}{l}{test error (vector field)} & \multicolumn{4}{l}{test error (trajectories)} \\
      & \# side information: &         0 &     1 &     2 &     3 &     0 &     1 &     2 &     3 &     0 &     1 &     2 &     3 \\
noise & \# trajectories &           &       &       &       &       &       &       &       &       &       &       &       \\
\midrule
\multirow{3}{*}{0.001} & 1 &     0.001 & 0.001 & 0.001 & 0.001 & 0.049 & 0.003 & 0.003 & 0.001 & 0.028 & 0.003 & 0.002 & 0.002 \\
      & 2 &     0.001 & 0.001 & 0.001 & 0.001 & 0.002 & 0.002 & 0.002 & 0.001 & 0.002 & 0.002 & 0.001 & 0.001 \\
      & 3 &     0.001 & 0.001 & 0.001 & 0.001 & 0.002 & 0.001 & 0.001 & 0.001 & 0.003 & 0.002 & 0.002 & 0.001 \\
\cline{1-14}
\multirow{3}{*}{0.010} & 1 &     0.007 & 0.007 & 0.008 & 0.008 & 0.491 &  0.03 & 0.029 & 0.009 & 0.285 & 0.033 & 0.028 & 0.018 \\
      & 2 &     0.008 & 0.008 & 0.008 & 0.009 &  0.02 & 0.018 & 0.018 & 0.007 & 0.018 & 0.019 & 0.016 & 0.008 \\
      & 3 &     0.008 & 0.008 & 0.008 & 0.009 & 0.018 & 0.014 & 0.013 & 0.007 & 0.025 & 0.018 & 0.019 & 0.005 \\
\cline{1-14}
\multirow{3}{*}{0.100} & 1 &     0.068 & 0.073 & 0.077 & 0.083 &  4.91 & 0.304 &  0.28 &  0.09 &  3.01 &  0.33 & 0.263 &  0.17 \\
      & 2 &     0.079 & 0.079 & 0.081 & 0.086 & 0.202 & 0.177 & 0.172 & 0.074 & 0.185 & 0.187 & 0.154 & 0.064 \\
      & 3 &     0.083 & 0.084 & 0.085 & 0.088 & 0.185 & 0.142 & 0.135 & 0.071 & 0.251 & 0.184 & 0.194 & 0.052 \\
\bottomrule
\end{tabular}

\section*{Lorentz, degree = $3$}\\

\begin{tabular}{llrrrr|rrrr|rrrr}
\toprule
      & {} & \multicolumn{4}{l}{training error} & \multicolumn{4}{l}{test error (vector field)} & \multicolumn{4}{l}{test error (trajectories)} \\
      & \# side information: &         0 &     1 &     2 &     3 &        0 &     1 &     2 &     3 &     0 &     1 &     2 &     3 \\
noise & \# trajectories &           &       &       &       &          &       &       &       &       &       &       &       \\
\midrule
\multirow{3}{*}{0.001} & 1 &         0 &     0 & 0.001 &     0 &      110 &   207 &    66 &  10.9 &   $\infty$ &   $\infty$ &   $\infty$ &  13.7 \\
      & 2 &     0.001 & 0.001 & 0.001 & 0.001 &    0.046 & 0.025 & 0.043 & 0.008 & 0.016 & 0.008 & 0.033 & 0.005 \\
      & 3 &     0.001 & 0.001 & 0.001 & 0.001 &    0.014 & 0.009 & 0.037 & 0.044 & 0.006 & 0.008 & 0.022 & 0.034 \\
\cline{1-14}
\multirow{3}{*}{0.010} & 1 &     0.003 & 0.003 & 0.005 & 0.005 &      192 &   187 &   226 &  10.9 &  57.9 &  61.6 &   $\infty$ &  14.2 \\
      & 2 &     0.006 & 0.006 & 0.007 & 0.007 &    0.461 & 0.251 & 0.256 & 0.063 & 0.157 & 0.084 & 0.164 &  0.05 \\
      & 3 &     0.008 & 0.008 & 0.008 & 0.008 &    0.138 & 0.094 & 0.133 & 0.035 & 0.058 & 0.076 & 0.062 & 0.019 \\
\cline{1-14}
\multirow{3}{*}{0.100} & 1 &     0.032 & 0.033 &  0.05 & 0.057 & 1.47e+03 &   516 &   664 &  54.9 &   237 &   $\infty$ &   $\infty$ &  23.6 \\
      & 2 &     0.064 & 0.065 & 0.068 & 0.071 &     4.61 &  2.51 &  2.25 & 0.963 &  1.59 & 0.899 &  1.46 & 0.461 \\
      & 3 &     0.075 & 0.076 & 0.078 & 0.078 &     1.38 & 0.943 & 0.787 & 0.352 & 0.576 &  0.77 & 0.525 & 0.279 \\
\bottomrule
\end{tabular}

\section*{Lorentz, degree = $4$}\\

\begin{tabular}{llrrrr|rrrr|rrrr}
\toprule
      & {} & \multicolumn{4}{l}{training error} & \multicolumn{4}{l}{test error (vector field)} & \multicolumn{4}{l}{test error (trajectories)} \\
      & \# side information: &         0 &     1 &     2 &     3 &        0 &        1 &        2 &        3 &     0 &     1 &    2 &     3 \\
noise & \# trajectories &           &       &       &       &          &          &          &          &       &       &      &       \\
\midrule
\multirow{3}{*}{0.001} & 1 &         0 &     0 &     0 &     0 &      167 &      243 & 9.29e+03 &      532 &  82.7 &   $\infty$ &  $\infty$ &  94.4 \\
      & 2 &         0 &     0 &     0 &     0 &     46.1 &       11 &      768 &    0.479 &  51.8 &  8.13 &  $\infty$ & 0.832 \\
      & 3 &     0.001 & 0.001 &     0 &     0 &    0.283 &    0.199 &     84.6 &    0.205 & 0.047 & 0.048 & 11.1 & 0.421 \\
\cline{1-14}
\multirow{3}{*}{0.010} & 1 &         0 &     0 &     0 & 0.001 &      858 & 1.08e+03 & 4.66e+04 & 6.22e+03 &   $\infty$ &   $\infty$ &  $\infty$ &   286 \\
      & 2 &     0.003 & 0.004 &     0 & 0.004 &      461 &      110 & 1.47e+03 &     1.71 &   $\infty$ &  48.4 &  $\infty$ &  1.97 \\
      & 3 &     0.006 & 0.006 & 0.002 & 0.005 &     2.83 &     1.99 &     99.5 &    0.407 & 0.468 & 0.486 &  $\infty$ & 0.179 \\
\cline{1-14}
\multirow{3}{*}{0.100} & 1 &         0 &     0 & 0.009 & 0.031 & 8.92e+03 & 8.93e+03 & 1.55e+05 & 2.55e+03 &   $\infty$ &   $\infty$ &  $\infty$ &   120 \\
      & 2 &     0.028 & 0.038 & 0.041 & 0.057 & 4.61e+03 &  1.1e+03 & 4.54e+03 &     6.21 &   $\infty$ &   $\infty$ &  $\infty$ &  5.15 \\
      & 3 &     0.061 & 0.062 & 0.053 & 0.069 &     28.3 &     19.9 &     87.1 &     2.47 &  4.84 &  4.93 &  $\infty$ & 0.939 \\
\bottomrule
\end{tabular}


==> Learning with Side Info r1 -arxiv submission jan 17 2022 compressed/header.tex <==
%\usepackage[most]{tcolorbox}
% \usepackage{algorithmic}

\usepackage{makecell}
\usepackage{amsfonts}
%\usepackage[inline]{enumitem}
\usepackage{amsmath}
\usepackage{amsopn}
\usepackage{amssymb}  %
\usepackage{array}
\usepackage{bold-extra}
\usepackage{braket}
\usepackage{calligra}
\usepackage{epstopdf}
\usepackage{float}
\usepackage{graphicx,epstopdf}
\usepackage{graphicx}
\usepackage{hyperref}
\usepackage{lipsum}
\usepackage{mathrsfs}
\usepackage{mathtools}
\usepackage{pgfplotstable}
\usepackage{pgfplots}
\usepackage{pgfplots}
\usepackage{pifont}
\usepackage{subcaption}
\usepackage{tikz}
\usepackage{wrapfig}
\usepackage{xspace}
%\usepackage[noabbrev,capitalise]{cleveref}

\usepackage{paralist}

\usepackage{times}
\usepackage{multirow}


\usepackage{amsmath}
\usepackage{amssymb}
%\usepackage{natbib}
\usepackage{graphicx}
\usepackage{url}
%\usepackage{algorithm2e}
\usepackage{booktabs}
% space savings
\makeatletter
\g@addto@macro\normalsize{%
  \setlength\abovedisplayskip{3pt}
  \setlength\belowdisplayskip{3pt}
  \setlength\abovedisplayshortskip{3pt}
  \setlength\belowdisplayshortskip{3pt}
}
\makeatother

%\renewcommand{\baselinestretch}{1}
% \usepackage{microtype}
%\usepackage[activate={true,nocompatibility},final,tracking=true,kerning=true,spacing=true,factor=1100,stretch=20,shrink=20]{microtype}
% activate={true,nocompatibility} - activate protrusion and expansion
% final - enable microtype; use "draft" to disable
% tracking=true, kerning=true, spacing=true - activate these techniques
% factor=1100 - add 10% to the protrusion amount (default is 1000)
% stretch=10, shrink=10 - reduce stretchability/shrinkability (default
% is 20/20)


% \edef\tmp{\pgfmathresult}
% \pgfkeys{/pgf/fpu=false}
% \pgfkeys{/pgf/fpu}
% \pgfmathparse{16383+1}
% \pgfplotsset{compat=1.12}
% \pgfplotstableset{col sep=comma}
% \tikzexternalize[prefix=cached_figures/, mode=list and make]
\usetikzlibrary{arrows.meta}
\usetikzlibrary{calc,patterns,angles,quotes}
\usetikzlibrary{external}
\usetikzlibrary{pgfplots.groupplots}
\colorlet{texcscolor}{blue!50!black}
\colorlet{texemcolor}{red!70!black}
\colorlet{texpreamble}{red!70!black}
\colorlet{codebackground}{black!25!white!25}



%%%% custom macros

\newcommand{\x}{x}
\newcommand{\ix}{x}
\newcommand{\iy}{{y}}
\newcommand{\ip}{{p}}
\newcommand{\iq}{{q}}
\newcommand{\R}{\mathbb R}
\newcommand{\Z}{\mathbb Z}
\newcommand{\originalvf}{\tilde f}
\newcommand{\ltwonorm}[1]{\|#1\|_2}
\newcommand{\coloneqq}{:=}
\newcommand{\metricsup}[2]{\|#1\|_{#2}}
\newcommand{\metricdyn}[3]{d_{#2, #3}(#1)}
\newcommand{\generalineq}{\unrhd}
\newcommand{\poly}[1]{\mathcal P_{#1}}
\newcommand{\SETALG}{\Lambda}
  
% path to images
%\graphicspath{ {./img/} }



\newcommand{\NINTERPOLATION}{\operatorname{{\bf Interp}}}
\newcommand{\NPOS}{\operatorname{{\bf Pos}}}
\newcommand{\NMON}{\operatorname{{\bf Mon}}}
\newcommand{\NINV}{\operatorname{{\bf Inv}}}
\newcommand{\NGRAD}{\operatorname{{\bf Grad}}}
\newcommand{\NHAMILTONIAN}{\operatorname{{\bf Ham}}}
\newcommand{\NSYM}{\operatorname{{\bf Sym}}}

  
\newcommand{\INTERPOLATION}[1]{\NINTERPOLATION(#1)}
\newcommand{\POS}[1]{\NPOS(#1)}
\newcommand{\MON}[1]{\NMON(#1)}
\newcommand{\INV}[1]{\NINV(#1)}
\newcommand{\GRAD}{\NGRAD}
\newcommand{\HAMILTONIAN}{\NHAMILTONIAN}
\newcommand{\SYM}[1]{\NSYM(#1)}


\newcommand{\LS}{{L_{S,\Omega}}}
\newcommand{\LiS}[1]{{L_{S_{#1},\Omega}}}

\newcommand{\CD}{{C_1^{\circ}(\Omega)}}


\newtheorem{mydef}{Definition}
\newtheorem{myexp}{Example}
\newtheorem{myremark}{Remark}
\usepackage[shortlabels]{enumitem}
%\usepackage{enumitem}

% \setlist{leftmargin=.5mm}

% \usepackage{titlesec}
% \titlespacing*{\section} {0pt}{6pt}{2pt}
% \titlespacing*{\subsection} {0pt}{6pt}{2pt}


\pgfplotsset{compat = 1.3}
% \titlespacing*{\subsection}
% {0pt}{5.5ex plus 1ex minus .2ex}{4.3ex plus .2ex}





%% Code style
\usepackage{listings}
\definecolor{commentgreen}{RGB}{2,112,10}
\definecolor{eminence}{RGB}{108,48,130}
\definecolor{weborange}{RGB}{255,165,0}
\definecolor{frenchplum}{RGB}{129,20,83}
\lstdefinestyle{JuliaListing}{
  language=Python,
  basicstyle=\small,
  numbers=none,
  stepnumber=1,
  numbersep=10pt,
  tabsize=4,
  showspaces=false,
  showstringspaces=false,
  commentstyle=\color{commentgreen},
  keywordstyle=\color{eminence},
  otherkeywords={@variable,@objective,@constraint,@polyvar},
  frame=tb,
  mathescape=true,
  escapechar=\%,
  captionpos=b,
}
\newcommand*{\CodeComment}[2][5.0cm]{\hfill\makebox[#1][l]{\textcolor{commentgreen}{\#
      #2}}}
\renewcommand{\lstlistingname}{Source Code}% Listing -> Algorithm

% \usepackage{jlcode}

  
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "Learning_with_side_information_SIREV_v1"
%%% End:


==> Learning with Side Info r1 -arxiv submission jan 17 2022 compressed/introduction.tex <==
\section{Introduction}
Our goal is to learn a dynamical system from a {limited}
number of {noisy} measurements of its
trajectories. Imagine, e.g., a passenger airplane that has
gone through sudden structural damage. Can we learn the new
dynamics on the fly so to autonomously land the plane?
Since data is scarce, side information (e.g., physical
laws/contextual knowledge) must be exploited. For instance,
we may know when the engines are off, the plane cannot
accelerate upwards, or some bounds on the velocities of all
the states.


% \begin{figure}\centering
%   \includegraphics[scale=.5]{airplane_example.png}
%   \caption{Caption}
% \end{figure}

% \begin{figure}\centering
%   \includegraphics[scale=.25]{sample_trajectories.png}
%   \caption{Sample trajectories.}
% \end{figure}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "Learning_with_side_information_L4DC_v1"
%%% End:


==> Learning with Side Info r1 -arxiv submission jan 17 2022 compressed/old_theorems.tex <==
\begin{theorem}\label{thm:sdp_finds_best_poly}
  Fix a degree $d$, training data $\mathcal D$ and a
  combination of side information $S_1, \ldots, S_m$ (where
  every $S_i$ is of the type in \cref{sec:side-info}). Let
  $\mathcal G \coloneqq \poly d \cap S_1 \cap \ldots \cap
  S_,$. Suppose that (i) the minimum value of training error 
  \[\sum_{(\x_i, \iy_i) \in \mathcal D}
    \ell(p(\x_i), \iy_i),\] over $\mathcal G$ is attained by
  $p^* \in \poly d$, and that (ii) $p^*$ satisfies the side
  information $S_1,\ldots,S_m$ strictly, then for $r$ large
  enough, the optimal value of the semidefinite
  program below gives a polynomial vector field that satisfies the
  side information $S_1, \ldots, S_m$ and gives the same
  training error as $p^*$.

  \begin{equation}
    \label{eq:learn_poly_vf_as_sdp}
    \begin{split}
    \min_{p \in \mathcal F}&
    \sum_{(\x_i, \iy_i) \in \mathcal D}
    \ell(p(\x_i), \iy_i)\\
    &p \in S_i^{(r)} \quad \text{for $i=1,\ldots,m$}.
    \end{split}
  \end{equation}
  
\end{theorem}

\begin{remark}
  Denote by $p$ the polynomial
  $x_1^4x_2^2 + x_1^2x_2^4 + x_3^6 - 3x_1^2x_2^2x_3^2,$
  known as the Motzkin polynomial, and let
  $g(x_1, x_2, x_3) \coloneqq 1 - (x_1^2 + x_2^2 + x_3^2)$.
  The polynomial $p$ is nonnegative on the unit ball
  \(\SETALG \coloneqq \{x \in \mathbb R^3 \; | \; g(x) \ge
  0\},\) yet there exists no certificate of the form in
  \cref{eq:putinar-certificate} to prove it, i.e., there
  exist no sum of squares $s_0$ and $s_1$ that satisfy
  $p = s_0 + s_1 g$ 
  (see \cite{motzkin_not_sos_ball_nie_2013}). This shows that the
  assumption that $p$ be positive (and not simply
  nonnegative) is truly needed for the result of
  \cref{th:putinar} to hold. We can use this observation to
  show that assumption (ii) in
  \cref{thm:sdp_finds_best_poly} is needed. Indeed, take
  $n=3$, $d=3$, and $S_1 = \INTERPOLATION{\{x_i, f(x_i)\}}$,
  then $S_1 \cap \poly 3 = \{ f \}$ but $S_1^{(r)} \cap \poly 3 = \emptyset$ for any integer $r$.

  
  
\end{remark}



\subsection{Polynomail approximation of continuously-differentiable vector fields}
\begin{theorem}
  Fix a compact set $\Omega \subset R^n$, a time horizon $T > 0$, and a desired accuracy $\varepsilon > 0$. Let $f: \mathbb R^n \rightarrow \mathbb R^n$ be a continuous differentiable vector field that satisfies any one of the following constraints
(i) equilibria at a given finite set of points,
(ii) invariance of a set satisfying (*) in \cref{def:strict_convex_set},
(iii) directional monotonicity,
(iv) nonnegativity,
(v) gradient or Hamiltonian structure,
(vi) sign symmetry.
Then there exists a polynomial vector field $p: \mathbb R^n \rightarrow \R^n$ such that
\[\metricdyn{f-g}{\Omega}{T} \le \varepsilon,\]
and $p$ satisfies the same side information as $f$. Furthermore, all such properties of $p$ come with an SOS certificate.
\end{theorem}


\begin{theorem}
  Fix a compact set $\Omega \subset R^n$, a time horizon $T > 0$, a desired accuracy $\varepsilon > 0$, and a room of error $\delta$. Let $f: \mathbb R^n \rightarrow \mathbb R^n$ be a continuous differentiable vector field that satisfies any \textit{combination} of the following constraints
(i) equilibria at a given finite set of points,
(ii) invariance of a set satisfying (*) in \cref{def:strict_convex_set}.
(iii) directional monotonicity,
(iv) nonnegativity,
(v) gradient or Hamiltonian structure,
(vi) sign symmetry.
Then there exists a polynomial vector field $p: \mathbb R^n \rightarrow R^n$ such that
\[\metricdyn{f-g}{\Omega}{T} \le \delta,\]
and $p$ $\delta\text{-satisfies}$ the same side information as $f$. Furthermore, all such properties of $p$ come with an SOS certificate.
\end{theorem}


\begin{definition}\label[definition]{def:strict_convex_set}
A set is said to satisfy (*) if (i) it is defined by finitely many inequalities $h_i(x) \ge 0$, where the $h_i$ are convex functions, and (ii) there exists $x_* \in \R^n$ such that $h_i(x_*) > 0 \; \forall i$.
\end{definition}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "Learning_with_side_information_L4DC_v1"
%%% End:


==> Learning with Side Info r1 -arxiv submission jan 17 2022 compressed/open_problems.tex <==
\section{Open Problems}
\begin{itemize}
\item Is it true that every semi-algebraic set can be made invariant by a non-zero polynomial vector field?
\item How about PDEs?
\item Statistical questions
\item Other side information than the one considered here? Non-convex side info?
\end{itemize}


%%% Local Variables:
%%% mode: latex
%%% TeX-engine: luatex
%%% TeX-master: "Learning_with_side_information_v1"
%%% End:


==> Learning with Side Info r1 -arxiv submission jan 17 2022 compressed/polynomial_vf.tex <==
\section{Learning Polynomial Vector Fields}


Let $S$ be a side information. A positive result is when $S \cap
\mathcal F$ is dense in $S$, otherwise, it is negative.

We summarize the results in the following table
%\def\checkmark{\tikz\fill[scale=0.4](0,.35) -- (.25,0) -- (1,.7) -- (.25,.15) -- cycle;} 
\newcommand{\Cross}{\ding{55}}%
\newcommand{\Checkmark}{$\color{black}\checkmark$}
\newcommand{\Unknownmark}{$\textbf{\color{red}??}$}

\begin{table}[H]
  \centering
  \begin{tabular}{l|c|c|c|c}
                  & nonnegativity & monotonicity & invariance   & Hamiltonian  \\
    \hline          
    interpolation & \Checkmark (if     & \Cross       & \Unknownmark & \Unknownmark \\
    nonnegativity &               & \Checkmark   & \Cross       & \Checkmark   \\ 
    monotonicity  &               &              & \Cross       & \Unknownmark \\
    invariance    &               &              &              & \Unknownmark \\
  \end{tabular}
  \caption{Which side information can be combined}
  \label{tab:summary-combine-side-info}
\end{table}

\begin{theorem}
  Let $S$ denote one of the sets below.  Then , the set $S$ at least
  one non-zero, continuously-differentiable vector field, and yet, the
  only polynomial vector field in $S$ is the identically zero vector field.
  \begin{itemize}
  \item $\INV{\Omega}$, where
    $\Omega \coloneqq \{ \frac1{2k\pi} \; | \; k \in \Z \setminus
    \{0\}\}$.
  \item
    $\INTERPOLATION{\{(x_i, v_i)\}_{i=1}^3} \cap \MON{([0, 1], \ge)}$,
    where $x_1=-1$, $x_2=0$, $x_3=1$ and $v_1=0$, $v_2=2$, $v_3=1$.
  \item $\INV{\Omega} \cap \POS{\Omega}$, where $\Omega = [-1, 0] \times [-1, 0]$ forces $f_1$ to be zero on $\{0\} \times \mathbb R$.
  \end{itemize}
\end{theorem}

% \begin{theorem}[Meta-theorem]
%   Let $f$ be a vector fields satisfying properties $P_1, \ldots, P_n$.
%   If all properties $P_i$ are strict, and at most one the $P_i$ is
%   nonopen, then for any positive scalar $\varepsilon$, there exists a
%   polynomial vector field $p$ such that $p$ satisfies
%   $P_1, \ldots, P_n$ and $\|f - p\| \le \varepsilon$.
% \end{theorem}

\subsection{Limitations of polynomials vector fields}
There are obvious limitations to polynomial vector fields. Imposing
too many side information can make the problem in (*) infeasible.


\subsubsection{No polynomial vector field makes the set $\Omega$ invariant}
The set $\Omega \coloneqq \{ \frac1{2k\pi} \; | \; k \in \Z \setminus \{0\}\}$
is clearly invariant for the dynamical system
$\dot x = x^2 \sin(\frac 1x)$. If the same set is invariant for a
dynamical system $\dot x = f(x)$ given by a polynomial function $f$,
then $f$ needs to have infinitely many roots, and therefore $f$ must
be identically zero.

\subsubsection{No polynomial vector field respects monotonicity and equilibirum points}
There exists no polynomial vector field $p: \R \rightarrow \R$ that respects the following side information
\begin{itemize}
\item $p(-1) = p(0) = 0$ and $p(1) = 1$
\item $p$ nondecreasing.
\end{itemize}

The (infinitely-many-times differentiable) function
\[f(x) \coloneqq \left\{ \begin{array}{ll}0&\text{if }x \le 0\\e^{1-\frac1{x^2}}&\text{if } x > 0\end{array}\right\}\]
does respect this side info.


\subsubsection{No polynomial vector field respects monotonicity and invariance}
The zero vector field is the only polynomial vector field $p: \R \rightarrow \R$ that respects the following side information
\begin{itemize}
\item $p$ leaves the interval $[0, 1]$ invariant.
\item $p$ is nondecreasing on $[0, 1]$.
\end{itemize}



\subsection{Positive results about polynomials vector fields}


The next theorem proves that any continuous function $f$ can be approximated uniformly by a polynomial $p$ on a compact set, even if we impose that $f$ and $p$ be equal on any finite number of points.

\begin{theorem}
  Let $\Omega \subseteq \R^N$ be a compact subset of $\R^n$ and consider a continuous function $f:\Omega\rightarrow \R$.
  For any $\varepsilon > 0$, for any $d$ points $\x_1, \ldots, \x_d \in \Omega$,
  there exists a polynomial $p \in \R[\x]$ such that
  \[\ltwonorm{p(\x) - f(\x)} \le \varepsilon \quad \forall x \in \Omega \text{ and } f(\x_i) = p(\x_i) \forall i \in \{1, \ldots, d\}\].
\end{theorem}

\begin{proof}
  Let $f:\Omega\rightarrow \R^n$ be a continuous vector field and fix a positive scalar $\varepsilon$. By Weirstrass theorem, there exists a polynomial $q \in \R[\x]$ such that $\ltwonorm{p(x) - f(x)} \le \varepsilon$ for all $x \in \Omega$.
  Now let  $\x_1, \ldots, \x_n \in \Omega$, and set $v_i \coloneqq f(\x_i) - q(\x_i)$. By Proposition \ref{prop:mon_vectors_are_indep}, there exists a polynomial $s \in \R_d[\x]$ such $s(\x_i) = v_i$ and $\max_{\Omega} |s| \le C(\x_1, \ldots, \x_d) \|v\|_2 \le \sqrt{d}C(\x_1, \ldots, \x_d) \varepsilon$.
  We let $p = q + s$, so that for any $\x \in \Omega$,
  \[\|f(\x) - p(\x)\| \le \|f(\x) - q(\x)\| + \|s(\x)\| \le (1+\sqrt{d}C(\x_1, \ldots, \x_d))\varepsilon,\]
  and for $i=1,\ldots,d$, $f(\x_i) - p(\x_i) = 0$.
  
\end{proof}


In the next theorem we prove that on any compact set, we can we can approximate vector field $f$ that satisfies some monotonicity constraints $\frac{\partial f_i}{\partial \x_j} \sim_{ij} 0$, where $\sim_{ij} \in \{ \ge , \le \}$ with a polynomial vector field that satisfies the same monotonicity constraints.
\begin{theorem}
  Let $\Omega \subseteq \R^N$ be a compact subset of $\R^n$, and consider  a continuously differentiable function $f:\Omega\rightarrow \R$ that satisfies:
  \[f \ge 0 \quad \forall \ix \in P, \]
  \[\frac{\partial f}{\partial \x_j}(\ix) >_j 0 \quad \forall \ix \in M_j \forall j \in \{1, \dots, n\}, \]
  where $>_i$ is either $\ge$ or $\le$, and $P$ and the $M_j$ are semi-algebraic sets.
  Then, for any $\varepsilon > 0$, there exists a polynomial function $p: \R^n \rightarrow \R$ such that
  \[\ltwonorm{p(\ix) - f(\ix)} \le \varepsilon \; \forall \ix \in \R^n,\quad   p \ge 0 \; \forall \ix \in P,\]
    \[\text{ and }
    \frac{\partial p}{\partial \x_j}(\ix) >_j 0 \; \forall \ix \in  M_j \forall j \in \{1, \dots, n\}, \]
\end{theorem}
\begin{proof}
  Consider the function $\tilde f$ defined by \[\tilde f = f + \beta\left(1  + \sum_{i, >_i = \ge} x_i - \sum_{i, >_i = \le} x_i\right).\]
  Then
  \[\ltwonorm{\tilde f(\ix) - f(\ix)} \le  \beta\; \forall \ix \in \R^n,\quad   \tilde f \ge \beta \; \forall \ix \in P,\]
    \[\text{ and }
    \frac{\partial \tilde f}{\partial \x_j}(\ix) >_j \beta \; \forall \ix \in  M_j \forall j \in \{1, \dots, n\}, \]
  The result follows by approximating $\tilde f$ by a polynomial uniformly for the $C^1\text{-norm}$.
\end{proof}

\begin{theorem}
  Let $\Omega \subseteq \R^N$ be a compact subset of $\R^n$, and consider  a continuously differentiable function $V:\Omega\rightarrow \R$ that satisfies:
  \[\frac{\partial V}{\partial x_i} >_i 0 \quad \forall \ix \in P_i, \]
  Then, for any $\varepsilon > 0$, there exists a polynomial function $W: \R^n \rightarrow \R$ such that
  \[\ltwonorm{\nabla V(\ix) - \nabla W(\ix)} \le \varepsilon \; \forall \ix \in \Omega,\quad   \frac{\partial W}{\partial x_i} >_i 0.\]
\end{theorem}

\begin{proof}
  Let $\tilde V = V + \beta \sum_{i=1}^n \pm x_i$
\end{proof}





% \section{Certificates of positivity in a Box}

% \begin{theorem}[Stengle]\label{thm:positivity in a box}
%   If a polynomial $p(x, y) \in \R[x, y]$ is positive on the box given by $\{(x, y) \; | \; x, y, 1-x, 1-y \ge 0\}$, then there exist sos polynomials $(\sigma_\alpha(x, y))$ indexed by $\alpha \in \{0, 1\}^4$ such that: 
%   \[p(x, y) =  \sum_{\alpha \in \{0, 1\}^4} \sigma_{\alpha}(x, y) x^{\alpha_1}y^{\alpha_2}(1-x)^{\alpha_3}(1-y)^{\alpha_4}\]
% \end{theorem}


\subsection{Multivariate Polynomial Interpolation}
\begin{proposition}[Proposition 4.3 in \cite{comon_symmetric_2008}]\label{prop:mon_vectors_are_indep}
  If $\x^1, \ldots, \x^d$ are $d$ different points of $\R^n$, the $m_d (\x^1), \ldots, m_d(\x^d)$ are linearly independent, where $m_d(\x^i) = (\x^i_{j_1}\ldots\x^i_{j_d})_{j_1, \ldots, j_d \in \{1, \ldots, n\}}$ is the vector of monomials in $\x_i$ up to degree $d$.
\end{proposition}
\begin{corollary}
  For any positive integers $d$ and $n$, for any $d$ points $\x^1, \ldots, \x^d$ in a compact set $\Omega$, there exists a constant $C(\x_1, \ldots, \x_d)$ such that the following holds:\\
  For any vector $v \in \R^d$, there exists a polynomial $p \in \R_d[\x]$ such that
  \[p(\x_i) = v_i, \quad i=1,\ldots,d \text{ and } \max_{\x \in \Omega} |p(\x)| \le C(\x_1, \ldots, \x_d) \|v\|_2\]
\end{corollary}
\begin{proof}
  By Proposition \ref{prop:mon_vectors_are_indep}, the system of linear equations
  \begin{equation}\label{eq:lin_system_poly}
    p(\x_i) = v_i \quad i=1,\ldots,n
    \end{equation}
    in the variable $p \in \R_d[\x]$ are independent. If we identify $p$ by its coefficients in the monomial basis, then we can rewrite the system in \eqref{eq:lin_system_poly} as
    \[A p = v,\]
    where $A = (m_d(\x^1), \ldots, m_d(\x^d))^T$ is a matrix depending only on $\x_1, \ldots, \x_d$ that has independent rows.
    The corollary follows by taking $C(\x_1, \ldots, \x_d)$ to be the operator norm of the matrix $M \coloneqq (A^TA)^{-1}A^T$ and $p = Mv$, and  
\end{proof}





\section{Polynomial Approximation of Vector Fields}

\begin{theorem}[Invariance]
  If the dynamical system $\dot \ix = f(\ix)$ leaves a star-shaped $B$
  invariant, then for every $\varepsilon > 0$, there exists a
  polynomial vector field $p$ that leaves the set $V$ invariant and
  \[\|f - p\| \le \varepsilon.\]
\end{theorem}


\begin{theorem}[Equilibrium Points]
  If the dynamical system $\dot \ix = f(\ix)$ leaves a star-shaped $B$
  invariant, then for every $\varepsilon > 0$, there exists a
  polynomial vector field $p$ that leaves the set $V$ invariant and
  \[\|f - p\| \le \varepsilon.\]
\end{theorem}

\begin{theorem}
  Let $f$ be vector field satisfying one of the following side information
  \begin{itemize}
  \item Nonnegativity on a set $B_1$, monotonicity on a set $B_2$, and strict invariance of a set $B_3$.
  \item Nonnegativity on a set $B_1$ and interpolation conditions $f(x_1) = v_1$, \dots, $f(x_m) = v_m$.
  \item Invariance of full-dimensional, star-shaped set $\Omega$.
  \end{itemize}
  Then, for every $\varepsilon > 0$, there exists a polynomial $p$ such that $\|p - f\| \le \varepsilon$ and $p$ satisfies the same side information as $p$.
\end{theorem}




%%% Local Variables:
%%% mode: latex
%%% TeX-engine: luatex
%%% TeX-command-extra-options: "-shell-escape"
%%% TeX-master: "Learning_with_side_information_v1"
%%% End:


==> Learning with Side Info r1 -arxiv submission jan 17 2022 compressed/problem_formulation.tex <==
\section{Introduction}


In several safety-critical applications, one has to learn
the behavior of an unknown dynamical system from noisy
observations of a very limited number of trajectories. For
example, to autonomously land an airplane that has just
gone through engine failure, limited time is available to
learn the modified dynamics of the plane before appropriate
control action can be taken. Similarly, when a new
infectious disease breaks out, few observations are
initially available to understand the dynamics of
contagion.  In situations of this type where data is
limited, it is essential to exploit ``side
information''---e.g. physical laws or contextual
knowledge---to assist the task of learning.

In this paper, we present a mathematical formalism of the
problem of learning a dynamical system with side
information, where side information means a concrete
collection of local and global properties of the dynamical
system that are commonly encountered in practice. We show
that sum of squares optimization is particularly suited for
learning a dynamical system that best agrees with the
observations and respects the side information.


\section{Problem formulation}
Our interest in this paper is to learn a dynamical system
\begin{equation}
  \frac{{\rm d}}{{\rm d}t} \ix(t) = f(\ix(t)), \quad f: \Omega \rightarrow \mathbb R^n,
  \label{eq:autonomous.dynamical.system}
\end{equation}
over a given compact set $\Omega \subset \R^n$. We consider
the setting where the vector field
$f: \Omega \rightarrow \mathbb R^n$ is unknown to us, and we
only require it to be continuously differentiable. This
requirement is often met in applications of interest to us,
and is known to be a sufficient condition for existence and
uniqueness of trajectories (see
\cite{khalil2002nonlinear}). We assume that we have access
to a set $\mathcal D$ of \textit{training data} of observed
trajectories and to \textit{side information} (We give a
concrete mathematical definition of this notion in
\cref{sec:side-info} below). Our training data is a set of
the form
\begin{equation}
 \mathcal D \coloneqq \{ (\ix_i, \iy_i),\quad i = 1,\ldots,N\},\label{eq:training-set}
\end{equation}
%
%
where every $\ix_i$ is a vector of $\mathbb R^n$, and
$\iy_i$ is a noisy measurement of $f(\ix_i)$. 
%
The evaluation points $\ix_i$ are either fixed vectors of
$\Omega$, or emanating from one (or few) trajectories
$\ix(t)$ at some snapshot times $t_i$, i.e.,
$\ix_i = \ix(t_i)$. The vectors $y_i$ could be directly
given (e.g., from sensor data), or approximated using a
finite-difference scheme.

%
Finding a vector field $f_{\mathcal F}$ that best agrees with
the unknown vector field $f$ among a class of
continuously-differentiable functions of interest
$\mathcal F$ amounts to solving the least-squares problem
\begin{equation}
  \label{eq:program_fit_vector_field} f_{\mathcal F} \in \arg \min_{p \in
\mathcal F} \sum_{(\ix_i, \iy_i) \in \mathcal D} \|p(\ix_i) - \iy_i\|,
\end{equation}
It turns out that our approach can readily handle other
types of losses (e.g., $\ell_1$ and $\ell_\infty$ losses,
any sos-convex loss function [**]).


\subsection{Side information}
\label{sec:side-info}

In addition to consistency with $f$, we want our learned
vector field $f_{\mathcal F}$ to also generalize reasonably
well in conditions that were not seen in the training
data. Indeed, the optimization problem
in~\eqref{eq:program_fit_vector_field} only dictates how the
candidate vector field should behave on the training data,
which could easily lead to over-fitting, especially if the
class of function $\mathcal F$ is large enough and the
observations are noisy and limited. Let us demonstrate this
issue with a simple example.

\begin{example}Consider the two-dimensional vector field
  $f(x_1, x_2) \coloneqq (x_2, -x_1)^T$. The trajectories
  of the system $\dot \ix = f(\ix)$ are given by circular
  orbits. In particular, if started from the initial condition
  $x_0 \coloneqq (1, 0)^T$, this trajectory is given by
  $\ix(t, x_0) =(\cos(t), \sin(t))^T$. As a result, for any
  function $g:\mathbb R^2\rightarrow \mathbb R^2$, the vector field
  \[h(\ix) \coloneqq f(\ix) + (x_1^2+x_2^2-1) g(\ix)\]
  agrees with $f$ on the sample trajectory $\ix(t, x_0)$,
  but the behavior of the trajectory of $h$ depend on the
  arbitrary choice of $g$. If $g(\ix) = \ix$ for instance,
  the trajectories of $h$ starting outside of the unit disk
  will diverge exponentially fast to infinity.


\end{example}


To address both issues of over-fitting and scarcity of data,
we suppose that we know, in addition to the the training
data $\mathcal D$, that the vector field $f$ or its
trajectories possess some additional properties that we call
{\it side information}. Formally, every side information is
a subset $S$ of the set of all continuously-differentiable
vector fields.  Our goal is then to learn a polynomial
vector field $p$ that satisfies the same side information,
i.e. $p \in S$, and agrees with $f$ on the training data to
arbitrary accuracy. The problem of learning a polynomial
vector field $p \in \mathcal F$ from data $\mathcal D$ and
side information $S_1, \dots, S_m$ can thus be formulated as
\begin{equation}
  \label{eq:program_fit_vector_field_with_side_info} \min_{p
\in \mathcal F \cap S_1 \cap \dots \cap S_m} \sum_{(\ix_i,
\iy_i) \in \mathcal D} \|p(\ix_i) - \iy_i\|^2.
\end{equation}

For arbitrary side information $S_1, \ldots, S_m$, the
problem in
\eqref{eq:program_fit_vector_field_with_side_info} is
challenging one. We focus our attention on the six types of
side information below. On the one hand, as we will see in
the numerical application section, they appear ubiquitously
in real life applications. On the other hand, they lead to a
semidefinite programming formulation of the problem in
\eqref{eq:program_fit_vector_field_with_side_info}.


\newcommand{\INTERPOLATION}[1]{\operatorname{{\bf
      INTERP}}(#1)}
\newcommand{\POS}[1]{\operatorname{{\bf
      POS}}(#1)}
\newcommand{\MON}[1]{\operatorname{{\bf
      MON}}(#1)}
\newcommand{\INV}[1]{\operatorname{{\bf
      INV}}(#1)}
\newcommand{\GRAD}{\operatorname{{\bf
      GRAD}}}
\newcommand{\HAMILTONIAN}{\operatorname{{\bf
      HAM}}}
\newcommand{\SYM}[2]{\operatorname{{\bf
SYM}}(#1, #2)}

\begin{itemize}
\setlength\itemsep{0em}
  
\item {\bf Interpolation at a finite set of points.} For
  every points $\ix_1, \ldots, \ix_m \in \mathbb R^n$ and
  scalars $y_1, \ldots, y_m \in \R^n$, we denote
  by $\INTERPOLATION{\{\ix_i,y_i\}}_{i=1}^m$ the set of
  vector fields $f$ that satisfy $f(\ix_i) = y_i$ for
  $i=1,\dots,m$. As an important special case, consider the
  setting where the scalars $y_i$ are equal to $0$,
  then the points $\ix_i$ correspond to equilibrium points
  of the vector field~$f$.
  
\item {\bf Sign symmetry.} For any two $n \times n$ diagonal matrices $A$ and $B$ with $1$ or $-1$ on the diagonal, We define $\SYM A B$ to be the set of vector fields $f$ satisfying the symmetry condition
  \[f(A\ix) = Bf(\ix) \quad \forall \ix \in \R^n.\]
  Note that the set $\SYM{-I} I$ (resp. $\SYM {-I} {-I}$) is the set of even (resp. odd) vector fields, where $I$ is the $n\times n$ identity matrix.

  
\item {\bf Coordinate nonnegativity.}  For sets
  $B_i \subseteq \Omega$, we denote by
  $\POS{ \{\generalineq_i, B_i\}_{i=1}^n }$ the set of
  vector fields $f$ that satisfy
  $f_i(\ix) \generalineq_i 0 \; \forall \ix \in B_i$ for
  $i \in \{1, \dots, n\}$, where $\generalineq_i$ stands for $\ge$ or~$\le$.

\item {\bf Coordinate-directional monotonicity.} Similarly,
  for sets $B_{i,j} \subseteq \Omega$, we denote the
  set of vector fields $f$ satisfying
  $\frac {\partial f_i}{x_j} (\ix) \generalineq_{i,j} 0 \; \forall \ix \in B_{i,j}$ for
  $i, j \in \{1, \dots, n\}$ by $\MON{ \{\generalineq_{i,j}, B_{i, j}\}_{i, j=1}^n}$.
  
\item {\bf Invariance of a set $B$.} We say that a set
  $B \subseteq \Omega$ is invariant for the vector field $f$
  if any trajectory of the dynamical system
  $\dot \ix = f(\ix)$, when started inside the set $B$,
  never leave $B$.

  In particular, if the set $B$ is
  given by inequalities $h_i(\ix) \ge 0$ for $i =1,\dots,m$,
  where the $h_i$ are continuously-differentiable functions,
  then the invariance of the set $B$ is given by the
  mathematical conditions
  %
  \begin{equation}
    \label{eq:eq-invariance} \langle f(\ix), \nabla h_i(\ix) \rangle \ge 0 \; \forall
\ix \in B_i \quad \text{where} \; B_i = B \cap \{h_i(x) = 0\},\text{ and } i=1,\dots,m.
\end{equation}
%
The set of all vector fields for which the set $B$ is invariant is denoted by $\INV{B}$.
  
\item {\bf Gradient and Hamiltonian systems.}  The vector
  field $f$ is said to be a \textit{gradient} if there
  exists a scalar-valued function $V: \R^n \rightarrow \R$
  such that
\begin{equation}
    \label{eq:def-gradient} f(\ix) = - \nabla V(\ix)\; \forall
\ix \in \R^n.
\end{equation}
Typically, the function $V$ is interpreted as a potential or
energy that decreases along the trajectories of the
dynamical system $\dot x = f(x)$.
The set of gradient vector fields is denoted by $\GRAD$.

A dynamical system is said to be \textit{Hamiltonian} if the dimension $n$ of the state space $x$ is even (say $n \eqqcolon 2k$), and a scalar-valued function $H: \R^k \times \R^k \longrightarrow \R$ such that

  \[\dot \ip = - \frac{\partial H}{\partial \iq} (\ip, \iq)
    \text{ and } \dot \iq = \frac{\partial H}{\partial \ip}
    (\ip, \iq),\] where $\ip^T = (\ix_1, \ldots, \ix_k)^T$
  and $\iq^T = (\ix_{k+1}, \ldots, \ix_n)^T$. The
  coordinates $\ip$ and $\iq$ are usually called
  \textit{momentum} and \textit{position} respectively,
  following naming convention in the field of physics. Note
  that in a Hamiltonian system, the quantity $H$ is
  conserved along its trajectories.  The set of Hamiltonian
  vector fields is denoted by $\HAMILTONIAN$. See
  \cite{greydanus2019hamiltonian,cheng2015learn}.
  
\end{itemize}



%%% local Variables:
%%% mode: latex
%%% TeX-engine: default
%%% TeX-master: "Learning_with_side_information_L4DC_v1"
%%% End:


==> Learning with Side Info r1 -arxiv submission jan 17 2022 compressed/review_sos.tex <==
\section{Learning Polynomial Vector Fields Subject to Side Information}
\label{sec:learn-poly-vec}


To completely define the problem in
\cref{eq:program_fit_vector_field_with_side_info}, we still
have to specify the set $\mathcal F$. Among the possible
choices are reproducing kernel Hilbert spaces
\cite{sindhwani2018learning,cheng2015learn}, trigonometric
functions, and functions parameterized by neural networks
\cite{neural_laypunov_nips_2019,greydanus2019hamiltonian}.
In this paper, we will take $\mathcal F$ to be set
\[ \poly d \coloneqq \{ p: \R^n \rightarrow \R^n \; | \; p_i
  \text{ is a polynomial of degree $d$ for $i=1,\ldots,n$}
  \}.\] Furthermore, we will assume that all subsets of
$\Omega$ considered in \cref{sec:side-info} in the
definition of side information (i.e., the sets $B_i$ in the
definition of nonnegativity, the sets $B_{ij}$ for the
definition of monotonicity, and the set $B$ in the
definition of invariance) are all \emph{closed basic
  semi-algebraic sets}. We recall that a closed basic
semialgebraic set is a subset of the Euclidean space of the
form
\begin{equation}\nonumber
\SETALG \coloneqq \{x\in\mathbb{R}^n|\ g_i(x)\geq 0, i=1,\ldots,m  \},
\end{equation}
where $g_1,\ldots,g_m$ are polynomial functions.


These choices are motivated by two reasons. The first is that polynomial functions are expressive enough to approximate a large family of functions. The second reason which shall be made clear in this paper is that because of some connections between real algebra and semidefinite optimization, several side information constraints that are commonly available in practice can be imposed on polynomial vector fields in a numerically tractable fashion. We note that the problem of fitting a polynomial vector field to data has appeared e.g. in \cite{schaeffer2018polylasso}, though the focus there is on imposing sparsity of the coefficients of the vector field as opposed to side information. The closest work in the literature to our work is that of Hall on shape-constrained regression \cite[Chapter 8]{phd:georgina18}, where similar algebraic techniques are used to impose constraints such as convexity and monotonicity on a polynomial regressor. See also \cite{shapeconstraints_aaa} for some statistical properties of these regressors and several applications. Our work can be seen as an extension of this approach to a dynamical system setting.



The optimization problem of interest to us has as decision
variables the coefficients of a candidate polynomial vector
field $p$. The objective function is a convex quadratic
function of these coefficients, and the constraints are
twofold: (i) affine constraints in the coefficients of $p$,
and (ii) constraints of the form
\begin{equation}\label{eq:p>=0.on.Omega}
q(x)\geq 0\  \forall x\in \SETALG,
\end{equation}
where $\SETALG$ is a given closed basic semialgebraic set, and $q$
is a (univariate) polynomial whose coefficients depend
linearly on the coefficients of the polynomial $q$.  For
example, it is easy to see that membership to
$\INTERPOLATION{\{\ix_i,\alpha_i\}}_{i=1}^m$, $\GRAD$, and
$\HAMILTONIAN$ are all given by affine constraints, while
membership $\POS{ \{>_i, B_i\}_{i=1}^n }$,
$\MON{ \{>_{i,j}, B_{i, j}\}_{i, j=1}^n}$, and $\INV{B}$ can
be case as a constraint of the type in (ii). Unfortunately,
imposing the constraint in (\ref{eq:p>=0.on.Omega})
is NP-hard already when $q$ is a quartic polynomial and
$\SETALG=\mathbb{R}^n$, or when $q$ is quadratic and $\SETALG$ is a
polytope.

An idea pioneered to a large extent by Lasserre~\cite{lasserre_moment} and Parrilo~\cite{sdprelax} has been to write algebraic sufficient conditions for (\ref{eq:p>=0.on.Omega}) based on the concept of sum of squares polynomials. We say that a polynomial $h$ is a \emph{sum of squares} (sos) if it can be written as $h=\sum_i q_i^2$ for some polynomials $q_i$. Observe that if we succeed in finding sos polynomials $\sigma_0,\sigma_1,\ldots, \sigma_m$ such that the polynomial identity
\begin{equation}\label{eq:putinar-certificate}
q(x)=\sigma_0(x)+\sum_{i=1}^{m}\sigma_i(x)g_i(x)
\end{equation}
holds, then, clearly, the constraint in (\ref{eq:p>=0.on.Omega}) must be satisfied. When the degree of the sos polynomials $\sigma_i$ is bounded by an integer $r$, we refer to \cref{eq:Putinar.proof} as the \emph{$r\text{-degree}$ Putinar's certificate} corresponding to the polynomial inequality \eqref{eq:p>=0.on.Omega}. Conversely, a celebrated result in algebraic geometry~\cite{putinar1993positive} states that if $g_1,\ldots,g_m$ satisfy the so-called ``Archimedean property'' (a condition slightly stronger than compactness of the set $\SETALG$), then positivity of $q$ on $\Lambda$ guarantees existence of an $r\text{-degree}$ Putinar's certificate for some integer $r$ large enough.

%:\mathbb{R}^n\rightarrow\mathbb{R}

The computational appeal of the sum of squares approach stems from the fact that the search for sos polynomials $\sigma_0,\sigma_1,\ldots, \sigma_m$ of a given degree that verify the polynomial identity in (\ref{eq:Putinar.proof}) can be automated via semidefinite programming. This is true even when some coefficients of the polynomial $p$ are left as decision variables. This claim is a straightforward consequence of the following well-known fact (see, e.g.,~\cite{PhD:Parrilo}): A polynomial $h$ of degree $2d$ is a sum of squares if and only if there exists a symmetric matrix $Q$ which is positive semidefinite and verifies the identity $$h(x)=z(x)^TQz(x),$$ where $z(x)$ here denotes the vector of all monomials in $x$ of degree less than or equal to $d$.

%%% Local Variables:
%%% mode: latex
%%% TeX-engine: default
%%% TeX-master: "Learning_with_side_information_L4DC_v1"
%%% End:


==> Learning with Side Info r1 -arxiv submission jan 17 2022 compressed/table_sideinfo.tex <==
\begin{table}[]
\begin{tabular}{lllll}
vector field used & x1 & x2 &  &  \\
LSQ               &    &    &  &  \\
LSQ               &    &    &  &  \\
                  &    &    &  & 
\end{tabular}
\end{table}


\begin{table}[]
\begin{tabular}{lll}
LSQ & 0.45 &  0.4\\
EQ & 0.41 &  0.29\\
EQ+INV & 0.31 &  0.12\\
EQ+INV+MON & 0.01 &  0.01\\
TRUE & 0.0 &  0.0
\end{tabular}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "Learning_with_side_information_SIREV_v1"
%%% End:


==> Learning with Side Info r1 -arxiv submission jan 17 2022 compressed/theorems.tex <==
\section{Approximation Results}

\subsection{Measure of similarity between vector fields}

Fix a compact set $\Omega \subset \R^n$. In order the assess
how close two vector fields $f, g: \Omega \rightarrow \R^n$
are, we define the following two metrics. The first one
compares directly the values taken by $f$ and $g$ on the
compact set $\Omega$:
\[\metricsup{f-g}{\Omega} \coloneqq \max_{\ix \in \Omega}
  \ltwonorm{f(\ix)-g(\ix)}\] From a dynamics point view, we
are also interested in how different the trajectories of $f$
and $g$ starting from an invariant set $\Omega$ are after
some time $T > 0$, i.e.
\[\metricdyn{f, g}{\Omega}{T} \coloneqq \sup_{\ix_0 \in \Omega,
    t \in [0, T]} \max\{\ltwonorm{\ix(t, \ix_0) - \iy(t,
    \ix_0)}, \ltwonorm{\dot \ix(t, \ix_0) - \dot \iy(t,
    \ix_0)}\] where $\ix(t, \ix_0)$ (resp. $\iy(t, \ix_0)$)
is the trajectory starting from $\ix_0 \in \Omega$ and
following the dynamics of $f$ (resp. $g$).
%

The metric $\metricdyn{\cdot, \cdot}{\Omega}{T}$ is ``finer'' than
$\metricsup{\cdot}{\Omega}$.  Indeed, by noting that
$\dot \ix(0, \ix_0) = f(\ix_0)$ and
$\dot \iy(0, \ix_0) = g(\ix_0)$, we obtain that
$\metricdyn{f, g}{\Omega}{T} \le \metricsup{f -
  g}{\Omega}$. The next proposition shows a reverse
inequality for Lipchitz vector fields that leave the set
$\Omega$ invariant.

\begin{proposition}\label{prop:equivalence-metric-vf} Fix a compact
set $\Omega \in \R^n$ and two positive scalars $T$ and
$L$. There exists a constant $C_{\Omega,T,L}$ such that
\[\metricsup{f-g}{\Omega} \le \metricdyn{f, g}{\Omega}{T} \le
  C_{\Omega,T,L} \metricsup{f-g}{\Omega}\] for every
continuously-differentiable vector field $f$ and for every
continuously-differentiable and $L\text{-Lipchitz}$ vector
field $g$ that leave the set $\Omega$.
\end{proposition}

\subsection{Satisfying side information approximately}
In section, we introduce the following notion approximately satisfying
side information.
\begin{definition}($\delta\text{-satisfiability}$) For any
  $\delta >0$ and side information $S$ presented in
  \cref{sec:side-info}, we say that a vector field $f$
  $\delta\text{-satisfies}$ $S$, and we write
  $f \in S^{\delta}$, if for any equality $a = b$
  (resp. inequality $a \le b$) appearing in the definition
  $S$, the vector field $f$ satisfies the modified version
  $|a - b| \le \delta$ (resp. $a \le b + \delta$).
\end{definition}

\begin{example}
  A vector $f$  $\delta\text{-satisfies}$ the side information $\INTERPOLATION{\{\ix_i,\alpha_i\}}_{i=1}^m$ if
  \( \|f(x_i) - \alpha_i\| \le \delta \quad i=1,\ldots,m. \)
\end{example}

The motivation for this definition is three-fold. First, we are happy in practice with a solution that satisfies an approximate version of the constraint. Second, due to numerical considerations, solvers return only a solution that satisfies an approximate version of the constraint. Finally, due to algebraic and approximation-theoretic reasons, if we take as our class of admissible vector fields polynomials of some bounded degree, a polynomial vector field satisfying the side information exactly might be computationally hard to find or simply not exist.


\subsection{Semidefinite programming hierarchy for approximating continuously-differentiable vector fields}

Let us now introduce some notation. For any side information
introduced in \cref{sec:side-info} given by a set $S$, we
denote by $S^{(r)}$ (resp. $S^{\delta, (r)}$) the set
obtained from $S$ by replacing any inequality of type
\eqref{eq:p>=0.on.Omega} with the corresponding equality in
\eqref{eq:putinar-certificate} suggested by Putinar's
Positivstellensatz, with the degree of the multipliers $s_i$
capped at $r$. Similarly, we define $S^{\delta, (r)}$ to be the set obtained from $S^{\delta}$, the $\delta\text{-approximation}$ of $S$.

\begin{example}
  % If \(S = \INTERPOLATION{\{\ix_i,\alpha_i\}}_{i=1}^m\),
  % then $S^{(r)} = S$ for all integers $r$. 
  If \(S = \INV B\), and $B$ is a closed semialgebraic set
  defined by polynomial inequalities $h_i(\ix) \ge 0$ for
  $i =1,\dots,m$, then, in view of \eqref{eq:eq-invariance},
  the set $S^\delta$ is given by continuously-differentiable vector fields $f$ that satisfy
  \[\langle f(\ix), \nabla h_j(\ix) \rangle \ge -\delta \quad \forall x \in B \cap \{h_j(x) = 0\}.\]
  Elements of \(S^{\delta, (r)}\)  are
  given by polynomial vector fields $p$ that satisfy the
  equalities
  \[\langle p(\ix), \nabla h_j(\ix) \rangle + \delta = \sum_{i=1}^m s_i^{(j)}(\ix) h_i(\ix) + r^{(j)}(\ix) h_j(\ix) \quad \forall x \in B \cap \{h_j(x) = 0\}\]
  for \(j=1,\ldots,m\), where the $r^{(j)}$
  (resp. $s^{(j)}_i$) are polynomials (resp. sos
  polynomials) of degree $r$.
\end{example}



The following theorem shows that polynomial vector fields can approximate any vector fields $f$ and satisfy the same side information as $f$ (up to an arbitrarily small error tolerance $\delta$).

\begin{theorem}\label{thm:poly_approx}
  Fix a compact set $\Omega \subset \R^n$, a time horizon
  $T > 0$, a desired accuracy $\varepsilon > 0$, and a room
  of error $\delta$. Let $f: \R^n \rightarrow \R^n$ be a
  continuously differentiable vector field that satisfies any
  combination of the side information in
  \cref{sec:side-info}. Then, there exists a polynomial
  vector field $p: \R^n \rightarrow \R^n$ such that
\[\metricdyn{f, p}{\Omega}{T} \le \varepsilon,\]
and $p$ $\delta\text{-satisfies}$ the same side information as $f$.
\end{theorem}

It should be clear that for any integer $r$ and scalar
$\delta$, the constraint ``$q~\in~S^{\delta, (r)}$'' is a
semidefinite-programming constraint. The following theorem
leverages this observation to show that the problem of
learning a polynomial vector field with side information can
be cast as a semidefinite program.


\begin{theorem}\label{thm:sdp_finds_best_poly}
  Fix a time horizon $T > 0$, a desired
  accuracy $\varepsilon > 0$, and a error tolerance
  $\delta > 0$. Let $f: \Omega \rightarrow \R^n$ be
  a continuous differentiable vector field that satisfies
  side information $S_1, \ldots, S_m$, and $\mathcal D$ be a training data. For $d$ and $r$ large enough, the semidefinite program 

  \begin{equation}
    \label{eq:learn_poly_vf_as_sdp}
    \begin{split}
    \min_{p \in \poly d}&
    \sum_{(\x_i, \iy_i) \in \mathcal D}
    \|p(\x_i) - \iy_i\|^2\\
    &p \in S_i^{\delta, (r)} \quad \text{for $i=1,\ldots,m$}.
    \end{split}
  \end{equation}
  becomes feasible. Furthermore, if we denote by
  $p^{d,r,\delta}$ an optimal solution to
  \eqref{eq:learn_poly_vf_as_sdp}, then the sequence of
  losses
  $\{\sum_{(\x_i, \iy_i) \in \mathcal D}
  \|p^{d,r,\delta}(\x_i) - \iy_i\|^2\}_{d,r}$ 
  is decreasing in both $d$ and $r$, and its limit as
  $d, r \rightarrow \infty$ is at most equal to
  $\sum_{(\x_i, \iy_i) \in \mathcal D} \|f(\x_i) -
  \iy_i\|^2$.
\end{theorem}


\subsection{Approximation of vector fields by polynomials that satisfy side information exactly}

In the previous section, we showed that polynomials are good
candidate for the task of learning vector fields from data
and side information if one is allowed to satisfy the side
information only approximately. Nevertheless, we think that
the mathematical question of deciding whether it is possible
to approximate an unknown vector field with a polynomial
vector field satisfying a given collection of side
information exactly is an interesting one. We give a
positive and a negative result in this direction.


The following definition establishes a notation that we will use in the statement of the results of this section.

\begin{definition}\label[definition]{def:strict_convex_set}
A closed semialgebraic set is said to be strictly convex if (i) it is defined by finitely many inequalities $h_i(x) \ge 0$, where the $h_i$ are convex polynomials, and (ii) there exists $x_* \in \R^n$ such that $h_i(x_*) > 0 \; \forall i$.
\end{definition}


\begin{theorem}
  Fix a compact set $\Omega \subset R^n$, a time horizon $T > 0$, and a desired accuracy $\varepsilon > 0$. Let $f: \mathbb R^n \rightarrow \mathbb R^n$ be a continuous differentiable vector field that satisfies exactly one of the following constraints
(i) equilibria at a given finite set of points,
(ii) invariance of a strictly convex set,
(iii) directional monotonicity,
(iv) nonnegativity,
(v) gradient or Hamiltonian structure,
(vi) sign symmetry.
Then there exists a polynomial vector field $p: \mathbb R^n \rightarrow \R^n$ such that
\[\metricdyn{f, p}{\Omega}{T} \le \varepsilon,\]
and $p$ satisfies the same side information as $f$. Furthermore, all such properties of $p$ come with an SOS certificate.
\end{theorem}

A natural question is whether the previous theorem could be generalized to allow for polynomial approximation of vector fields satisfying \emph{combinations} of side information exactly. The next simple example shows that the answer is negative, even when the dimension of the state variable is one.


\begin{example}
  Let $f:[-1, 1]\rightarrow\R$ be the continuously differentiable function defined piece wise by $f(x) = 0$ when $x < 0$ and $f(x) = e^{-1/x^2}$. The function $f$ can be viewed as vector field satisfying the side information (i) $S_1 \coloneqq \INTERPOLATION{ (-1, 0), (0, 0)}$ (i.e., $f(-1) = f(0) = 0$) and (ii) $S_2  \coloneqq \MON{[-1, 1], \ge}$ (i.e., $f$ nondecreasing on $[-1, 1]$). However, it is easy to see that the only polynomial contained in $S_1 \cap S_2$ is the identically zero polynomial.
\end{example}


The next example shows that even in the case where the unknown vector field happen to be polynomial, 

\begin{example}
  Denote by $p$ the polynomial
  $x_1^4x_2^2 + x_1^2x_2^4 + x_3^6 - 3x_1^2x_2^2x_3^2,$
  known as the Motzkin polynomial, and let
  $g(x_1, x_2, x_3) \coloneqq 1 - (x_1^2 + x_2^2 + x_3^2)$.
  The polynomial $p$ is nonnegative on the unit ball
  \(\SETALG \coloneqq \{x \in \R^3 \; | \; g(x) \ge 0\},\)
  yet there exists no certificate of the form in
  \eqref{eq:putinar-certificate} to prove it, i.e., there
  exist no sum of squares $s_0$ and $s_1$ that satisfy
  $p = s_0 + s_1 g$ (see
  \cite{motzkin_not_sos_ball_nie_2013}). This shows that the
  assumption that $p$ be positive (and not simply
  nonnegative) is truly needed for the result of
  \cref{th:putinar} to hold. We can use this observation to
  show that setting $\delta = 0$ in
  \cref{thm:sdp_finds_best_poly} would lead to an infeasible
  problem. Indeed, take $n=3$, $d=3$, and
  $S_1 = \INTERPOLATION{\{x_i, f(x_i)\}}$, then
  $S_1 \cap \poly 3 = \{ f \}$ but
  $S_1^{(r)} \cap \poly 3 = \emptyset$ for any integer $r$.
\end{example}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "Learning_with_side_information_L4DC_v1"
%%% End:


==> Learning with Side Info r1 -arxiv submission jan 17 2022 compressed/tikz_img/cancer_true_vf.tex <==
\loadvf{data/cancer/segments_two_compartment_model_vf.csv}{data/cancer/arrows_two_compartment_model_vf.csv}
\begin{figure}[H]
  \centering
  \begin{tikzpicture}
    \begin{axis}[no markers, enlargelimits=false, scale=1,
      xmin=-.1,xmax=2,
      ymin=-.1,ymax=2]
      \plotsegmentsvf{}
      \plotarrowsvf{}
      \draw[dashed, red, very thick] (0, -.1) -- (0, 4);
      \draw[dashed, red, very thick] (-.1, 0) -- (4, 0);
      \addplot[only marks, mark=*, red] table [x=N, y=K, col sep=comma]
      {data/cancer/cancer_data_points.csv};
    \end{axis}
    
  \end{tikzpicture}
  \caption{{\label{fig:two_compartment_model_vf}Vector
  field describing the dynamics of the population of tumor cells.}}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-engine: luatex
%%% TeX-master: "main.tex"
%%% End:


==> Learning with Side Info r1 -arxiv submission jan 17 2022 compressed/tikz_img/comparison_trajectory_pendulum.tex <==
\begin{figure}[H]
  \begin{tikzpicture}
    \begin{groupplot}[group style={
                              group size=1 by 3,
                              vertical sep=2cm,
                              ylabels at=edge left},
                              width=.75\textwidth,
                              height=6cm]
\nextgroupplot[title = {Trajectories generated form the polynomial vector field learned from data.}, legend pos=north east, xlabel=$t$, ylabel=$\theta(t)$]{
    \addlegendentry{Data}
    \addplot[restrict x to domain=0:3.1, mark=*, red, mark repeat={10}] table [x=t, y=theta1, col sep=comma]
    {data/pendulum/trajectory_simple_pendulum_true_vf.csv};

    \addlegendentry{Ground truth}
    \addplot[smooth, restrict x to domain=0:20,  red, dashed] table [x=t, y=theta1, col sep=comma]
    {data/pendulum/trajectory_simple_pendulum_true_vf.csv};

    \addlegendentry{Polynomial vector field}
    \addplot[smooth] table [x=t, y=theta1, restrict x to domain=0:20,
    col sep=comma]
    {data/pendulum/trajectory_simple_pendulum_poly_vf.csv};

    \addplot[dashed, mark=none] coordinates {(3, -1) (3, 2)};
    \coordinate (top) at (axis cs:1,\pgfkeysvalueof{/pgfplots/ymax});
  }
  
\nextgroupplot[align=center, title = {Trajectories generated form the polynomial vector field learned from data taking\\ into account all the side info.}, legend pos=north east, xlabel=$t$, ylabel=$\theta(t)$, xtick={0, 5, ..., 20}, yticklabels={$-\frac{\pi}4$, $0$, $\frac{\pi}{4}$}, ytick={-0.7854, 0, 0.7854}]{
 % \begin{axis}[legend pos=outer north east, xlabel=$t$, ylabel=$\theta$]
    \addlegendentry{Data}
    \addplot[restrict x to domain=0:3.1, mark=*, red, mark repeat={10}] table [x=t, y=theta1, col sep=comma]
    {data/pendulum/trajectory_simple_pendulum_true_vf.csv};

    \addlegendentry{Ground truth}
    \addplot[smooth, restrict x to domain=0:20,  red, dashed] table [x=t, y=theta1, col sep=comma]
    {data/pendulum/trajectory_simple_pendulum_true_vf.csv};

    \addlegendentry{Poly+side info}
    \addplot[smooth] table [x=t, y=theta1, restrict x to domain=0:20,
    col sep=comma]
    {data/pendulum/trajectory_simple_pendulum_hamiltonian_sym_pos_vf.csv};

    \addplot[dashed, mark=none] coordinates {(3, -1) (3, 2)};
    \coordinate (bot) at (axis cs:1,\pgfkeysvalueof{/pgfplots/ymin});
  }
  \end{groupplot}
  %\draw [thin] (top) -- (bot);


  \end{tikzpicture}
  \caption{\label{fig:abserror}Plot showing (a) position ${\mathbf{P_{T}}}$ and (b) the Parameters Absolute Errors.}
\end{figure}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End:


==> Learning with Side Info r1 -arxiv submission jan 17 2022 compressed/tikz_img/disease_true_vf.tex <==
\newcommand{\boxtikz}{\draw[dashed] (0,0) -- (1,0) -- (1,1) -- (0,1) -- (0,0);}

\begin{figure}[ht!]
  \centering
  \begin{tikzpicture}
    \begin{axis}[no markers, enlargelimits=false]
      \boxtikz
      \plotsegmentsvf{}
      \plotarrowsvf{}
      \addplot[red, thick, mark=+,  mark size=8pt] table [x=x, y=y]{data/disease/disease_training_data.csv};
    \end{axis}
  \end{tikzpicture}
  \caption{\label{fig:vf_diffusion_disease}The vector field in \eqref{eq:diffusion_disease} corresponding to $(a_1, a_2, b_1, b_2, c_1, c_2) = (.05,.1,.05,.1,1.,1.)$ together with some sample trajectories.}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> Learning with Side Info r1 -arxiv submission jan 17 2022 compressed/tikz_img/invariance_explanation.tex <==
\begin{center}
  \begin{tikzpicture}[scale=.2]
    \draw[rounded corners=.5cm] (0,0) -- (0,5) -- (10,10) -- (15, 5) -- (10,0) -- cycle node[text=black] {$\partial B$};
    \draw[rounded corners=.5cm, fill=gray!20] (0,0) -- (0,5) -- (10,10) -- (15, 5) -- (10,0) -- cycle;
    \draw[blue, -{Latex[length=2mm, width=1mm]}] (5, 7.5) -- (3, 10)node[left]{$n(x)$};
    \draw[red, -{Latex[length=2mm, width=1mm]}] (5, 7.5) -- (3, 5)node[right]{$p(x)$};
  \end{tikzpicture}
\end{center}

  
%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> Learning with Side Info r1 -arxiv submission jan 17 2022 compressed/tikz_img/plot_cancer_N_K.tex <==

\begin{tikzpicture}
  \begin{axis}[legend pos=north west,
    xlabel=$t$]
  \addplot[smooth, mark=*,each nth point={10},red] table [x=t, y=K, col
  sep=comma] {data/cancer/trajectory_grwoth_tumor.csv};
  \addlegendentry{$K(t)$}
  \addplot[smooth, mark=+,each nth point={10},blue] table [x=t, y=N, col sep=comma]
  {data/cancer/trajectory_grwoth_tumor.csv};
  \addlegendentry{$N(t)$}
\end{axis}
\end{tikzpicture}

%%% Local Variables:
%%% mode: latex
%%% TeX-engine: luatex
%%% TeX-master: "main.tex"
%%% End:







==> Learning with Side Info r1 -arxiv submission jan 17 2022 compressed/tikz_img/vf_learned_cancer.tex <==
\newcommand{\plotcancerlearnedvf}[3]{
  \nextgroupplot[align=left, title = {#2}, enlargelimits=false,
  xmin=-.1,xmax=2,
  ymin=-.1,ymax=2]{
    \loadvf{data/cancer/segments_#1.csv}{data/cancer/arrows_#1.csv}
    \plotsegmentsvf{}
    \plotarrowsvf{}
    \draw[dashed, red, very thick] (0, -.1) -- (0, 4);
    \draw[dashed, red, very thick] (-.1, 0) -- (4, 0);
    #3
}
}


\begin{figure}[H]
  \begin{tikzpicture}
    \begin{groupplot}[group style={
                              group size=2 by 1,
                              vertical sep=2cm,
                              ylabels at=edge left},
                              width=.5\textwidth,
                              height=6cm]
\plotcancerlearnedvf{two_compartment_model_learned_vf_no_side_info_deg_4}
{\label{fig:two_compartment_model_learned_vf_no_side_info}Best polynomial vector field of\\ degree 4 without side info.}{\draw[dashed, black, very thick] (0.05, 1.8) circle (.4cm);}

\plotcancerlearnedvf{two_compartment_model_learned_vf_with_side_info_deg_4}{\label{fig:two_compartment_model_learned_vf_with_side_info}Best polynomial vector field\\ of degree 4 with side info.}{}
\end{groupplot}
\end{tikzpicture}
\caption{Learned vector fields with and without side information.}

\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-engine: luatex
%%% TeX-master: "main.tex"
%%% End:
 

==> Learning with Side Info r1 -arxiv submission jan 17 2022 compressed/tikz_img/vf_learned_pendulum.tex <==
\newcommand{\plotpendulumlearnedvf}[3]{
  \nextgroupplot[title = {#2}, enlargelimits=false,
  xtick={-3.14, 0, 3.14}, xticklabels={$-\pi$, $0$, $\pi$},
  ytick={-3.14, 0, 3.14}, yticklabels={$-\pi$, $0$, $\pi$}]{
    \loadvf{data/pendulum/segments_#1_vf.csv}{data/pendulum/arrows_#1_vf.csv}
    \plotsegmentsvf{}
    \plotarrowsvf{}
    \draw[red, dashed, very thick] (-3.14,-3.14) -- (-3.14,3.14) --
    (3.14,3.14) -- (3.14,-3.14) -- cycle;
    \addplot[restrict x to domain=0:3.1, only marks, mark=*, red, mark repeat={10}] table [x=theta1, y=theta_dot1, col sep=comma]
    {data/pendulum/trajectory_simple_pendulum_true_vf.csv};
    \addplot[restrict x to domain=0:3.1, only marks, mark=*, red, mark repeat={10}] table [x=theta2, y=theta_dot2, col sep=comma]
    {data/pendulum/trajectory_simple_pendulum_true_vf.csv};
    #3
    
}
}


\begin{figure}[H]
  \begin{tikzpicture}
    \begin{groupplot}[group style={
                              group size=2 by 2,
                              vertical sep=2cm,
                              ylabels at=edge left},
                              width=.5\textwidth,
                              height=6cm]
\plotpendulumlearnedvf{poly}{Polynomial}{}
\plotpendulumlearnedvf{hamiltonian}{Hamiltonian}{}
\plotpendulumlearnedvf{hamiltonian_sym}{Hamiltonian + Symmetry}{
  \draw[dashed, black, very thick] (-3.14,3.14) circle (.4cm);
}
\plotpendulumlearnedvf{hamiltonian_sym_pos}{Hamiltonian + Symmetry +
  Pos}{}
\end{groupplot}

\end{tikzpicture}
\caption{Learned vector fields with side information.}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-engine: luatex
%%% TeX-master: "main.tex"
%%% End:
 

==> Learning with Side Info r1 -arxiv submission jan 17 2022 compressed/tikz_img/vf_true_pendulum.tex <==
\begin{figure}[H]
  \centering
    \loadvf{data/pendulum/segments_true_vf.csv}{data/pendulum/arrows_true_vf.csv}
  \begin{tikzpicture}
    \begin{axis}[no markers, enlargelimits=false]
        \plotsegmentsvf{}
        \plotarrowsvf{}
    \end{axis}
  \end{tikzpicture}
  \caption{True pendulum vector field}
\end{figure}




==> abstract.tex <==
We present a mathematical formalism of the problem of
learning a dynamical system from (scarce and limited)
observed trajectories and contextual side information
(e.g. physical laws or contextual knowledge). We show
that sum of squares optimization is particularly suited
for learning a dynamical system that best agrees with the
observations and respects the side information.  We
demonstrate the efficacy of our learning technique to
applications from epidemiology and physics.

% In several safety-critical applications, one has
% to learn the behavior of an unknown dynamical
% system from noisy observations of a very limited
% number of trajectories. For example, to
% autonomously land an airplane that has just gone
% through engine failure, limited time is available
% to learn the modified dynamics of the plane before
% appropriate control action can be
% taken. Similarly, when a new infectious disease
% breaks out, few observations are initially
% available to understand the dynamics of contagion.
% In situations of this type where data is limited,
% it is essential to 


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "Learning_with_side_information_L4DC_v1"
%%% End:


==> applications.tex <==
\section{Illustrative Experiments}

\subsection{Diffusion of a contagious disease}
The following dynamical system has appeared in the epidemiology literature (see, e.g., \cite{anderson1992infectious}) as a model for the spread of Gonorrhea in a heterosexual population:
\begin{equation}  \label{eq:diffusion_disease}
    \dot \ix = f(\ix)
  \quad \text{where} \; \ix \in \R^2 \text{ and }
  f(\ix) = \left(
    \begin{array}{l}
      -a_1   x_1 + b_1 (1-x_1) x_2\\
      -a_2   x_2 + b_2 (1-x_1) x_2
    \end{array}\right).
\end{equation}
Here, the quantity $x_1(t)$ (resp. $x_2(t)$) represents the fraction of infected males (resp. females). The parameters $a_i$ and $b_i$ denotes the recovery and infection rates respectively for males when $i=1$, and for females when $i=2$. We take \[(a_1, b_1, a_2, b_2) = (0.05 , 0.1, 0.05, 0.1),\] and we plot the resulting vector field $f$ in \cref{fig:vf_diffusion_disease}. We suppose that this vector field is unknown to us, and our goal is to approximate it based on the noisy sample observations
\[ \mathcal D \coloneqq \left\{ (\ix(t_i), f(\ix(t_i))+ 10^{-4} \begin{pmatrix}\varepsilon_i^1\\\varepsilon_i^2\end{pmatrix}) \right\}_{i=1}^{20}, \]
where $\ix(t, x_0)$ is the trajectory obtained when the flow in \eqref{eq:diffusion_disease} is started from the initial condition $\ix_0 = (0.7, 0.3)^T$, the $t_i \coloneqq  i/20$ represent regular subdivision of the time interval $[0, 1]$, and the $\varepsilon_i^{1}, \varepsilon_i^{2}$ are independent standard normal variables.

\begin{figure}
  \centering
  % Vertical alignment is controlled through optional argumants [c], [t] or [b] of minipage`.
  \begin{minipage}[c]{.5\textwidth}
    \includegraphics[width=.5\textwidth, trim=0 10 0 0, clip]{imgs/disease/disease_true_vf.png}
  \end{minipage}
  \begin{minipage}[c]{.4\textwidth}
    \caption{\label{fig:vf_diffusion_disease}The vector field in \eqref{eq:diffusion_disease} corresponding to $(a_1, a_2, b_1, b_2, c_1, c_2) = (.05,.1,.05,.1,1.,1.)$ together with a sample trajectory.}
  \end{minipage}
\end{figure}

Following our methodology in \cref{sec:learn-poly-vec}, we
parameterize our candidate vector field $p: \R^2 \rightarrow \R^2$ as
a polynomial of degree $d$, and we minimize the least square error
between the values taken by the vector fields $f$ and $p$ on the
observed trajectories; i.e., we solve the following convex
optimization problem:

\begin{equation}
  \min_{p \in \mathcal P_d} \sum_{(\ix_i, \iy_i) \in \mathcal D} \| p(\ix_i) - \iy_i\|^2.\label{eq:disease-fitting-polynomial-lsq}
\end{equation}

Note that the ground vector field $f$ is a polynomial of degree
$2$. In the following, we pretend that $f$ is unknown to us and we
consider an over-parameterized model of the truth by taking $d=3$.  To
help with the task of learning, we consider, the following list of side
information (that we can guess without knowing the exact structure
$f$). We also show that the imposing this side information leads to a
semidefinite programming constraints.

\begin{itemize}
\item {\bf Equilibrium point at the origin.} A disease cannot spread
  if no male or female is already infected. This corresponds to our
  vector field $p$ having an equilibrium at the origin, i.e.,
  $p(0, 0) = 0$. The is a simple linear constraint that we add to our
  optimization problem in \eqref{eq:disease-fitting-polynomial-lsq}.
  
\item {\bf Invariance of the box $[0, 1] \times [0, 1]$.} The
  components of a trajectory $\ix(t)$ following the dynamics in
  \eqref{eq:diffusion_disease} represents fractions, and as such, the
  vector $\ix(t)$ should be contained in the box
  $[0, 1] \times [0, 1]$ at all times $t \ge 0$. Mathematically, this
  corresponds to the constraints
  %
  \[p_2(x_1, 0) \ge 0, p_2(x_1, 1) \le 0 \quad \forall x_1 \in [0, 1],
    \quad p_1(0, x_2) \ge 0, p_2(1, x_2) \ge 0 \quad \forall x_2 \in
    [0, 1],\]
  %
  which imply that the vector field is pointing inwards on
  the boundaries of the unit box.
  % 
  Note that since
  $[0, 1] = \{ u \in \R \; | \; u \ge 0, 1-u \ge 0 \}$, the set
  $[0, 1]$ is closed semialgebraic. Following our discussion in
  \cref{sec:learn-poly-vec}, we replace these nonnegativity
  constraints with their corresponding Putinar's certificate in
  \eqref{eq:putinar-certificate} of degree two. For instance, we
  replace the constraint $p_2(x_1, 0) \ge 0$ with the linear
  constraints obtained from equating the coefficients of the two side
  of the polynomial equation
  $p_2(x_1, 0) = x_1s_0(x_1) + (1-x_1) s_1(x_1)$.  Here, the new
  decision variables $s_0$ and $s_1$ are (univariate) quadratic
  sum-of-squares polynomials.
  
\item {\bf Directional monotonicity.}
%
  We expect that, everything else being equal, if the fraction of
  males infected rises in the population, the rate of infection of
  females should increase. Mathematically, we can write
  \[\frac {\partial p_2}{\partial x_1}(\ix) \ge 0 \quad \forall \ix
    \in [0, 1]^2.\]
%
  Similarly, by changing the roles played by males and females, we
  obtain the constraint
    \[\frac {\partial p_1}{\partial x_2}(\ix) \ge 0 \quad \forall \ix
      \in [0, 1]^2.\]
%
    Note again that $[0, 1]^2$ is closed semialgebraic, so in the same
    spirit as the previous bullet point, we replace each one of these
    constraints with their corresponding Putinar's certificate of
    degree two.
\end{itemize}


We show in \cref{fig:disease-lsq-deg-3} the streamplot of the best
polynomial vector fields of degree $3$ obtained by solving the
least-squares problem in \eqref{eq:disease-fitting-polynomial-lsq} and
imposing some or all of the side information above.


\begin{figure}
  \subfigure[Least-squares\\ solution]{
    \includegraphics[width=.25\textwidth, trim=0 10 0 0, clip]{imgs/disease/deg_3_no_side_info.png}}~\;~
  \subfigure[Equilibrium at\\ the origin]{
    \includegraphics[width=.25\textwidth, trim=0 10 0 0, clip]{imgs/disease/deg_3_eq.png}}~\;~
  \subfigure[Equilibrium \\+ Invariance]{
    \includegraphics[width=.25\textwidth, trim=0 10 0 0, clip]{imgs/disease/deg_3_eq_invariance.png}}~\;~
  \subfigure[Equilibrium \\+ Invariance \\+ Monotonicity]{
    \includegraphics[width=.25\textwidth, trim=0 10 0 0, clip]{imgs/disease/deg_3_eq_invariance_monotone.png}}
  \caption{\label{fig:disease-lsq-deg-3}Streamplot of the best
  polynomial solution of degree 2 fitting the vector field $f$ defined
in \eqref{eq:diffusion_disease}}
\end{figure}


% \newcommand{\plotvfdisease}[2]{
%   \begin{minipage}[b]{.48\textwidth}
%     \begin{tikzpicture}[scale=.7]
%       \loadvf{data/disease/disease_segments_#1.csv}{data/disease/disease_arrows_#1.csv}
%       \begin{axis}[no markers, enlargelimits=false]
%         \boxtikz
%         %\draw[red, thick] (0, 0) circle (.3cm);
%         \plotsegmentsvf{}
%         \plotarrowsvf{}
%       \end{axis}
%   \end{tikzpicture}
%   \caption{#2}
%   \end{minipage}
% }
% \tikzsetnextfilename{disease_poly_deg_3_vf_pdf}
% \begin{figure}[H]
%   \centering
%   \plotvfdisease{deg_3_no_side_info}{\label{fig:deg-3-node-side-info}No
%   side information}~%
%   \plotvfdisease{deg_3_eq}{\label{fig:deg-3-eq}Equilibrium point at
%     the origin.}\\
%   \plotvfdisease{deg_3_eq_invariance}{\label{fig:deg-3-eq-invariance}Equilibrium point at the origin and invariance of the box $[0,1]\times[0,1]$.}~\plotvfdisease{deg_3_eq_invariance_monotone}{\label{fig:deg-3-eq-invariance-monotone}Equilibrium point at the origin, invariance of the box $[0,1]\times[0,1]$, and monotonicity.}
%   \caption{\label{fig:disease-lsq-deg-3}Streamplot of the best
%     polynomial vector fields of degree 3 solution to \eqref{eq:disease-fitting-polynomial-lsq} and satisfying additiona side information.}
% \end{figure}


\subsection{The simple pendulum}

\tikzsetnextfilename{simple_pendulum_pdf}
\begin{figure}[H]
  \centering
  \begin{minipage}[c]{.6\textwidth}
  \input{img/simple_pendulum.tikz}\quad\quad\quad\quad\quad\quad
  \includegraphics[width=.5\textwidth]{imgs/pendulum/pendulum_true_vf_with_data.png}
\end{minipage}
\begin{minipage}[c]{.3\textwidth}
  \caption{\label{fig:simple-pendulum}(Left) Simple pendulum. (Right) Phase portrait of the simple pendulum.}
\end{minipage}
\end{figure}

In this section we consider the simple pendulum system, i.e., a mass
$m$ hanging from a mass-less string of length $\ell$ and attached to a
fixed point $O$ (see \cref{fig:simple-pendulum}). By applying Newton's
second law for rotational systems, the equation of motion for the
pendulum may be obtained
\[ \ddot \theta = -\frac g\ell \sin \theta,\] where $g$ is is the
local acceleration of gravity.  This is a one-dimensional second-order
system. We convert it to a first-order system as follows.
\begin{equation}
\begin{pmatrix}\ddot \theta\\\dot \theta\end{pmatrix} =  f(\dot \theta, \theta) \coloneqq \begin{pmatrix}-\frac g\ell \sin \theta\\\dot \theta\end{pmatrix}.\label{eq:ode-pendulum}
\end{equation}


We take the vector field in \eqref{eq:ode-pendulum} to be the ground
truth with $g=\ell=1$, and we generate from it two noisy trajectories
$\theta_1$ and $\theta_2$ sampled at times $t_k = k/5$. More
precisely, we assume that we have the following data
\begin{equation}
  \mathcal D \coloneqq \left\{ (\ddot \theta_1(t_k), \dot \theta_1(t_k), \theta_1(t_k)) + 10^{-2} \varepsilon_k^1 \right\}_{k=0, \ldots, 5} \cup \left\{ (\ddot \theta_2(t_k), \dot \theta_2(t_k), \theta_2(t_k)) + 10^{-2} \varepsilon_k^2 \right\}_{k=0, \ldots, 5},\label{eq:data-pendulum}
\end{equation}
%
where the trajectory $\theta_1$ (resp. $\theta_2$) was obtained by
displacing the mass from to an initial angle $\frac \pi 3$ (resp.
$\frac{9\pi}{20}$) and released with a zero initial angular velocity,
and the $\varepsilon^i_k$ (for $i=1,2$ and $k=0,\ldots,5$) are
independent $3 \times 1$ normal vectors. The trajectories $\theta_1$
and $\theta_2$ together with the training data is plotted in
\cref{fig:trajectory-pendulum}.


We are interested in learning the vector field $f$ over the set
$\Omega = [-\pi, \pi]^2$ from the training data in
\eqref{eq:data-pendulum} and the side information below. We
parameterize our candidate vector field $p$ as a $\text{degree-}5$
polynomial.

\begin{itemize}
\item{\bf Hamiltonian.} The system in \eqref{eq:ode-pendulum} is {Hamiltonian}. Indeed,
  we assume that there is no dissipation of energy (through resistance
  of the air for example) so the total energy associated to the
  pendulum is conserved and is a Hamiltonian associated with the
  system.
  \begin{equation}
    E(\theta, \dot \theta) = \frac m2 {\dot \theta}^2 + \frac12 \frac gl (1 - \cos(\theta))\label{eq:total-energy-pendulum}
  \end{equation}
  The two terms appearing in the left can be interpreted physically as
  the kinetic energy and potential energy. Note that neither the
  vector field in \eqref{eq:ode-pendulum} describing the dynamics of
  the simple pendulum or the associated Hamiltonian in
  \eqref{eq:total-energy-pendulum} are polynomial functions.  In our
  learning procedure, we use only the fact that the system is
  Hamiltonian, i.e., that there exists a function $H$ such that
%
  \[ p_1(\dot \theta, \theta) = - \frac{\partial H}{\partial \dot
      \theta}(\dot \theta, \theta), \quad p_2(\dot \theta, \theta) =
    \frac{\partial H}{\partial \theta}(\dot \theta, \theta), \]
%
  but not the exact form of this Hamiltonian
  \eqref{eq:total-energy-pendulum}. Note that this is an affine
  constraint in the coefficients of the polynomial $p$.
  
\item {\bf Symmetry.} The pendulum system in \cref{fig:simple-pendulum} is symmetric
  with respect the vertical dotted axis. Then, our candidate vector
  field $p$ needs to satisfy the same symmetries.
  \[p(- \dot \theta, - \theta) = - p(\dot \theta, \theta) \quad
    \forall \theta, \dot \theta \in \R.\] Note that this is again an
  affine constraint in the coefficients of the polynomial $p$.
\item {\bf Coordinate nonnegativity.} The only external force applied on the pendulum system is gravitational force represented by the vector $g$ in \cref{fig:simple-pendulum}. This force pulls the mass down and pushes the angle $\theta$ towards $0$. In other terms, the angular velocity $\dot \theta$  decreases when $\theta$ is positive and increases when $\theta$ is negative. 
Mathematically,
\[p_2(\dot \theta, \theta) \le 0 \; \forall (\dot\theta,\theta) \in
  [-\pi, \pi] \times [0, \pi] \text{ and } p_2(\dot \theta, \theta)
  \ge 0 \; \forall (\dot\theta,\theta) \in [-\pi, \pi]\times [-\pi,
  0].\]
We replace each one of these constraints with their corresponding Putinar's certificate of degree $5$.
(Note that, because of symmetry, we actually only need to impose the first of these two constraints.)
\end{itemize}



\begin{figure}
  \subfigure[Least-squares solution]{
    \includegraphics[width=.25\textwidth, trim=0 10 0 0,
    clip]{imgs/pendulum/deg_5_sym_false_sign_false_hamiltonian_false.png}}~\;~
  \subfigure[Symmetry]{ \includegraphics[width=.25\textwidth,
    trim=0 10 0 0,
    clip]{imgs/pendulum/deg_5_sym_true_sign_false_hamiltonian_false.png}}~\;~
  \subfigure[Symmetry + Sign]{\includegraphics[width=.25\textwidth, trim=0 10 0 0,
    clip]{imgs/pendulum/deg_5_sym_true_sign_true_hamiltonian_false.png}}~\;~
  \subfigure[Symmetry \\+ Sign \\+ Hamiltonian]{\includegraphics[width=.25\textwidth, trim=0 10
    0
    0,clip]{imgs/pendulum/deg_5_sym_true_sign_false_hamiltonian_true.png}}
  
  \caption{\label{fig:simple-pendulum-learned-vf}Streamplots of learned vector fields of degree 5.}
\end{figure}

\input{imgs/pendulum/trajectory_pendulum.tikz}

%%% Local Variables:
%%% mode: latex
%%% TeX-engine: default
%%% TeX-master: "Learning_with_side_information_L4DC_v1"
%%% End:


==> data/tables/disease_10_samples.tex <==

\section*{Diffusion of a contagious diseas, degree = $2$}\\

\begin{tabular}{llrrrr|rrrr|rrrr}
\toprule
      & {} & \multicolumn{4}{l}{training error} & \multicolumn{4}{l}{test error (vector field)} & \multicolumn{4}{l}{test error (trajectories)} \\
      & \# side information: &         0 &     1 &     2 &     3 &        0 &     1 &     2 &     3 &     0 &     1 &     2 &     3 \\
noise & \# trajectories &           &       &       &       &          &       &       &       &       &       &       &       \\
\midrule
\multirow{4}{*}{0.001} & 1 &     0.001 & 0.001 & 0.001 & 0.001 &      219 &  4.42 & 0.863 &  0.09 &   $\infty$ &   $\infty$ & 0.048 &  0.01 \\
      & 2 &     0.001 & 0.001 & 0.002 & 0.002 &    0.061 & 0.019 & 0.076 & 0.076 & 0.004 & 0.002 & 0.005 & 0.005 \\
      & 3 &     0.001 & 0.001 & 0.002 & 0.002 &    0.015 & 0.016 & 0.083 & 0.083 & 0.002 & 0.002 & 0.006 & 0.006 \\
      & 4 &     0.001 & 0.001 & 0.002 & 0.002 &    0.006 & 0.006 & 0.065 & 0.074 &     0 &     0 & 0.002 & 0.003 \\
\cline{1-14}
\multirow{4}{*}{0.010} & 1 &     0.008 & 0.008 &  0.01 &  0.01 & 2.19e+03 &  44.2 &  1.08 & 0.098 &   $\infty$ &   $\infty$ & 0.095 & 0.012 \\
      & 2 &      0.01 &  0.01 &  0.01 &  0.01 &    0.612 & 0.191 & 0.148 &   0.1 & 0.044 &  0.02 & 0.017 & 0.012 \\
      & 3 &      0.01 &  0.01 &  0.01 &  0.01 &    0.147 & 0.159 & 0.129 &   0.1 & 0.015 & 0.015 & 0.012 &  0.01 \\
      & 4 &      0.01 &  0.01 &  0.01 &  0.01 &    0.063 & 0.056 & 0.082 & 0.086 & 0.003 & 0.003 & 0.004 & 0.004 \\
\cline{1-14}
\multirow{4}{*}{0.100} & 1 &     0.082 & 0.083 & 0.096 & 0.098 & 2.19e+04 &   442 &  6.15 & 0.588 &   $\infty$ &   $\infty$ & 0.675 & 0.097 \\
      & 2 &     0.095 & 0.096 & 0.098 & 0.098 &     6.12 &  1.91 & 0.548 & 0.302 &   $\infty$ & 0.197 & 0.076 & 0.053 \\
      & 3 &     0.097 & 0.097 & 0.099 & 0.099 &     1.47 &  1.58 & 0.345 &  0.34 &   $\infty$ &   $\infty$ & 0.021 & 0.022 \\
      & 4 &     0.098 & 0.098 &   0.1 &   0.1 &     0.63 & 0.557 & 0.233 & 0.229 &   $\infty$ &   $\infty$ &  0.01 & 0.009 \\
\bottomrule
\end{tabular}

\section*{Diffusion of a contagious diseas, degree = $3$}\\

\begin{tabular}{llrrrr|rrrr|rrrr}
\toprule
      & {} & \multicolumn{4}{l}{training error} & \multicolumn{4}{l}{test error (vector field)} & \multicolumn{4}{l}{test error (trajectories)} \\
      & \# side information: &         0 &     1 &     2 &     3 &        0 &        1 &        2 &     3 &    0 &    1 &     2 &     3 \\
noise & \# trajectories &           &       &       &       &          &          &          &       &      &      &       &       \\
\midrule
\multirow{4}{*}{0.001} & 1 &         0 &     0 & 0.001 & 0.001 & 3.08e+07 & 3.13e+06 &  3.2e+04 & 0.638 &  $\infty$ &  $\infty$ &   $\infty$ & 0.036 \\
      & 2 &     0.001 & 0.001 & 0.001 & 0.001 &     36.2 &     54.6 &    0.403 & 0.292 &  $\infty$ &  $\infty$ & 0.025 & 0.014 \\
      & 3 &     0.001 & 0.001 & 0.001 & 0.001 &     2.37 &     3.04 &    0.297 &  0.16 &  $\infty$ &  $\infty$ & 0.016 & 0.007 \\
      & 4 &     0.001 & 0.001 & 0.001 & 0.001 &    0.693 &    0.489 &    0.171 & 0.095 &  $\infty$ & 0.02 & 0.002 & 0.002 \\
\cline{1-14}
\multirow{4}{*}{0.010} & 1 &         0 & 0.002 & 0.008 & 0.009 & 3.08e+08 & 3.12e+07 & 3.14e+05 &  7.55 &  $\infty$ &  $\infty$ &   $\infty$ &  0.37 \\
      & 2 &     0.009 & 0.009 & 0.009 &  0.01 &      362 &      546 &     1.61 & 0.544 &  $\infty$ &  $\infty$ & 0.106 & 0.046 \\
      & 3 &     0.009 & 0.009 &  0.01 &  0.01 &     23.7 &     30.4 &    0.698 & 0.206 &  $\infty$ &  $\infty$ & 0.046 & 0.018 \\
      & 4 &      0.01 &  0.01 &  0.01 &  0.01 &     6.93 &     4.89 &    0.168 & 0.097 &  $\infty$ &  $\infty$ & 0.006 & 0.004 \\
\cline{1-14}
\multirow{4}{*}{0.100} & 1 &         0 & 0.024 & 0.077 & 0.093 & 3.08e+09 & 3.12e+08 & 2.48e+06 &  80.4 &  $\infty$ &  $\infty$ &   $\infty$ &  3.73 \\
      & 2 &     0.085 & 0.087 & 0.095 & 0.097 & 3.62e+03 & 5.46e+03 &     14.2 &  3.53 &  $\infty$ &  $\infty$ & 0.878 & 0.321 \\
      & 3 &     0.093 & 0.093 & 0.097 & 0.098 &      237 &      304 &     5.18 &  0.56 &  $\infty$ &  $\infty$ & 0.348 & 0.042 \\
      & 4 &     0.096 & 0.096 & 0.099 & 0.099 &     69.3 &     48.9 &     1.25 &  1.13 &  $\infty$ &  $\infty$ & 0.018 & 0.014 \\
\bottomrule
\end{tabular}

\section*{Diffusion of a contagious diseas, degree = $4$}\\

\begin{tabular}{llrrrr|rrrr|rrrr}
\toprule
      & {} & \multicolumn{4}{l}{training error} & \multicolumn{4}{l}{test error (vector field)} & \multicolumn{4}{l}{test error (trajectories)} \\
      & \# side information: &         0 &     1 &     2 &     3 &        0 &        1 &        2 &     3 &    0 &   1 &     2 &     3 \\
noise & \# trajectories &           &       &       &       &          &          &          &       &      &     &       &       \\
\midrule
\multirow{4}{*}{0.001} & 1 &     0.001 & 0.001 & 0.001 & 0.001 & 4.85e+03 & 4.57e+03 & 4.66e+03 &  4.56 &  $\infty$ & $\infty$ &   $\infty$ & 0.112 \\
      & 2 &     0.001 & 0.001 & 0.001 & 0.001 & 1.32e+03 & 1.39e+04 &     82.1 &  2.55 &  $\infty$ & $\infty$ &  1.97 & 0.041 \\
      & 3 &     0.001 & 0.001 & 0.001 & 0.001 & 1.56e+03 & 1.38e+03 &     3.31 &  1.58 &  $\infty$ & $\infty$ & 0.091 & 0.022 \\
      & 4 &     0.001 & 0.001 & 0.001 & 0.001 &     29.2 &     20.2 &        3 & 0.254 &  $\infty$ & $\infty$ & 0.018 & 0.001 \\
\cline{1-14}
\multirow{4}{*}{0.010} & 1 &     0.006 & 0.006 & 0.007 & 0.009 &    4e+04 & 4.44e+04 & 4.34e+04 &  56.8 &  $\infty$ & $\infty$ &   $\infty$ & 0.796 \\
      & 2 &     0.008 & 0.007 & 0.008 & 0.009 & 1.32e+04 & 1.39e+05 &      751 &  12.1 &  $\infty$ & $\infty$ &  18.1 & 0.295 \\
      & 3 &     0.009 & 0.009 & 0.009 & 0.009 & 1.56e+04 & 1.38e+04 &     20.8 &  7.05 &  $\infty$ & $\infty$ & 0.175 & 0.127 \\
      & 4 &     0.009 & 0.009 &  0.01 &  0.01 &      292 &      202 &     4.67 & 0.704 &  $\infty$ & $\infty$ & 0.017 & 0.004 \\
\cline{1-14}
\multirow{4}{*}{0.100} & 1 &     0.057 & 0.057 & 0.065 & 0.091 & 3.44e+05 & 3.12e+05 & 4.69e+05 &   574 &  $\infty$ & $\infty$ &   $\infty$ &  7.67 \\
      & 2 &     0.076 & 0.067 & 0.082 & 0.095 & 1.32e+05 & 1.39e+06 & 7.35e+03 &  51.6 &  $\infty$ & $\infty$ &   $\infty$ &  2.03 \\
      & 3 &     0.085 & 0.087 & 0.094 & 0.096 & 1.56e+05 & 1.38e+05 &      205 &  40.5 &  $\infty$ & $\infty$ &  1.46 &  1.22 \\
      & 4 &     0.093 & 0.093 & 0.098 & 0.098 & 2.92e+03 & 2.02e+03 &     16.1 &  6.19 &  $\infty$ & $\infty$ & 0.068 & 0.019 \\
\bottomrule
\end{tabular}



==> data/tables/disease_20_samples.tex <==

\section*{Diffusion of a contagious diseas, degree = $2$}\\

\begin{tabular}{llrrrr|rrrr|rrrr}
\toprule
      & {} & \multicolumn{4}{l}{training error} & \multicolumn{4}{l}{test error (vector field)} & \multicolumn{4}{l}{test error (trajectories)} \\
      & \# side information: &         0 &     1 &     2 &     3 &        0 &     1 &     2 &     3 &     0 &     1 &     2 &     3 \\
noise & \# trajectories &           &       &       &       &          &       &       &       &       &       &       &       \\
\midrule
\multirow{3}{*}{0.001} & 1 &     0.001 & 0.001 & 0.001 & 0.001 &      189 &  1.42 & 0.432 & 0.068 &   $\infty$ &   $\infty$ & 0.045 & 0.008 \\
      & 2 &     0.001 & 0.001 & 0.002 & 0.002 &    0.044 & 0.023 & 0.081 & 0.081 & 0.004 & 0.002 & 0.005 & 0.005 \\
      & 3 &     0.001 & 0.001 & 0.002 & 0.002 &    0.018 & 0.018 & 0.083 & 0.083 & 0.002 & 0.002 & 0.005 & 0.005 \\
\cline{1-14}
\multirow{3}{*}{0.010} & 1 &     0.008 & 0.008 & 0.008 & 0.009 & 1.89e+03 &  14.2 &   1.3 & 0.071 &   $\infty$ &   $\infty$ & 0.129 & 0.012 \\
      & 2 &     0.008 & 0.008 & 0.009 & 0.009 &    0.444 & 0.233 & 0.062 & 0.061 & 0.031 &   $\infty$ & 0.006 & 0.004 \\
      & 3 &     0.009 & 0.009 & 0.009 & 0.009 &    0.179 &  0.18 & 0.075 & 0.074 &   $\infty$ &   $\infty$ & 0.007 & 0.006 \\
\cline{1-14}
\multirow{3}{*}{0.100} & 1 &      0.08 & 0.082 & 0.085 & 0.087 & 1.89e+04 &   142 &  8.08 & 0.075 &   $\infty$ &   $\infty$ & 0.665 &  0.02 \\
      & 2 &     0.085 & 0.085 & 0.087 & 0.088 &     4.44 &  2.33 & 0.077 & 0.068 &   $\infty$ &   $\infty$ & 0.021 & 0.019 \\
      & 3 &     0.086 & 0.086 & 0.088 & 0.088 &     1.78 &   1.8 & 0.088 &  0.11 &   $\infty$ &   $\infty$ & 0.019 & 0.016 \\
\bottomrule
\end{tabular}

\section*{Diffusion of a contagious diseas, degree = $3$}\\

\begin{tabular}{llrrrr|rrrr|rrrr}
\toprule
      & {} & \multicolumn{4}{l}{training error} & \multicolumn{4}{l}{test error (vector field)} & \multicolumn{4}{l}{test error (trajectories)} \\
      & \# side information: &         0 &     1 &     2 &     3 &        0 &        1 &        2 &     3 &    0 &     1 &     2 &     3 \\
noise & \# trajectories &           &       &       &       &          &          &          &       &      &       &       &       \\
\midrule
\multirow{3}{*}{0.001} & 1 &     0.001 & 0.001 & 0.001 & 0.001 &      229 &      363 &      497 &  4.22 &  $\infty$ &   $\infty$ &  12.3 & 0.065 \\
      & 2 &     0.001 & 0.001 & 0.001 & 0.001 &     21.8 &     22.2 &    0.221 & 0.248 &  $\infty$ &   $\infty$ &  0.01 & 0.005 \\
      & 3 &     0.001 & 0.001 & 0.001 & 0.001 &     1.65 &     2.15 &    0.141 & 0.151 &  $\infty$ & 0.026 & 0.003 & 0.004 \\
\cline{1-14}
\multirow{3}{*}{0.010} & 1 &     0.008 & 0.008 & 0.008 & 0.008 & 2.29e+03 & 3.63e+03 & 4.86e+03 &  43.4 &  $\infty$ &   $\infty$ &   $\infty$ & 0.581 \\
      & 2 &     0.008 & 0.008 & 0.008 & 0.009 &      218 &      222 &     1.92 &  0.47 &  $\infty$ &   $\infty$ & 0.081 & 0.013 \\
      & 3 &     0.008 & 0.008 & 0.009 & 0.009 &     16.5 &     21.5 &     0.47 & 0.292 &  $\infty$ & 0.251 & 0.008 & 0.007 \\
\cline{1-14}
\multirow{3}{*}{0.100} & 1 &     0.079 & 0.079 &  0.08 & 0.084 & 2.29e+04 & 3.63e+04 &  4.2e+04 &   435 &  $\infty$ &   $\infty$ &   $\infty$ &   5.8 \\
      & 2 &     0.082 & 0.083 & 0.085 & 0.087 & 2.18e+03 & 2.22e+03 &     15.9 &  2.64 &  $\infty$ &   $\infty$ & 0.662 & 0.079 \\
      & 3 &     0.084 & 0.084 & 0.086 & 0.087 &      165 &      215 &     3.12 & 0.982 &  $\infty$ &   $\infty$ & 0.052 & 0.023 \\
\bottomrule
\end{tabular}

\section*{Diffusion of a contagious diseas, degree = $4$}\\

\begin{tabular}{llrrrr|rrrr|rrrr}
\toprule
      & {} & \multicolumn{4}{l}{training error} & \multicolumn{4}{l}{test error (vector field)} & \multicolumn{4}{l}{test error (trajectories)} \\
      & \# side information: &         0 &     1 &     2 &     3 &        0 &        1 &        2 &        3 &    0 &   1 &     2 &     3 \\
noise & \# trajectories &           &       &       &       &          &          &          &          &      &     &       &       \\
\midrule
\multirow{3}{*}{0.001} & 1 &     0.001 & 0.001 & 0.001 & 0.001 & 1.63e+04 &      831 &      232 &     21.7 &  $\infty$ & $\infty$ &  14.6 & 0.092 \\
      & 2 &     0.001 & 0.001 & 0.001 & 0.001 & 2.58e+03 &      407 &     39.7 &    0.726 &  $\infty$ & $\infty$ & 0.097 & 0.004 \\
      & 3 &     0.001 & 0.001 & 0.001 & 0.001 &      421 &      393 &     15.2 &    0.575 &  $\infty$ & $\infty$ & 0.107 & 0.002 \\
\cline{1-14}
\multirow{3}{*}{0.010} & 1 &     0.008 & 0.008 & 0.008 & 0.008 & 1.62e+05 & 8.31e+03 &  1.6e+03 &      191 &  $\infty$ & $\infty$ &   $\infty$ & 0.822 \\
      & 2 &     0.008 & 0.008 & 0.008 & 0.009 & 2.58e+04 & 4.07e+03 &      300 &     1.83 &  $\infty$ & $\infty$ &  1.12 & 0.046 \\
      & 3 &     0.008 & 0.008 & 0.008 & 0.009 & 4.21e+03 & 3.93e+03 &      162 &     1.53 &  $\infty$ & $\infty$ & 0.792 & 0.031 \\
\cline{1-14}
\multirow{3}{*}{0.100} & 1 &     0.076 & 0.075 &  0.08 & 0.083 & 1.57e+06 & 8.31e+04 & 1.63e+04 & 1.92e+03 &  $\infty$ & $\infty$ &   $\infty$ &  8.22 \\
      & 2 &     0.079 & 0.079 & 0.082 & 0.087 & 2.58e+05 & 4.07e+04 & 2.91e+03 &     8.01 &  $\infty$ & $\infty$ &  11.9 & 0.018 \\
      & 3 &     0.081 & 0.082 & 0.084 & 0.087 & 4.21e+04 & 3.93e+04 & 1.77e+03 &     7.99 &  $\infty$ & $\infty$ &  6.31 & 0.017 \\
\bottomrule
\end{tabular}


==> data/tables/lorenz_10_samples.tex <==

\section*{Lorentz, degree = $2$}\\

\begin{tabular}{llrrrr|rrrr|rrrr}
\toprule
      & {} & \multicolumn{4}{l}{training error} & \multicolumn{4}{l}{test error (vector field)} & \multicolumn{4}{l}{test error (trajectories)} \\
      & \# side information: &         0 &     1 &     2 &     3 &     0 &     1 &     2 &     3 &     0 &     1 &     2 &     3 \\
noise & \# trajectories &           &       &       &       &       &       &       &       &       &       &       &       \\
\midrule
\multirow{4}{*}{0.001} & 1 &        -0 &     0 &     0 & 0.001 &  0.49 & 0.208 &  0.17 & 0.003 &  1.04 & 0.235 & 0.134 & 0.003 \\
      & 2 &     0.001 & 0.001 & 0.001 & 0.001 & 0.003 & 0.002 & 0.002 & 0.001 & 0.005 & 0.005 & 0.004 & 0.003 \\
      & 3 &     0.001 & 0.001 & 0.001 & 0.001 & 0.002 & 0.001 & 0.002 & 0.001 & 0.004 & 0.003 & 0.003 & 0.003 \\
      & 4 &     0.001 & 0.001 & 0.001 & 0.001 & 0.001 & 0.001 & 0.001 & 0.001 & 0.003 & 0.002 & 0.002 & 0.002 \\
\cline{1-14}
\multirow{4}{*}{0.010} & 1 &        -0 & 0.003 & 0.004 & 0.007 &   4.9 &  2.08 &   1.7 & 0.027 &   9.8 &  2.31 &  1.33 & 0.033 \\
      & 2 &     0.007 & 0.007 & 0.007 & 0.008 &  0.03 & 0.024 & 0.021 & 0.011 & 0.053 & 0.049 & 0.047 & 0.025 \\
      & 3 &     0.007 & 0.007 & 0.007 & 0.008 & 0.024 & 0.013 & 0.015 & 0.006 & 0.041 &  0.03 & 0.027 & 0.027 \\
      & 4 &     0.007 & 0.007 & 0.007 & 0.008 & 0.011 & 0.008 & 0.008 & 0.006 & 0.027 & 0.025 & 0.023 & 0.023 \\
\cline{1-14}
\multirow{4}{*}{0.100} & 1 &        -0 & 0.026 & 0.043 & 0.074 &    49 &  20.8 &    17 & 0.267 &  55.8 &  19.9 &  13.4 & 0.331 \\
      & 2 &     0.066 & 0.068 & 0.071 & 0.078 & 0.297 &  0.24 & 0.214 & 0.109 & 0.533 & 0.487 & 0.466 & 0.243 \\
      & 3 &     0.071 & 0.073 & 0.074 & 0.079 & 0.237 & 0.128 & 0.158 & 0.065 & 0.412 & 0.302 & 0.273 & 0.271 \\
      & 4 &     0.071 & 0.072 & 0.074 & 0.079 & 0.113 & 0.082 & 0.076 & 0.064 & 0.274 & 0.247 &  0.23 & 0.212 \\
\bottomrule
\end{tabular}

\section*{Lorentz, degree = $3$}\\

\begin{tabular}{llrrrr|rrrr|rrrr}
\toprule
      & {} & \multicolumn{4}{l}{training error} & \multicolumn{4}{l}{test error (vector field)} & \multicolumn{4}{l}{test error (trajectories)} \\
      & \# side information: &         0 &     1 &     2 &     3 &     0 &     1 &     2 &        3 &     0 &     1 &     2 &     3 \\
noise & \# trajectories &           &       &       &       &       &       &       &          &       &       &       &       \\
\midrule
\multirow{4}{*}{0.001} & 1 &         0 &     0 &     0 &     0 &   165 &   165 &   157 &      267 &   $\infty$ &   $\infty$ &   $\infty$ &   $\infty$ \\
      & 2 &         0 &     0 &     0 &     0 &  3.64 &  3.17 &  30.4 &    0.076 &  1.34 & 0.758 &  5.57 & 0.022 \\
      & 3 &     0.001 & 0.001 &     0 &     0 &  0.25 & 0.157 & 0.851 &    0.019 & 0.058 & 0.026 & 0.219 & 0.022 \\
      & 4 &     0.001 & 0.001 & 0.001 & 0.001 &  0.01 & 0.006 &  0.03 &    0.009 & 0.004 & 0.003 & 0.018 & 0.005 \\
\cline{1-14}
\multirow{4}{*}{0.010} & 1 &         0 &     0 & 0.003 & 0.003 &   166 &   166 &   158 & 1.09e+03 &   $\infty$ &   $\infty$ &   $\infty$ &   $\infty$ \\
      & 2 &         0 & 0.003 & 0.004 & 0.005 &  37.7 &  31.4 &  34.6 &    0.521 &  10.7 &  8.51 &  7.79 & 0.402 \\
      & 3 &     0.006 & 0.006 & 0.006 & 0.006 &   2.5 &  1.57 &  1.46 &    0.049 & 0.577 & 0.258 & 0.242 &  0.07 \\
      & 4 &     0.006 & 0.006 & 0.007 & 0.007 & 0.098 & 0.065 &  0.04 &     0.03 & 0.042 &  0.03 & 0.034 & 0.034 \\
\cline{1-14}
\multirow{4}{*}{0.100} & 1 &         0 &     0 & 0.039 & 0.038 &   168 &   168 &   160 &      668 &   $\infty$ &   $\infty$ &   $\infty$ &   $\infty$ \\
      & 2 &         0 & 0.035 & 0.046 & 0.058 &   375 &   312 &   338 &     9.38 &   $\infty$ &   $\infty$ &   $\infty$ &  8.25 \\
      & 3 &      0.06 & 0.062 & 0.066 & 0.069 &    25 &  15.7 &    15 &    0.542 &  5.49 &  2.61 &  2.71 & 0.616 \\
      & 4 &     0.064 & 0.065 & 0.068 & 0.069 & 0.985 & 0.648 &  0.37 &    0.234 & 0.419 & 0.306 & 0.349 & 0.313 \\
\bottomrule
\end{tabular}

\section*{Lorentz, degree = $4$}\\

\begin{tabular}{llrrrr|rrrr|rrrr}
\toprule
      & {} & \multicolumn{4}{l}{training error} & \multicolumn{4}{l}{test error (vector field)} & \multicolumn{4}{l}{test error (trajectories)} \\
      & \# side information: &         0 &     1 &     2 &     3 &        0 &        1 &        2 &       3 &     0 &    1 &   2 &     3 \\
noise & \# trajectories &           &       &       &       &          &          &          &         &       &      &     &       \\
\midrule
\multirow{4}{*}{0.001} & 1 &         0 &     0 &     0 &     0 &      118 &      118 &      108 & 1.1e+03 &   $\infty$ &  $\infty$ & $\infty$ &   134 \\
      & 2 &         0 &     0 &     0 &     0 &      579 &      580 &      570 &    98.8 &   $\infty$ &  $\infty$ & $\infty$ &  25.3 \\
      & 3 &         0 &     0 &     0 &     0 &      934 &      919 & 9.81e+03 &    0.95 &   $\infty$ &  140 & $\infty$ & 0.389 \\
      & 4 &         0 &     0 &     0 &     0 &     9.23 &     8.32 & 1.91e+03 &   0.094 & 0.968 & 1.03 & $\infty$ & 0.236 \\
\cline{1-14}
\multirow{4}{*}{0.010} & 1 &         0 &     0 &     0 &     0 &      118 &      118 &      108 &     587 &   $\infty$ &  $\infty$ & $\infty$ &   109 \\
      & 2 &         0 &     0 &     0 &     0 &      576 &      577 &      567 &     214 &   $\infty$ &  $\infty$ & $\infty$ &  46.3 \\
      & 3 &         0 &     0 & 0.002 & 0.002 &      972 &      948 &  2.7e+03 &    2.17 &   $\infty$ &  $\infty$ & 243 &  1.35 \\
      & 4 &     0.004 & 0.004 & 0.001 & 0.004 &     92.3 &     83.2 & 1.66e+03 &   0.657 &   $\infty$ &  $\infty$ & $\infty$ & 0.378 \\
\cline{1-14}
\multirow{4}{*}{0.100} & 1 &         0 &     0 &     0 &     0 &      118 &      118 &      111 &     966 &   $\infty$ &  $\infty$ & $\infty$ &   126 \\
      & 2 &         0 &     0 & 0.008 & 0.037 &      554 &      555 &      544 &     152 &   177 &  177 & 168 &  28.2 \\
      & 3 &         0 &     0 &  0.03 &  0.05 & 1.29e+03 & 1.27e+03 & 1.81e+03 &    17.9 &   $\infty$ &  $\infty$ & 200 &  3.46 \\
      & 4 &     0.039 &  0.04 & 0.035 & 0.054 &      923 &      832 & 8.92e+03 &    2.84 &   $\infty$ &  $\infty$ & $\infty$ &  1.07 \\
\bottomrule
\end{tabular}


==> data/tables/lorenz_20_samples.tex <==

\section*{Lorentz, degree = $2$}\\

\begin{tabular}{llrrrr|rrrr|rrrr}
\toprule
      & {} & \multicolumn{4}{l}{training error} & \multicolumn{4}{l}{test error (vector field)} & \multicolumn{4}{l}{test error (trajectories)} \\
      & \# side information: &         0 &     1 &     2 &     3 &     0 &     1 &     2 &     3 &     0 &     1 &     2 &     3 \\
noise & \# trajectories &           &       &       &       &       &       &       &       &       &       &       &       \\
\midrule
\multirow{3}{*}{0.001} & 1 &     0.001 & 0.001 & 0.001 & 0.001 & 0.049 & 0.003 & 0.003 & 0.001 & 0.028 & 0.003 & 0.002 & 0.002 \\
      & 2 &     0.001 & 0.001 & 0.001 & 0.001 & 0.002 & 0.002 & 0.002 & 0.001 & 0.002 & 0.002 & 0.001 & 0.001 \\
      & 3 &     0.001 & 0.001 & 0.001 & 0.001 & 0.002 & 0.001 & 0.001 & 0.001 & 0.003 & 0.002 & 0.002 & 0.001 \\
\cline{1-14}
\multirow{3}{*}{0.010} & 1 &     0.007 & 0.007 & 0.008 & 0.008 & 0.491 &  0.03 & 0.029 & 0.009 & 0.285 & 0.033 & 0.028 & 0.018 \\
      & 2 &     0.008 & 0.008 & 0.008 & 0.009 &  0.02 & 0.018 & 0.018 & 0.007 & 0.018 & 0.019 & 0.016 & 0.008 \\
      & 3 &     0.008 & 0.008 & 0.008 & 0.009 & 0.018 & 0.014 & 0.013 & 0.007 & 0.025 & 0.018 & 0.019 & 0.005 \\
\cline{1-14}
\multirow{3}{*}{0.100} & 1 &     0.068 & 0.073 & 0.077 & 0.083 &  4.91 & 0.304 &  0.28 &  0.09 &  3.01 &  0.33 & 0.263 &  0.17 \\
      & 2 &     0.079 & 0.079 & 0.081 & 0.086 & 0.202 & 0.177 & 0.172 & 0.074 & 0.185 & 0.187 & 0.154 & 0.064 \\
      & 3 &     0.083 & 0.084 & 0.085 & 0.088 & 0.185 & 0.142 & 0.135 & 0.071 & 0.251 & 0.184 & 0.194 & 0.052 \\
\bottomrule
\end{tabular}

\section*{Lorentz, degree = $3$}\\

\begin{tabular}{llrrrr|rrrr|rrrr}
\toprule
      & {} & \multicolumn{4}{l}{training error} & \multicolumn{4}{l}{test error (vector field)} & \multicolumn{4}{l}{test error (trajectories)} \\
      & \# side information: &         0 &     1 &     2 &     3 &        0 &     1 &     2 &     3 &     0 &     1 &     2 &     3 \\
noise & \# trajectories &           &       &       &       &          &       &       &       &       &       &       &       \\
\midrule
\multirow{3}{*}{0.001} & 1 &         0 &     0 & 0.001 &     0 &      110 &   207 &    66 &  10.9 &   $\infty$ &   $\infty$ &   $\infty$ &  13.7 \\
      & 2 &     0.001 & 0.001 & 0.001 & 0.001 &    0.046 & 0.025 & 0.043 & 0.008 & 0.016 & 0.008 & 0.033 & 0.005 \\
      & 3 &     0.001 & 0.001 & 0.001 & 0.001 &    0.014 & 0.009 & 0.037 & 0.044 & 0.006 & 0.008 & 0.022 & 0.034 \\
\cline{1-14}
\multirow{3}{*}{0.010} & 1 &     0.003 & 0.003 & 0.005 & 0.005 &      192 &   187 &   226 &  10.9 &  57.9 &  61.6 &   $\infty$ &  14.2 \\
      & 2 &     0.006 & 0.006 & 0.007 & 0.007 &    0.461 & 0.251 & 0.256 & 0.063 & 0.157 & 0.084 & 0.164 &  0.05 \\
      & 3 &     0.008 & 0.008 & 0.008 & 0.008 &    0.138 & 0.094 & 0.133 & 0.035 & 0.058 & 0.076 & 0.062 & 0.019 \\
\cline{1-14}
\multirow{3}{*}{0.100} & 1 &     0.032 & 0.033 &  0.05 & 0.057 & 1.47e+03 &   516 &   664 &  54.9 &   237 &   $\infty$ &   $\infty$ &  23.6 \\
      & 2 &     0.064 & 0.065 & 0.068 & 0.071 &     4.61 &  2.51 &  2.25 & 0.963 &  1.59 & 0.899 &  1.46 & 0.461 \\
      & 3 &     0.075 & 0.076 & 0.078 & 0.078 &     1.38 & 0.943 & 0.787 & 0.352 & 0.576 &  0.77 & 0.525 & 0.279 \\
\bottomrule
\end{tabular}

\section*{Lorentz, degree = $4$}\\

\begin{tabular}{llrrrr|rrrr|rrrr}
\toprule
      & {} & \multicolumn{4}{l}{training error} & \multicolumn{4}{l}{test error (vector field)} & \multicolumn{4}{l}{test error (trajectories)} \\
      & \# side information: &         0 &     1 &     2 &     3 &        0 &        1 &        2 &        3 &     0 &     1 &    2 &     3 \\
noise & \# trajectories &           &       &       &       &          &          &          &          &       &       &      &       \\
\midrule
\multirow{3}{*}{0.001} & 1 &         0 &     0 &     0 &     0 &      167 &      243 & 9.29e+03 &      532 &  82.7 &   $\infty$ &  $\infty$ &  94.4 \\
      & 2 &         0 &     0 &     0 &     0 &     46.1 &       11 &      768 &    0.479 &  51.8 &  8.13 &  $\infty$ & 0.832 \\
      & 3 &     0.001 & 0.001 &     0 &     0 &    0.283 &    0.199 &     84.6 &    0.205 & 0.047 & 0.048 & 11.1 & 0.421 \\
\cline{1-14}
\multirow{3}{*}{0.010} & 1 &         0 &     0 &     0 & 0.001 &      858 & 1.08e+03 & 4.66e+04 & 6.22e+03 &   $\infty$ &   $\infty$ &  $\infty$ &   286 \\
      & 2 &     0.003 & 0.004 &     0 & 0.004 &      461 &      110 & 1.47e+03 &     1.71 &   $\infty$ &  48.4 &  $\infty$ &  1.97 \\
      & 3 &     0.006 & 0.006 & 0.002 & 0.005 &     2.83 &     1.99 &     99.5 &    0.407 & 0.468 & 0.486 &  $\infty$ & 0.179 \\
\cline{1-14}
\multirow{3}{*}{0.100} & 1 &         0 &     0 & 0.009 & 0.031 & 8.92e+03 & 8.93e+03 & 1.55e+05 & 2.55e+03 &   $\infty$ &   $\infty$ &  $\infty$ &   120 \\
      & 2 &     0.028 & 0.038 & 0.041 & 0.057 & 4.61e+03 &  1.1e+03 & 4.54e+03 &     6.21 &   $\infty$ &   $\infty$ &  $\infty$ &  5.15 \\
      & 3 &     0.061 & 0.062 & 0.053 & 0.069 &     28.3 &     19.9 &     87.1 &     2.47 &  4.84 &  4.93 &  $\infty$ & 0.939 \\
\bottomrule
\end{tabular}


==> introduction.tex <==
\section{Introduction}
Our goal is to learn a dynamical system from a {limited}
number of {noisy} measurements of its
trajectories. Imagine, e.g., a passenger airplane that has
gone through sudden structural damage. Can we learn the new
dynamics on the fly so to autonomously land the plane?
Since data is scarce, side information (e.g., physical
laws/contextual knowledge) must be exploited. For instance,
we may know when the engines are off, the plane cannot
accelerate upwards, or some bounds on the velocities of all
the states.


% \begin{figure}\centering
%   \includegraphics[scale=.5]{airplane_example.png}
%   \caption{Caption}
% \end{figure}

% \begin{figure}\centering
%   \includegraphics[scale=.25]{sample_trajectories.png}
%   \caption{Sample trajectories.}
% \end{figure}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "Learning_with_side_information_L4DC_v1"
%%% End:


==> old_theorems.tex <==
\begin{theorem}\label{thm:sdp_finds_best_poly}
  Fix a degree $d$, training data $\mathcal D$ and a
  combination of side information $S_1, \ldots, S_m$ (where
  every $S_i$ is of the type in \cref{sec:side-info}). Let
  $\mathcal G \coloneqq \poly d \cap S_1 \cap \ldots \cap
  S_,$. Suppose that (i) the minimum value of training error 
  \[\sum_{(\x_i, \iy_i) \in \mathcal D}
    \ell(p(\x_i), \iy_i),\] over $\mathcal G$ is attained by
  $p^* \in \poly d$, and that (ii) $p^*$ satisfies the side
  information $S_1,\ldots,S_m$ strictly, then for $r$ large
  enough, the optimal value of the semidefinite
  program below gives a polynomial vector field that satisfies the
  side information $S_1, \ldots, S_m$ and gives the same
  training error as $p^*$.

  \begin{equation}
    \label{eq:learn_poly_vf_as_sdp}
    \begin{split}
    \min_{p \in \mathcal F}&
    \sum_{(\x_i, \iy_i) \in \mathcal D}
    \ell(p(\x_i), \iy_i)\\
    &p \in S_i^{(r)} \quad \text{for $i=1,\ldots,m$}.
    \end{split}
  \end{equation}
  
\end{theorem}

\begin{remark}
  Denote by $p$ the polynomial
  $x_1^4x_2^2 + x_1^2x_2^4 + x_3^6 - 3x_1^2x_2^2x_3^2,$
  known as the Motzkin polynomial, and let
  $g(x_1, x_2, x_3) \coloneqq 1 - (x_1^2 + x_2^2 + x_3^2)$.
  The polynomial $p$ is nonnegative on the unit ball
  \(\SETALG \coloneqq \{x \in \mathbb R^3 \; | \; g(x) \ge
  0\},\) yet there exists no certificate of the form in
  \cref{eq:putinar-certificate} to prove it, i.e., there
  exist no sum of squares $s_0$ and $s_1$ that satisfy
  $p = s_0 + s_1 g$ 
  (see \cite{motzkin_not_sos_ball_nie_2013}). This shows that the
  assumption that $p$ be positive (and not simply
  nonnegative) is truly needed for the result of
  \cref{th:putinar} to hold. We can use this observation to
  show that assumption (ii) in
  \cref{thm:sdp_finds_best_poly} is needed. Indeed, take
  $n=3$, $d=3$, and $S_1 = \INTERPOLATION{\{x_i, f(x_i)\}}$,
  then $S_1 \cap \poly 3 = \{ f \}$ but $S_1^{(r)} \cap \poly 3 = \emptyset$ for any integer $r$.

  
  
\end{remark}



\subsection{Polynomail approximation of continuously-differentiable vector fields}
\begin{theorem}
  Fix a compact set $\Omega \subset R^n$, a time horizon $T > 0$, and a desired accuracy $\varepsilon > 0$. Let $f: \mathbb R^n \rightarrow \mathbb R^n$ be a continuous differentiable vector field that satisfies any one of the following constraints
(i) equilibria at a given finite set of points,
(ii) invariance of a set satisfying (*) in \cref{def:strict_convex_set},
(iii) directional monotonicity,
(iv) nonnegativity,
(v) gradient or Hamiltonian structure,
(vi) sign symmetry.
Then there exists a polynomial vector field $p: \mathbb R^n \rightarrow \R^n$ such that
\[\metricdyn{f-g}{\Omega}{T} \le \varepsilon,\]
and $p$ satisfies the same side information as $f$. Furthermore, all such properties of $p$ come with an SOS certificate.
\end{theorem}


\begin{theorem}
  Fix a compact set $\Omega \subset R^n$, a time horizon $T > 0$, a desired accuracy $\varepsilon > 0$, and a room of error $\delta$. Let $f: \mathbb R^n \rightarrow \mathbb R^n$ be a continuous differentiable vector field that satisfies any \textit{combination} of the following constraints
(i) equilibria at a given finite set of points,
(ii) invariance of a set satisfying (*) in \cref{def:strict_convex_set}.
(iii) directional monotonicity,
(iv) nonnegativity,
(v) gradient or Hamiltonian structure,
(vi) sign symmetry.
Then there exists a polynomial vector field $p: \mathbb R^n \rightarrow R^n$ such that
\[\metricdyn{f-g}{\Omega}{T} \le \delta,\]
and $p$ $\delta\text{-satisfies}$ the same side information as $f$. Furthermore, all such properties of $p$ come with an SOS certificate.
\end{theorem}


\begin{definition}\label[definition]{def:strict_convex_set}
A set is said to satisfy (*) if (i) it is defined by finitely many inequalities $h_i(x) \ge 0$, where the $h_i$ are convex functions, and (ii) there exists $x_* \in \R^n$ such that $h_i(x_*) > 0 \; \forall i$.
\end{definition}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "Learning_with_side_information_L4DC_v1"
%%% End:


==> open_problems.tex <==
\section{Open Problems}
\begin{itemize}
\item Is it true that every semi-algebraic set can be made invariant by a non-zero polynomial vector field?
\item How about PDEs?
\item Statistical questions
\item Other side information than the one considered here? Non-convex side info?
\end{itemize}


%%% Local Variables:
%%% mode: latex
%%% TeX-engine: luatex
%%% TeX-master: "Learning_with_side_information_v1"
%%% End:


==> polynomial_vf.tex <==
\section{Learning Polynomial Vector Fields}


Let $S$ be a side information. A positive result is when $S \cap
\mathcal F$ is dense in $S$, otherwise, it is negative.

We summarize the results in the following table
%\def\checkmark{\tikz\fill[scale=0.4](0,.35) -- (.25,0) -- (1,.7) -- (.25,.15) -- cycle;} 
\newcommand{\Cross}{\ding{55}}%
\newcommand{\Checkmark}{$\color{black}\checkmark$}
\newcommand{\Unknownmark}{$\textbf{\color{red}??}$}

\begin{table}[H]
  \centering
  \begin{tabular}{l|c|c|c|c}
                  & nonnegativity & monotonicity & invariance   & Hamiltonian  \\
    \hline          
    interpolation & \Checkmark (if     & \Cross       & \Unknownmark & \Unknownmark \\
    nonnegativity &               & \Checkmark   & \Cross       & \Checkmark   \\ 
    monotonicity  &               &              & \Cross       & \Unknownmark \\
    invariance    &               &              &              & \Unknownmark \\
  \end{tabular}
  \caption{Which side information can be combined}
  \label{tab:summary-combine-side-info}
\end{table}

\begin{theorem}
  Let $S$ denote one of the sets below.  Then , the set $S$ at least
  one non-zero, continuously-differentiable vector field, and yet, the
  only polynomial vector field in $S$ is the identically zero vector field.
  \begin{itemize}
  \item $\INV{\Omega}$, where
    $\Omega \coloneqq \{ \frac1{2k\pi} \; | \; k \in \Z \setminus
    \{0\}\}$.
  \item
    $\INTERPOLATION{\{(x_i, v_i)\}_{i=1}^3} \cap \MON{([0, 1], \ge)}$,
    where $x_1=-1$, $x_2=0$, $x_3=1$ and $v_1=0$, $v_2=2$, $v_3=1$.
  \item $\INV{\Omega} \cap \POS{\Omega}$, where $\Omega = [-1, 0] \times [-1, 0]$ forces $f_1$ to be zero on $\{0\} \times \mathbb R$.
  \end{itemize}
\end{theorem}

% \begin{theorem}[Meta-theorem]
%   Let $f$ be a vector fields satisfying properties $P_1, \ldots, P_n$.
%   If all properties $P_i$ are strict, and at most one the $P_i$ is
%   nonopen, then for any positive scalar $\varepsilon$, there exists a
%   polynomial vector field $p$ such that $p$ satisfies
%   $P_1, \ldots, P_n$ and $\|f - p\| \le \varepsilon$.
% \end{theorem}

\subsection{Limitations of polynomials vector fields}
There are obvious limitations to polynomial vector fields. Imposing
too many side information can make the problem in (*) infeasible.


\subsubsection{No polynomial vector field makes the set $\Omega$ invariant}
The set $\Omega \coloneqq \{ \frac1{2k\pi} \; | \; k \in \Z \setminus \{0\}\}$
is clearly invariant for the dynamical system
$\dot x = x^2 \sin(\frac 1x)$. If the same set is invariant for a
dynamical system $\dot x = f(x)$ given by a polynomial function $f$,
then $f$ needs to have infinitely many roots, and therefore $f$ must
be identically zero.

\subsubsection{No polynomial vector field respects monotonicity and equilibirum points}
There exists no polynomial vector field $p: \R \rightarrow \R$ that respects the following side information
\begin{itemize}
\item $p(-1) = p(0) = 0$ and $p(1) = 1$
\item $p$ nondecreasing.
\end{itemize}

The (infinitely-many-times differentiable) function
\[f(x) \coloneqq \left\{ \begin{array}{ll}0&\text{if }x \le 0\\e^{1-\frac1{x^2}}&\text{if } x > 0\end{array}\right\}\]
does respect this side info.


\subsubsection{No polynomial vector field respects monotonicity and invariance}
The zero vector field is the only polynomial vector field $p: \R \rightarrow \R$ that respects the following side information
\begin{itemize}
\item $p$ leaves the interval $[0, 1]$ invariant.
\item $p$ is nondecreasing on $[0, 1]$.
\end{itemize}



\subsection{Positive results about polynomials vector fields}


The next theorem proves that any continuous function $f$ can be approximated uniformly by a polynomial $p$ on a compact set, even if we impose that $f$ and $p$ be equal on any finite number of points.

\begin{theorem}
  Let $\Omega \subseteq \R^N$ be a compact subset of $\R^n$ and consider a continuous function $f:\Omega\rightarrow \R$.
  For any $\varepsilon > 0$, for any $d$ points $\x_1, \ldots, \x_d \in \Omega$,
  there exists a polynomial $p \in \R[\x]$ such that
  \[\ltwonorm{p(\x) - f(\x)} \le \varepsilon \quad \forall x \in \Omega \text{ and } f(\x_i) = p(\x_i) \forall i \in \{1, \ldots, d\}\].
\end{theorem}

\begin{proof}
  Let $f:\Omega\rightarrow \R^n$ be a continuous vector field and fix a positive scalar $\varepsilon$. By Weirstrass theorem, there exists a polynomial $q \in \R[\x]$ such that $\ltwonorm{p(x) - f(x)} \le \varepsilon$ for all $x \in \Omega$.
  Now let  $\x_1, \ldots, \x_n \in \Omega$, and set $v_i \coloneqq f(\x_i) - q(\x_i)$. By Proposition \ref{prop:mon_vectors_are_indep}, there exists a polynomial $s \in \R_d[\x]$ such $s(\x_i) = v_i$ and $\max_{\Omega} |s| \le C(\x_1, \ldots, \x_d) \|v\|_2 \le \sqrt{d}C(\x_1, \ldots, \x_d) \varepsilon$.
  We let $p = q + s$, so that for any $\x \in \Omega$,
  \[\|f(\x) - p(\x)\| \le \|f(\x) - q(\x)\| + \|s(\x)\| \le (1+\sqrt{d}C(\x_1, \ldots, \x_d))\varepsilon,\]
  and for $i=1,\ldots,d$, $f(\x_i) - p(\x_i) = 0$.
  
\end{proof}


In the next theorem we prove that on any compact set, we can we can approximate vector field $f$ that satisfies some monotonicity constraints $\frac{\partial f_i}{\partial \x_j} \sim_{ij} 0$, where $\sim_{ij} \in \{ \ge , \le \}$ with a polynomial vector field that satisfies the same monotonicity constraints.
\begin{theorem}
  Let $\Omega \subseteq \R^N$ be a compact subset of $\R^n$, and consider  a continuously differentiable function $f:\Omega\rightarrow \R$ that satisfies:
  \[f \ge 0 \quad \forall \ix \in P, \]
  \[\frac{\partial f}{\partial \x_j}(\ix) >_j 0 \quad \forall \ix \in M_j \forall j \in \{1, \dots, n\}, \]
  where $>_i$ is either $\ge$ or $\le$, and $P$ and the $M_j$ are semi-algebraic sets.
  Then, for any $\varepsilon > 0$, there exists a polynomial function $p: \R^n \rightarrow \R$ such that
  \[\ltwonorm{p(\ix) - f(\ix)} \le \varepsilon \; \forall \ix \in \R^n,\quad   p \ge 0 \; \forall \ix \in P,\]
    \[\text{ and }
    \frac{\partial p}{\partial \x_j}(\ix) >_j 0 \; \forall \ix \in  M_j \forall j \in \{1, \dots, n\}, \]
\end{theorem}
\begin{proof}
  Consider the function $\tilde f$ defined by \[\tilde f = f + \beta\left(1  + \sum_{i, >_i = \ge} x_i - \sum_{i, >_i = \le} x_i\right).\]
  Then
  \[\ltwonorm{\tilde f(\ix) - f(\ix)} \le  \beta\; \forall \ix \in \R^n,\quad   \tilde f \ge \beta \; \forall \ix \in P,\]
    \[\text{ and }
    \frac{\partial \tilde f}{\partial \x_j}(\ix) >_j \beta \; \forall \ix \in  M_j \forall j \in \{1, \dots, n\}, \]
  The result follows by approximating $\tilde f$ by a polynomial uniformly for the $C^1\text{-norm}$.
\end{proof}

\begin{theorem}
  Let $\Omega \subseteq \R^N$ be a compact subset of $\R^n$, and consider  a continuously differentiable function $V:\Omega\rightarrow \R$ that satisfies:
  \[\frac{\partial V}{\partial x_i} >_i 0 \quad \forall \ix \in P_i, \]
  Then, for any $\varepsilon > 0$, there exists a polynomial function $W: \R^n \rightarrow \R$ such that
  \[\ltwonorm{\nabla V(\ix) - \nabla W(\ix)} \le \varepsilon \; \forall \ix \in \Omega,\quad   \frac{\partial W}{\partial x_i} >_i 0.\]
\end{theorem}

\begin{proof}
  Let $\tilde V = V + \beta \sum_{i=1}^n \pm x_i$
\end{proof}





% \section{Certificates of positivity in a Box}

% \begin{theorem}[Stengle]\label{thm:positivity in a box}
%   If a polynomial $p(x, y) \in \R[x, y]$ is positive on the box given by $\{(x, y) \; | \; x, y, 1-x, 1-y \ge 0\}$, then there exist sos polynomials $(\sigma_\alpha(x, y))$ indexed by $\alpha \in \{0, 1\}^4$ such that: 
%   \[p(x, y) =  \sum_{\alpha \in \{0, 1\}^4} \sigma_{\alpha}(x, y) x^{\alpha_1}y^{\alpha_2}(1-x)^{\alpha_3}(1-y)^{\alpha_4}\]
% \end{theorem}


\subsection{Multivariate Polynomial Interpolation}
\begin{proposition}[Proposition 4.3 in \cite{comon_symmetric_2008}]\label{prop:mon_vectors_are_indep}
  If $\x^1, \ldots, \x^d$ are $d$ different points of $\R^n$, the $m_d (\x^1), \ldots, m_d(\x^d)$ are linearly independent, where $m_d(\x^i) = (\x^i_{j_1}\ldots\x^i_{j_d})_{j_1, \ldots, j_d \in \{1, \ldots, n\}}$ is the vector of monomials in $\x_i$ up to degree $d$.
\end{proposition}
\begin{corollary}
  For any positive integers $d$ and $n$, for any $d$ points $\x^1, \ldots, \x^d$ in a compact set $\Omega$, there exists a constant $C(\x_1, \ldots, \x_d)$ such that the following holds:\\
  For any vector $v \in \R^d$, there exists a polynomial $p \in \R_d[\x]$ such that
  \[p(\x_i) = v_i, \quad i=1,\ldots,d \text{ and } \max_{\x \in \Omega} |p(\x)| \le C(\x_1, \ldots, \x_d) \|v\|_2\]
\end{corollary}
\begin{proof}
  By Proposition \ref{prop:mon_vectors_are_indep}, the system of linear equations
  \begin{equation}\label{eq:lin_system_poly}
    p(\x_i) = v_i \quad i=1,\ldots,n
    \end{equation}
    in the variable $p \in \R_d[\x]$ are independent. If we identify $p$ by its coefficients in the monomial basis, then we can rewrite the system in \eqref{eq:lin_system_poly} as
    \[A p = v,\]
    where $A = (m_d(\x^1), \ldots, m_d(\x^d))^T$ is a matrix depending only on $\x_1, \ldots, \x_d$ that has independent rows.
    The corollary follows by taking $C(\x_1, \ldots, \x_d)$ to be the operator norm of the matrix $M \coloneqq (A^TA)^{-1}A^T$ and $p = Mv$, and  
\end{proof}





\section{Polynomial Approximation of Vector Fields}

\begin{theorem}[Invariance]
  If the dynamical system $\dot \ix = f(\ix)$ leaves a star-shaped $B$
  invariant, then for every $\varepsilon > 0$, there exists a
  polynomial vector field $p$ that leaves the set $V$ invariant and
  \[\|f - p\| \le \varepsilon.\]
\end{theorem}


\begin{theorem}[Equilibrium Points]
  If the dynamical system $\dot \ix = f(\ix)$ leaves a star-shaped $B$
  invariant, then for every $\varepsilon > 0$, there exists a
  polynomial vector field $p$ that leaves the set $V$ invariant and
  \[\|f - p\| \le \varepsilon.\]
\end{theorem}

\begin{theorem}
  Let $f$ be vector field satisfying one of the following side information
  \begin{itemize}
  \item Nonnegativity on a set $B_1$, monotonicity on a set $B_2$, and strict invariance of a set $B_3$.
  \item Nonnegativity on a set $B_1$ and interpolation conditions $f(x_1) = v_1$, \dots, $f(x_m) = v_m$.
  \item Invariance of full-dimensional, star-shaped set $\Omega$.
  \end{itemize}
  Then, for every $\varepsilon > 0$, there exists a polynomial $p$ such that $\|p - f\| \le \varepsilon$ and $p$ satisfies the same side information as $p$.
\end{theorem}




%%% Local Variables:
%%% mode: latex
%%% TeX-engine: luatex
%%% TeX-command-extra-options: "-shell-escape"
%%% TeX-master: "Learning_with_side_information_v1"
%%% End:


==> problem_formulation.tex <==
\section{Introduction}


In several safety-critical applications, one has to learn
the behavior of an unknown dynamical system from noisy
observations of a very limited number of trajectories. For
example, to autonomously land an airplane that has just
gone through engine failure, limited time is available to
learn the modified dynamics of the plane before appropriate
control action can be taken. Similarly, when a new
infectious disease breaks out, few observations are
initially available to understand the dynamics of
contagion.  In situations of this type where data is
limited, it is essential to exploit ``side
information''---e.g. physical laws or contextual
knowledge---to assist the task of learning.

In this paper, we present a mathematical formalism of the
problem of learning a dynamical system with side
information, where side information means a concrete
collection of local and global properties of the dynamical
system that are commonly encountered in practice. We show
that sum of squares optimization is particularly suited for
learning a dynamical system that best agrees with the
observations and respects the side information.


\section{Problem formulation}
Our interest in this paper is to learn a dynamical system
\begin{equation}
  \frac{{\rm d}}{{\rm d}t} \ix(t) = f(\ix(t)), \quad f: \Omega \rightarrow \mathbb R^n,
  \label{eq:autonomous.dynamical.system}
\end{equation}
over a given compact set $\Omega \subset \R^n$. We consider
the setting where the vector field
$f: \Omega \rightarrow \mathbb R^n$ is unknown to us, and we
only require it to be continuously differentiable. This
requirement is often met in applications of interest to us,
and is known to be a sufficient condition for existence and
uniqueness of trajectories (see
\cite{khalil2002nonlinear}). We assume that we have access
to a set $\mathcal D$ of \textit{training data} of observed
trajectories and to \textit{side information} (We give a
concrete mathematical definition of this notion in
\cref{sec:side-info} below). Our training data is a set of
the form
\begin{equation}
 \mathcal D \coloneqq \{ (\ix_i, \iy_i),\quad i = 1,\ldots,N\},\label{eq:training-set}
\end{equation}
%
%
where every $\ix_i$ is a vector of $\mathbb R^n$, and
$\iy_i$ is a noisy measurement of $f(\ix_i)$. 
%
The evaluation points $\ix_i$ are either fixed vectors of
$\Omega$, or emanating from one (or few) trajectories
$\ix(t)$ at some snapshot times $t_i$, i.e.,
$\ix_i = \ix(t_i)$. The vectors $y_i$ could be directly
given (e.g., from sensor data), or approximated using a
finite-difference scheme.

%
Finding a vector field $f_{\mathcal F}$ that best agrees with
the unknown vector field $f$ among a class of
continuously-differentiable functions of interest
$\mathcal F$ amounts to solving the least-squares problem
\begin{equation}
  \label{eq:program_fit_vector_field} f_{\mathcal F} \in \arg \min_{p \in
\mathcal F} \sum_{(\ix_i, \iy_i) \in \mathcal D} \|p(\ix_i) - \iy_i\|,
\end{equation}
It turns out that our approach can readily handle other
types of losses (e.g., $\ell_1$ and $\ell_\infty$ losses,
any sos-convex loss function [**]).


\subsection{Side information}
\label{sec:side-info}

In addition to consistency with $f$, we want our learned
vector field $f_{\mathcal F}$ to also generalize reasonably
well in conditions that were not seen in the training
data. Indeed, the optimization problem
in~\eqref{eq:program_fit_vector_field} only dictates how the
candidate vector field should behave on the training data,
which could easily lead to over-fitting, especially if the
class of function $\mathcal F$ is large enough and the
observations are noisy and limited. Let us demonstrate this
issue with a simple example.

\begin{example}Consider the two-dimensional vector field
  $f(x_1, x_2) \coloneqq (x_2, -x_1)^T$. The trajectories
  of the system $\dot \ix = f(\ix)$ are given by circular
  orbits. In particular, if started from the initial condition
  $x_0 \coloneqq (1, 0)^T$, this trajectory is given by
  $\ix(t, x_0) =(\cos(t), \sin(t))^T$. As a result, for any
  function $g:\mathbb R^2\rightarrow \mathbb R^2$, the vector field
  \[h(\ix) \coloneqq f(\ix) + (x_1^2+x_2^2-1) g(\ix)\]
  agrees with $f$ on the sample trajectory $\ix(t, x_0)$,
  but the behavior of the trajectory of $h$ depend on the
  arbitrary choice of $g$. If $g(\ix) = \ix$ for instance,
  the trajectories of $h$ starting outside of the unit disk
  will diverge exponentially fast to infinity.


\end{example}


To address both issues of over-fitting and scarcity of data,
we suppose that we know, in addition to the the training
data $\mathcal D$, that the vector field $f$ or its
trajectories possess some additional properties that we call
{\it side information}. Formally, every side information is
a subset $S$ of the set of all continuously-differentiable
vector fields.  Our goal is then to learn a polynomial
vector field $p$ that satisfies the same side information,
i.e. $p \in S$, and agrees with $f$ on the training data to
arbitrary accuracy. The problem of learning a polynomial
vector field $p \in \mathcal F$ from data $\mathcal D$ and
side information $S_1, \dots, S_m$ can thus be formulated as
\begin{equation}
  \label{eq:program_fit_vector_field_with_side_info} \min_{p
\in \mathcal F \cap S_1 \cap \dots \cap S_m} \sum_{(\ix_i,
\iy_i) \in \mathcal D} \|p(\ix_i) - \iy_i\|^2.
\end{equation}

For arbitrary side information $S_1, \ldots, S_m$, the
problem in
\eqref{eq:program_fit_vector_field_with_side_info} is
challenging one. We focus our attention on the six types of
side information below. On the one hand, as we will see in
the numerical application section, they appear ubiquitously
in real life applications. On the other hand, they lead to a
semidefinite programming formulation of the problem in
\eqref{eq:program_fit_vector_field_with_side_info}.


\newcommand{\INTERPOLATION}[1]{\operatorname{{\bf
      INTERP}}(#1)}
\newcommand{\POS}[1]{\operatorname{{\bf
      POS}}(#1)}
\newcommand{\MON}[1]{\operatorname{{\bf
      MON}}(#1)}
\newcommand{\INV}[1]{\operatorname{{\bf
      INV}}(#1)}
\newcommand{\GRAD}{\operatorname{{\bf
      GRAD}}}
\newcommand{\HAMILTONIAN}{\operatorname{{\bf
      HAM}}}
\newcommand{\SYM}[2]{\operatorname{{\bf
SYM}}(#1, #2)}

\begin{itemize}
\setlength\itemsep{0em}
  
\item {\bf Interpolation at a finite set of points.} For
  every points $\ix_1, \ldots, \ix_m \in \mathbb R^n$ and
  scalars $y_1, \ldots, y_m \in \R^n$, we denote
  by $\INTERPOLATION{\{\ix_i,y_i\}}_{i=1}^m$ the set of
  vector fields $f$ that satisfy $f(\ix_i) = y_i$ for
  $i=1,\dots,m$. As an important special case, consider the
  setting where the scalars $y_i$ are equal to $0$,
  then the points $\ix_i$ correspond to equilibrium points
  of the vector field~$f$.
  
\item {\bf Sign symmetry.} For any two $n \times n$ diagonal matrices $A$ and $B$ with $1$ or $-1$ on the diagonal, We define $\SYM A B$ to be the set of vector fields $f$ satisfying the symmetry condition
  \[f(A\ix) = Bf(\ix) \quad \forall \ix \in \R^n.\]
  Note that the set $\SYM{-I} I$ (resp. $\SYM {-I} {-I}$) is the set of even (resp. odd) vector fields, where $I$ is the $n\times n$ identity matrix.

  
\item {\bf Coordinate nonnegativity.}  For sets
  $B_i \subseteq \Omega$, we denote by
  $\POS{ \{\generalineq_i, B_i\}_{i=1}^n }$ the set of
  vector fields $f$ that satisfy
  $f_i(\ix) \generalineq_i 0 \; \forall \ix \in B_i$ for
  $i \in \{1, \dots, n\}$, where $\generalineq_i$ stands for $\ge$ or~$\le$.

\item {\bf Coordinate-directional monotonicity.} Similarly,
  for sets $B_{i,j} \subseteq \Omega$, we denote the
  set of vector fields $f$ satisfying
  $\frac {\partial f_i}{x_j} (\ix) \generalineq_{i,j} 0 \; \forall \ix \in B_{i,j}$ for
  $i, j \in \{1, \dots, n\}$ by $\MON{ \{\generalineq_{i,j}, B_{i, j}\}_{i, j=1}^n}$.
  
\item {\bf Invariance of a set $B$.} We say that a set
  $B \subseteq \Omega$ is invariant for the vector field $f$
  if any trajectory of the dynamical system
  $\dot \ix = f(\ix)$, when started inside the set $B$,
  never leave $B$.

  In particular, if the set $B$ is
  given by inequalities $h_i(\ix) \ge 0$ for $i =1,\dots,m$,
  where the $h_i$ are continuously-differentiable functions,
  then the invariance of the set $B$ is given by the
  mathematical conditions
  %
  \begin{equation}
    \label{eq:eq-invariance} \langle f(\ix), \nabla h_i(\ix) \rangle \ge 0 \; \forall
\ix \in B_i \quad \text{where} \; B_i = B \cap \{h_i(x) = 0\},\text{ and } i=1,\dots,m.
\end{equation}
%
The set of all vector fields for which the set $B$ is invariant is denoted by $\INV{B}$.
  
\item {\bf Gradient and Hamiltonian systems.}  The vector
  field $f$ is said to be a \textit{gradient} if there
  exists a scalar-valued function $V: \R^n \rightarrow \R$
  such that
\begin{equation}
    \label{eq:def-gradient} f(\ix) = - \nabla V(\ix)\; \forall
\ix \in \R^n.
\end{equation}
Typically, the function $V$ is interpreted as a potential or
energy that decreases along the trajectories of the
dynamical system $\dot x = f(x)$.
The set of gradient vector fields is denoted by $\GRAD$.

A dynamical system is said to be \textit{Hamiltonian} if the dimension $n$ of the state space $x$ is even (say $n \eqqcolon 2k$), and a scalar-valued function $H: \R^k \times \R^k \longrightarrow \R$ such that

  \[\dot \ip = - \frac{\partial H}{\partial \iq} (\ip, \iq)
    \text{ and } \dot \iq = \frac{\partial H}{\partial \ip}
    (\ip, \iq),\] where $\ip^T = (\ix_1, \ldots, \ix_k)^T$
  and $\iq^T = (\ix_{k+1}, \ldots, \ix_n)^T$. The
  coordinates $\ip$ and $\iq$ are usually called
  \textit{momentum} and \textit{position} respectively,
  following naming convention in the field of physics. Note
  that in a Hamiltonian system, the quantity $H$ is
  conserved along its trajectories.  The set of Hamiltonian
  vector fields is denoted by $\HAMILTONIAN$. See
  \cite{greydanus2019hamiltonian,cheng2015learn}.
  
\end{itemize}



%%% local Variables:
%%% mode: latex
%%% TeX-engine: default
%%% TeX-master: "Learning_with_side_information_L4DC_v1"
%%% End:


==> review_sos.tex <==
\section{Learning Polynomial Vector Fields Subject to Side Information}
\label{sec:learn-poly-vec}


To completely define the problem in
\cref{eq:program_fit_vector_field_with_side_info}, we still
have to specify the set $\mathcal F$. Among the possible
choices are reproducing kernel Hilbert spaces
\cite{sindhwani2018learning,cheng2015learn}, trigonometric
functions, and functions parameterized by neural networks
\cite{neural_laypunov_nips_2019,greydanus2019hamiltonian}.
In this paper, we will take $\mathcal F$ to be set
\[ \poly d \coloneqq \{ p: \R^n \rightarrow \R^n \; | \; p_i
  \text{ is a polynomial of degree $d$ for $i=1,\ldots,n$}
  \}.\] Furthermore, we will assume that all subsets of
$\Omega$ considered in \cref{sec:side-info} in the
definition of side information (i.e., the sets $B_i$ in the
definition of nonnegativity, the sets $B_{ij}$ for the
definition of monotonicity, and the set $B$ in the
definition of invariance) are all \emph{closed basic
  semi-algebraic sets}. We recall that a closed basic
semialgebraic set is a subset of the Euclidean space of the
form
\begin{equation}\nonumber
\SETALG \coloneqq \{x\in\mathbb{R}^n|\ g_i(x)\geq 0, i=1,\ldots,m  \},
\end{equation}
where $g_1,\ldots,g_m$ are polynomial functions.


These choices are motivated by two reasons. The first is that polynomial functions are expressive enough to approximate a large family of functions. The second reason which shall be made clear in this paper is that because of some connections between real algebra and semidefinite optimization, several side information constraints that are commonly available in practice can be imposed on polynomial vector fields in a numerically tractable fashion. We note that the problem of fitting a polynomial vector field to data has appeared e.g. in \cite{schaeffer2018polylasso}, though the focus there is on imposing sparsity of the coefficients of the vector field as opposed to side information. The closest work in the literature to our work is that of Hall on shape-constrained regression \cite[Chapter 8]{phd:georgina18}, where similar algebraic techniques are used to impose constraints such as convexity and monotonicity on a polynomial regressor. See also \cite{shapeconstraints_aaa} for some statistical properties of these regressors and several applications. Our work can be seen as an extension of this approach to a dynamical system setting.



The optimization problem of interest to us has as decision
variables the coefficients of a candidate polynomial vector
field $p$. The objective function is a convex quadratic
function of these coefficients, and the constraints are
twofold: (i) affine constraints in the coefficients of $p$,
and (ii) constraints of the form
\begin{equation}\label{eq:p>=0.on.Omega}
q(x)\geq 0\  \forall x\in \SETALG,
\end{equation}
where $\SETALG$ is a given closed basic semialgebraic set, and $q$
is a (univariate) polynomial whose coefficients depend
linearly on the coefficients of the polynomial $q$.  For
example, it is easy to see that membership to
$\INTERPOLATION{\{\ix_i,\alpha_i\}}_{i=1}^m$, $\GRAD$, and
$\HAMILTONIAN$ are all given by affine constraints, while
membership $\POS{ \{>_i, B_i\}_{i=1}^n }$,
$\MON{ \{>_{i,j}, B_{i, j}\}_{i, j=1}^n}$, and $\INV{B}$ can
be case as a constraint of the type in (ii). Unfortunately,
imposing the constraint in (\ref{eq:p>=0.on.Omega})
is NP-hard already when $q$ is a quartic polynomial and
$\SETALG=\mathbb{R}^n$, or when $q$ is quadratic and $\SETALG$ is a
polytope.

An idea pioneered to a large extent by Lasserre~\cite{lasserre_moment} and Parrilo~\cite{sdprelax} has been to write algebraic sufficient conditions for (\ref{eq:p>=0.on.Omega}) based on the concept of sum of squares polynomials. We say that a polynomial $h$ is a \emph{sum of squares} (sos) if it can be written as $h=\sum_i q_i^2$ for some polynomials $q_i$. Observe that if we succeed in finding sos polynomials $\sigma_0,\sigma_1,\ldots, \sigma_m$ such that the polynomial identity
\begin{equation}\label{eq:putinar-certificate}
q(x)=\sigma_0(x)+\sum_{i=1}^{m}\sigma_i(x)g_i(x)
\end{equation}
holds, then, clearly, the constraint in (\ref{eq:p>=0.on.Omega}) must be satisfied. When the degree of the sos polynomials $\sigma_i$ is bounded by an integer $r$, we refer to \cref{eq:Putinar.proof} as the \emph{$r\text{-degree}$ Putinar's certificate} corresponding to the polynomial inequality \eqref{eq:p>=0.on.Omega}. Conversely, a celebrated result in algebraic geometry~\cite{putinar1993positive} states that if $g_1,\ldots,g_m$ satisfy the so-called ``Archimedean property'' (a condition slightly stronger than compactness of the set $\SETALG$), then positivity of $q$ on $\Lambda$ guarantees existence of an $r\text{-degree}$ Putinar's certificate for some integer $r$ large enough.

%:\mathbb{R}^n\rightarrow\mathbb{R}

The computational appeal of the sum of squares approach stems from the fact that the search for sos polynomials $\sigma_0,\sigma_1,\ldots, \sigma_m$ of a given degree that verify the polynomial identity in (\ref{eq:Putinar.proof}) can be automated via semidefinite programming. This is true even when some coefficients of the polynomial $p$ are left as decision variables. This claim is a straightforward consequence of the following well-known fact (see, e.g.,~\cite{PhD:Parrilo}): A polynomial $h$ of degree $2d$ is a sum of squares if and only if there exists a symmetric matrix $Q$ which is positive semidefinite and verifies the identity $$h(x)=z(x)^TQz(x),$$ where $z(x)$ here denotes the vector of all monomials in $x$ of degree less than or equal to $d$.

%%% Local Variables:
%%% mode: latex
%%% TeX-engine: default
%%% TeX-master: "Learning_with_side_information_L4DC_v1"
%%% End:


==> table_sideinfo.tex <==
\begin{table}[]
\begin{tabular}{lllll}
vector field used & x1 & x2 &  &  \\
LSQ               &    &    &  &  \\
LSQ               &    &    &  &  \\
                  &    &    &  & 
\end{tabular}
\end{table}


\begin{table}[]
\begin{tabular}{lll}
LSQ & 0.45 &  0.4\\
EQ & 0.41 &  0.29\\
EQ+INV & 0.31 &  0.12\\
EQ+INV+MON & 0.01 &  0.01\\
TRUE & 0.0 &  0.0
\end{tabular}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "Learning_with_side_information_SIREV_v1"
%%% End:


==> theorems.tex <==
\section{Approximation Results}

\subsection{Measure of similarity between vector fields}

Fix a compact set $\Omega \subset \R^n$. In order the assess
how close two vector fields $f, g: \Omega \rightarrow \R^n$
are, we define the following two metrics. The first one
compares directly the values taken by $f$ and $g$ on the
compact set $\Omega$:
\[\metricsup{f-g}{\Omega} \coloneqq \max_{\ix \in \Omega}
  \ltwonorm{f(\ix)-g(\ix)}\] From a dynamics point view, we
are also interested in how different the trajectories of $f$
and $g$ starting from an invariant set $\Omega$ are after
some time $T > 0$, i.e.
\[\metricdyn{f, g}{\Omega}{T} \coloneqq \sup_{\ix_0 \in \Omega,
    t \in [0, T]} \max\{\ltwonorm{\ix(t, \ix_0) - \iy(t,
    \ix_0)}, \ltwonorm{\dot \ix(t, \ix_0) - \dot \iy(t,
    \ix_0)}\] where $\ix(t, \ix_0)$ (resp. $\iy(t, \ix_0)$)
is the trajectory starting from $\ix_0 \in \Omega$ and
following the dynamics of $f$ (resp. $g$).
%

The metric $\metricdyn{\cdot, \cdot}{\Omega}{T}$ is ``finer'' than
$\metricsup{\cdot}{\Omega}$.  Indeed, by noting that
$\dot \ix(0, \ix_0) = f(\ix_0)$ and
$\dot \iy(0, \ix_0) = g(\ix_0)$, we obtain that
$\metricdyn{f, g}{\Omega}{T} \le \metricsup{f -
  g}{\Omega}$. The next proposition shows a reverse
inequality for Lipchitz vector fields that leave the set
$\Omega$ invariant.

\begin{proposition}\label{prop:equivalence-metric-vf} Fix a compact
set $\Omega \in \R^n$ and two positive scalars $T$ and
$L$. There exists a constant $C_{\Omega,T,L}$ such that
\[\metricsup{f-g}{\Omega} \le \metricdyn{f, g}{\Omega}{T} \le
  C_{\Omega,T,L} \metricsup{f-g}{\Omega}\] for every
continuously-differentiable vector field $f$ and for every
continuously-differentiable and $L\text{-Lipchitz}$ vector
field $g$ that leave the set $\Omega$.
\end{proposition}

\subsection{Satisfying side information approximately}
In section, we introduce the following notion approximately satisfying
side information.
\begin{definition}($\delta\text{-satisfiability}$) For any
  $\delta >0$ and side information $S$ presented in
  \cref{sec:side-info}, we say that a vector field $f$
  $\delta\text{-satisfies}$ $S$, and we write
  $f \in S^{\delta}$, if for any equality $a = b$
  (resp. inequality $a \le b$) appearing in the definition
  $S$, the vector field $f$ satisfies the modified version
  $|a - b| \le \delta$ (resp. $a \le b + \delta$).
\end{definition}

\begin{example}
  A vector $f$  $\delta\text{-satisfies}$ the side information $\INTERPOLATION{\{\ix_i,\alpha_i\}}_{i=1}^m$ if
  \( \|f(x_i) - \alpha_i\| \le \delta \quad i=1,\ldots,m. \)
\end{example}

The motivation for this definition is three-fold. First, we are happy in practice with a solution that satisfies an approximate version of the constraint. Second, due to numerical considerations, solvers return only a solution that satisfies an approximate version of the constraint. Finally, due to algebraic and approximation-theoretic reasons, if we take as our class of admissible vector fields polynomials of some bounded degree, a polynomial vector field satisfying the side information exactly might be computationally hard to find or simply not exist.


\subsection{Semidefinite programming hierarchy for approximating continuously-differentiable vector fields}

Let us now introduce some notation. For any side information
introduced in \cref{sec:side-info} given by a set $S$, we
denote by $S^{(r)}$ (resp. $S^{\delta, (r)}$) the set
obtained from $S$ by replacing any inequality of type
\eqref{eq:p>=0.on.Omega} with the corresponding equality in
\eqref{eq:putinar-certificate} suggested by Putinar's
Positivstellensatz, with the degree of the multipliers $s_i$
capped at $r$. Similarly, we define $S^{\delta, (r)}$ to be the set obtained from $S^{\delta}$, the $\delta\text{-approximation}$ of $S$.

\begin{example}
  % If \(S = \INTERPOLATION{\{\ix_i,\alpha_i\}}_{i=1}^m\),
  % then $S^{(r)} = S$ for all integers $r$. 
  If \(S = \INV B\), and $B$ is a closed semialgebraic set
  defined by polynomial inequalities $h_i(\ix) \ge 0$ for
  $i =1,\dots,m$, then, in view of \eqref{eq:eq-invariance},
  the set $S^\delta$ is given by continuously-differentiable vector fields $f$ that satisfy
  \[\langle f(\ix), \nabla h_j(\ix) \rangle \ge -\delta \quad \forall x \in B \cap \{h_j(x) = 0\}.\]
  Elements of \(S^{\delta, (r)}\)  are
  given by polynomial vector fields $p$ that satisfy the
  equalities
  \[\langle p(\ix), \nabla h_j(\ix) \rangle + \delta = \sum_{i=1}^m s_i^{(j)}(\ix) h_i(\ix) + r^{(j)}(\ix) h_j(\ix) \quad \forall x \in B \cap \{h_j(x) = 0\}\]
  for \(j=1,\ldots,m\), where the $r^{(j)}$
  (resp. $s^{(j)}_i$) are polynomials (resp. sos
  polynomials) of degree $r$.
\end{example}



The following theorem shows that polynomial vector fields can approximate any vector fields $f$ and satisfy the same side information as $f$ (up to an arbitrarily small error tolerance $\delta$).

\begin{theorem}\label{thm:poly_approx}
  Fix a compact set $\Omega \subset \R^n$, a time horizon
  $T > 0$, a desired accuracy $\varepsilon > 0$, and a room
  of error $\delta$. Let $f: \R^n \rightarrow \R^n$ be a
  continuously differentiable vector field that satisfies any
  combination of the side information in
  \cref{sec:side-info}. Then, there exists a polynomial
  vector field $p: \R^n \rightarrow \R^n$ such that
\[\metricdyn{f, p}{\Omega}{T} \le \varepsilon,\]
and $p$ $\delta\text{-satisfies}$ the same side information as $f$.
\end{theorem}

It should be clear that for any integer $r$ and scalar
$\delta$, the constraint ``$q~\in~S^{\delta, (r)}$'' is a
semidefinite-programming constraint. The following theorem
leverages this observation to show that the problem of
learning a polynomial vector field with side information can
be cast as a semidefinite program.


\begin{theorem}\label{thm:sdp_finds_best_poly}
  Fix a time horizon $T > 0$, a desired
  accuracy $\varepsilon > 0$, and a error tolerance
  $\delta > 0$. Let $f: \Omega \rightarrow \R^n$ be
  a continuous differentiable vector field that satisfies
  side information $S_1, \ldots, S_m$, and $\mathcal D$ be a training data. For $d$ and $r$ large enough, the semidefinite program 

  \begin{equation}
    \label{eq:learn_poly_vf_as_sdp}
    \begin{split}
    \min_{p \in \poly d}&
    \sum_{(\x_i, \iy_i) \in \mathcal D}
    \|p(\x_i) - \iy_i\|^2\\
    &p \in S_i^{\delta, (r)} \quad \text{for $i=1,\ldots,m$}.
    \end{split}
  \end{equation}
  becomes feasible. Furthermore, if we denote by
  $p^{d,r,\delta}$ an optimal solution to
  \eqref{eq:learn_poly_vf_as_sdp}, then the sequence of
  losses
  $\{\sum_{(\x_i, \iy_i) \in \mathcal D}
  \|p^{d,r,\delta}(\x_i) - \iy_i\|^2\}_{d,r}$ 
  is decreasing in both $d$ and $r$, and its limit as
  $d, r \rightarrow \infty$ is at most equal to
  $\sum_{(\x_i, \iy_i) \in \mathcal D} \|f(\x_i) -
  \iy_i\|^2$.
\end{theorem}


\subsection{Approximation of vector fields by polynomials that satisfy side information exactly}

In the previous section, we showed that polynomials are good
candidate for the task of learning vector fields from data
and side information if one is allowed to satisfy the side
information only approximately. Nevertheless, we think that
the mathematical question of deciding whether it is possible
to approximate an unknown vector field with a polynomial
vector field satisfying a given collection of side
information exactly is an interesting one. We give a
positive and a negative result in this direction.


The following definition establishes a notation that we will use in the statement of the results of this section.

\begin{definition}\label[definition]{def:strict_convex_set}
A closed semialgebraic set is said to be strictly convex if (i) it is defined by finitely many inequalities $h_i(x) \ge 0$, where the $h_i$ are convex polynomials, and (ii) there exists $x_* \in \R^n$ such that $h_i(x_*) > 0 \; \forall i$.
\end{definition}


\begin{theorem}
  Fix a compact set $\Omega \subset R^n$, a time horizon $T > 0$, and a desired accuracy $\varepsilon > 0$. Let $f: \mathbb R^n \rightarrow \mathbb R^n$ be a continuous differentiable vector field that satisfies exactly one of the following constraints
(i) equilibria at a given finite set of points,
(ii) invariance of a strictly convex set,
(iii) directional monotonicity,
(iv) nonnegativity,
(v) gradient or Hamiltonian structure,
(vi) sign symmetry.
Then there exists a polynomial vector field $p: \mathbb R^n \rightarrow \R^n$ such that
\[\metricdyn{f, p}{\Omega}{T} \le \varepsilon,\]
and $p$ satisfies the same side information as $f$. Furthermore, all such properties of $p$ come with an SOS certificate.
\end{theorem}

A natural question is whether the previous theorem could be generalized to allow for polynomial approximation of vector fields satisfying \emph{combinations} of side information exactly. The next simple example shows that the answer is negative, even when the dimension of the state variable is one.


\begin{example}
  Let $f:[-1, 1]\rightarrow\R$ be the continuously differentiable function defined piece wise by $f(x) = 0$ when $x < 0$ and $f(x) = e^{-1/x^2}$. The function $f$ can be viewed as vector field satisfying the side information (i) $S_1 \coloneqq \INTERPOLATION{ (-1, 0), (0, 0)}$ (i.e., $f(-1) = f(0) = 0$) and (ii) $S_2  \coloneqq \MON{[-1, 1], \ge}$ (i.e., $f$ nondecreasing on $[-1, 1]$). However, it is easy to see that the only polynomial contained in $S_1 \cap S_2$ is the identically zero polynomial.
\end{example}


The next example shows that even in the case where the unknown vector field happen to be polynomial, 

\begin{example}
  Denote by $p$ the polynomial
  $x_1^4x_2^2 + x_1^2x_2^4 + x_3^6 - 3x_1^2x_2^2x_3^2,$
  known as the Motzkin polynomial, and let
  $g(x_1, x_2, x_3) \coloneqq 1 - (x_1^2 + x_2^2 + x_3^2)$.
  The polynomial $p$ is nonnegative on the unit ball
  \(\SETALG \coloneqq \{x \in \R^3 \; | \; g(x) \ge 0\},\)
  yet there exists no certificate of the form in
  \eqref{eq:putinar-certificate} to prove it, i.e., there
  exist no sum of squares $s_0$ and $s_1$ that satisfy
  $p = s_0 + s_1 g$ (see
  \cite{motzkin_not_sos_ball_nie_2013}). This shows that the
  assumption that $p$ be positive (and not simply
  nonnegative) is truly needed for the result of
  \cref{th:putinar} to hold. We can use this observation to
  show that setting $\delta = 0$ in
  \cref{thm:sdp_finds_best_poly} would lead to an infeasible
  problem. Indeed, take $n=3$, $d=3$, and
  $S_1 = \INTERPOLATION{\{x_i, f(x_i)\}}$, then
  $S_1 \cap \poly 3 = \{ f \}$ but
  $S_1^{(r)} \cap \poly 3 = \emptyset$ for any integer $r$.
\end{example}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "Learning_with_side_information_L4DC_v1"
%%% End:


==> tikz_img/cancer_true_vf.tex <==
\loadvf{data/cancer/segments_two_compartment_model_vf.csv}{data/cancer/arrows_two_compartment_model_vf.csv}
\begin{figure}[H]
  \centering
  \begin{tikzpicture}
    \begin{axis}[no markers, enlargelimits=false, scale=1,
      xmin=-.1,xmax=2,
      ymin=-.1,ymax=2]
      \plotsegmentsvf{}
      \plotarrowsvf{}
      \draw[dashed, red, very thick] (0, -.1) -- (0, 4);
      \draw[dashed, red, very thick] (-.1, 0) -- (4, 0);
      \addplot[only marks, mark=*, red] table [x=N, y=K, col sep=comma]
      {data/cancer/cancer_data_points.csv};
    \end{axis}
    
  \end{tikzpicture}
  \caption{{\label{fig:two_compartment_model_vf}Vector
  field describing the dynamics of the population of tumor cells.}}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-engine: luatex
%%% TeX-master: "main.tex"
%%% End:


==> tikz_img/comparison_trajectory_pendulum.tex <==
\begin{figure}[H]
  \begin{tikzpicture}
    \begin{groupplot}[group style={
                              group size=1 by 3,
                              vertical sep=2cm,
                              ylabels at=edge left},
                              width=.75\textwidth,
                              height=6cm]
\nextgroupplot[title = {Trajectories generated form the polynomial vector field learned from data.}, legend pos=north east, xlabel=$t$, ylabel=$\theta(t)$]{
    \addlegendentry{Data}
    \addplot[restrict x to domain=0:3.1, mark=*, red, mark repeat={10}] table [x=t, y=theta1, col sep=comma]
    {data/pendulum/trajectory_simple_pendulum_true_vf.csv};

    \addlegendentry{Ground truth}
    \addplot[smooth, restrict x to domain=0:20,  red, dashed] table [x=t, y=theta1, col sep=comma]
    {data/pendulum/trajectory_simple_pendulum_true_vf.csv};

    \addlegendentry{Polynomial vector field}
    \addplot[smooth] table [x=t, y=theta1, restrict x to domain=0:20,
    col sep=comma]
    {data/pendulum/trajectory_simple_pendulum_poly_vf.csv};

    \addplot[dashed, mark=none] coordinates {(3, -1) (3, 2)};
    \coordinate (top) at (axis cs:1,\pgfkeysvalueof{/pgfplots/ymax});
  }
  
\nextgroupplot[align=center, title = {Trajectories generated form the polynomial vector field learned from data taking\\ into account all the side info.}, legend pos=north east, xlabel=$t$, ylabel=$\theta(t)$, xtick={0, 5, ..., 20}, yticklabels={$-\frac{\pi}4$, $0$, $\frac{\pi}{4}$}, ytick={-0.7854, 0, 0.7854}]{
 % \begin{axis}[legend pos=outer north east, xlabel=$t$, ylabel=$\theta$]
    \addlegendentry{Data}
    \addplot[restrict x to domain=0:3.1, mark=*, red, mark repeat={10}] table [x=t, y=theta1, col sep=comma]
    {data/pendulum/trajectory_simple_pendulum_true_vf.csv};

    \addlegendentry{Ground truth}
    \addplot[smooth, restrict x to domain=0:20,  red, dashed] table [x=t, y=theta1, col sep=comma]
    {data/pendulum/trajectory_simple_pendulum_true_vf.csv};

    \addlegendentry{Poly+side info}
    \addplot[smooth] table [x=t, y=theta1, restrict x to domain=0:20,
    col sep=comma]
    {data/pendulum/trajectory_simple_pendulum_hamiltonian_sym_pos_vf.csv};

    \addplot[dashed, mark=none] coordinates {(3, -1) (3, 2)};
    \coordinate (bot) at (axis cs:1,\pgfkeysvalueof{/pgfplots/ymin});
  }
  \end{groupplot}
  %\draw [thin] (top) -- (bot);


  \end{tikzpicture}
  \caption{\label{fig:abserror}Plot showing (a) position ${\mathbf{P_{T}}}$ and (b) the Parameters Absolute Errors.}
\end{figure}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End:


==> tikz_img/disease_true_vf.tex <==
\newcommand{\boxtikz}{\draw[dashed] (0,0) -- (1,0) -- (1,1) -- (0,1) -- (0,0);}

\begin{figure}[ht!]
  \centering
  \begin{tikzpicture}
    \begin{axis}[no markers, enlargelimits=false]
      \boxtikz
      \plotsegmentsvf{}
      \plotarrowsvf{}
      \addplot[red, thick, mark=+,  mark size=8pt] table [x=x, y=y]{data/disease/disease_training_data.csv};
    \end{axis}
  \end{tikzpicture}
  \caption{\label{fig:vf_diffusion_disease}The vector field in \eqref{eq:diffusion_disease} corresponding to $(a_1, a_2, b_1, b_2, c_1, c_2) = (.05,.1,.05,.1,1.,1.)$ together with some sample trajectories.}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> tikz_img/invariance_explanation.tex <==
\begin{center}
  \begin{tikzpicture}[scale=.2]
    \draw[rounded corners=.5cm] (0,0) -- (0,5) -- (10,10) -- (15, 5) -- (10,0) -- cycle node[text=black] {$\partial B$};
    \draw[rounded corners=.5cm, fill=gray!20] (0,0) -- (0,5) -- (10,10) -- (15, 5) -- (10,0) -- cycle;
    \draw[blue, -{Latex[length=2mm, width=1mm]}] (5, 7.5) -- (3, 10)node[left]{$n(x)$};
    \draw[red, -{Latex[length=2mm, width=1mm]}] (5, 7.5) -- (3, 5)node[right]{$p(x)$};
  \end{tikzpicture}
\end{center}

  
%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> tikz_img/plot_cancer_N_K.tex <==

\begin{tikzpicture}
  \begin{axis}[legend pos=north west,
    xlabel=$t$]
  \addplot[smooth, mark=*,each nth point={10},red] table [x=t, y=K, col
  sep=comma] {data/cancer/trajectory_grwoth_tumor.csv};
  \addlegendentry{$K(t)$}
  \addplot[smooth, mark=+,each nth point={10},blue] table [x=t, y=N, col sep=comma]
  {data/cancer/trajectory_grwoth_tumor.csv};
  \addlegendentry{$N(t)$}
\end{axis}
\end{tikzpicture}

%%% Local Variables:
%%% mode: latex
%%% TeX-engine: luatex
%%% TeX-master: "main.tex"
%%% End:







==> tikz_img/vf_learned_cancer.tex <==
\newcommand{\plotcancerlearnedvf}[3]{
  \nextgroupplot[align=left, title = {#2}, enlargelimits=false,
  xmin=-.1,xmax=2,
  ymin=-.1,ymax=2]{
    \loadvf{data/cancer/segments_#1.csv}{data/cancer/arrows_#1.csv}
    \plotsegmentsvf{}
    \plotarrowsvf{}
    \draw[dashed, red, very thick] (0, -.1) -- (0, 4);
    \draw[dashed, red, very thick] (-.1, 0) -- (4, 0);
    #3
}
}


\begin{figure}[H]
  \begin{tikzpicture}
    \begin{groupplot}[group style={
                              group size=2 by 1,
                              vertical sep=2cm,
                              ylabels at=edge left},
                              width=.5\textwidth,
                              height=6cm]
\plotcancerlearnedvf{two_compartment_model_learned_vf_no_side_info_deg_4}
{\label{fig:two_compartment_model_learned_vf_no_side_info}Best polynomial vector field of\\ degree 4 without side info.}{\draw[dashed, black, very thick] (0.05, 1.8) circle (.4cm);}

\plotcancerlearnedvf{two_compartment_model_learned_vf_with_side_info_deg_4}{\label{fig:two_compartment_model_learned_vf_with_side_info}Best polynomial vector field\\ of degree 4 with side info.}{}
\end{groupplot}
\end{tikzpicture}
\caption{Learned vector fields with and without side information.}

\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-engine: luatex
%%% TeX-master: "main.tex"
%%% End:
 

==> tikz_img/vf_learned_pendulum.tex <==
\newcommand{\plotpendulumlearnedvf}[3]{
  \nextgroupplot[title = {#2}, enlargelimits=false,
  xtick={-3.14, 0, 3.14}, xticklabels={$-\pi$, $0$, $\pi$},
  ytick={-3.14, 0, 3.14}, yticklabels={$-\pi$, $0$, $\pi$}]{
    \loadvf{data/pendulum/segments_#1_vf.csv}{data/pendulum/arrows_#1_vf.csv}
    \plotsegmentsvf{}
    \plotarrowsvf{}
    \draw[red, dashed, very thick] (-3.14,-3.14) -- (-3.14,3.14) --
    (3.14,3.14) -- (3.14,-3.14) -- cycle;
    \addplot[restrict x to domain=0:3.1, only marks, mark=*, red, mark repeat={10}] table [x=theta1, y=theta_dot1, col sep=comma]
    {data/pendulum/trajectory_simple_pendulum_true_vf.csv};
    \addplot[restrict x to domain=0:3.1, only marks, mark=*, red, mark repeat={10}] table [x=theta2, y=theta_dot2, col sep=comma]
    {data/pendulum/trajectory_simple_pendulum_true_vf.csv};
    #3
    
}
}


\begin{figure}[H]
  \begin{tikzpicture}
    \begin{groupplot}[group style={
                              group size=2 by 2,
                              vertical sep=2cm,
                              ylabels at=edge left},
                              width=.5\textwidth,
                              height=6cm]
\plotpendulumlearnedvf{poly}{Polynomial}{}
\plotpendulumlearnedvf{hamiltonian}{Hamiltonian}{}
\plotpendulumlearnedvf{hamiltonian_sym}{Hamiltonian + Symmetry}{
  \draw[dashed, black, very thick] (-3.14,3.14) circle (.4cm);
}
\plotpendulumlearnedvf{hamiltonian_sym_pos}{Hamiltonian + Symmetry +
  Pos}{}
\end{groupplot}

\end{tikzpicture}
\caption{Learned vector fields with side information.}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-engine: luatex
%%% TeX-master: "main.tex"
%%% End:
 

==> tikz_img/vf_true_pendulum.tex <==
\begin{figure}[H]
  \centering
    \loadvf{data/pendulum/segments_true_vf.csv}{data/pendulum/arrows_true_vf.csv}
  \begin{tikzpicture}
    \begin{axis}[no markers, enlargelimits=false]
        \plotsegmentsvf{}
        \plotarrowsvf{}
    \end{axis}
  \end{tikzpicture}
  \caption{True pendulum vector field}
\end{figure}



